Wasserstein Auto-encoded MDPs: Formal Verification of Efficiently Distilled RL Policies with Many-sided Guarantees

Although deep reinforcement learning (DRL) has many success stories, the large-scale deployment of policies learned through these advanced techniques in safety-critical scenarios is hindered by their lack of formal guarantees. Variational Markov Decision Processes (VAE-MDPs) are discrete latent space models that provide a reliable framework for distilling formally verifiable controllers from any RL policy. While the related guarantees address relevant practical aspects such as the satisfaction of performance and safety properties, the VAE approach suffers from several learning flaws (posterior collapse, slow learning speed, poor dynamics estimates), primarily due to the absence of abstraction and representation guarantees to support latent optimization. We introduce the Wasserstein auto-encoded MDP (WAE-MDP), a latent space model that fixes those issues by minimizing a penalized form of the optimal transport between the behaviors of the agent executing the original policy and the distilled policy, for which the formal guarantees apply. Our approach yields bisimulation guarantees while learning the distilled policy, allowing concrete optimization of the abstraction and representation model quality. Our experiments show that, besides distilling policies up to 10 times faster, the latent model quality is indeed better in general. Moreover, we present experiments from a simple time-to-failure verification algorithm on the latent space. The fact that our approach enables such simple verification techniques highlights its applicability.

==> abstract.tex <==
We consider the challenge of policy simplification and verification in the
context of policies learned through reinforcement learning (RL) in continuous environments. In well-behaved settings, RL algorithms have convergence
guarantees in the limit. While these guarantees are valuable, they are insufficient for
safety-critical applications. Furthermore, they are lost when
applying advanced techniques such as deep-RL. To recover guarantees when
applying advanced RL algorithms to  more complex environments with (i)
reachability, (ii) safety-constrained reachability, or (iii) discounted-reward
objectives, we build upon the DeepMDP framework introduced by Gelada et al. to
derive new bisimulation bounds between the unknown environment and a learned discrete
latent model of it. Our bisimulation bounds enable the application of
formal methods for Markov decision processes. Finally, we
show how one can use a policy obtained via state-of-the-art RL to efficiently train a
variational autoencoder that yields a discrete latent model with provably
approximately correct bisimulation guarantees. Additionally, we obtain
a distilled version of the policy for the latent model.

==> deepmdp.tex <==
From now on, fix MDPs $\mdp = \mdptuple$ and $\latentmdp = \latentmdptuple$ such that $\latentstates$ is equipped with metric $\distance_{\latentstates}$.
Let $\embed\colon \states \to \latentstates$ and $\embeda \colon \states \times \latentactions \to \actions$ be respectively state and action \emph{embedding functions}.
Intuitively, $\embed$ and $\embeda$ connect the state and action spaces of the two MDPs.
We refer to $\tuple{\latentmdp, \embed, \embeda}$ as a \emph{latent space model} of $\mdp$ and $\latentmdp$ as its \emph{latent MDP}.
We write $\latentmpolicies = \mpolicies{\latentmdp}$, and ${\latentvaluessymbol{\latentpolicy}{}}$ (resp. ${\latentqvaluessymbol{\latentpolicy}{}}$) for the value (resp. action-value) function of a policy $\latentpolicy \in \latentmpolicies$ in $\latentmdp$.
We can also consider $\latentpolicy$ as a policy in $\mdp$, where states passed to $\latentpolicy$ are embedded with $\embed$. Then, actions executed are embedded with $\embeda$.
Let $\latentpolicy \in \latentmpolicies$ and $\state \in \states$, we write $\latentaction \sim \latentpolicy\fun{\sampledot \mid \state}$ for $ \latentaction \sim \latentpolicy\fun{\sampledot \mid \embed\fun{\state}}$.
We further write $\qvalues{\latentpolicy}{}{\state}{\latentaction}$ as shorthand for $\qvalues{\latentpolicy}{}{\state}{\embeda\fun{\state, \latentaction}}$.
%$\action \sim \latentpolicy\fun{\sampledot \mid \state} \equiv \latentaction \sim \latentpolicy\fun{\sampledot \mid \state}, \,\action = \latentaction$
%Note that we can similarly define latent space models where $\mdp$ and $\latentmdp$ share the same action space $\actions$. In that case, the embedding action function $\embeda\fun{\state, \sampledot}$ is the identity function for all $\state \in \states$.

A particular point of interest is to focus on discrete latent models when $\mdp$ is continuous.
In that case, we assume $\distance_{\latentstates}$ to be the discrete metric, i.e., $\condition{\neq}$.
%This enables the use of model checking to verify properties in $\latentmdp$.
% and synthesis to construct policies in $\latentpolicies$.
%
% \subsection{Definitions}
%
In the following, we adopt the latent space model formalism of
\citet{DBLP:conf/icml/GeladaKBNB19}.
%\todo{F: I cut here. We already mentioned that in the intro}
% They refer to their models as \emph{DeepMDPs}, i.e., latent space models where $\embed$ is learned through the minimization of tractable losses (usually via neural networks). %, coming with theoretical guarantees.
% Note that they focus on the continuous setting and they do not consider action embedding functions.
%\FD{I revised this sub-section. Smooth-valuations and Lipschitzness definitions have been moved to the Appendix.}

\smallparagraph{Notations.}~Let $\latentpolicy \in \latentmpolicies$, we write $\Rmax{\latentpolicy}$ for $\sup_{\latentstate \in \latentstates} \left| \latentrewards_{\latentpolicy}\fun{\latentstate} \right|$.
We say that $\latentmdp$ is \emph{$\langle \KR{\latentpolicy}, \KP{\latentpolicy}\rangle$-Lipschitz} if for all $\latentstate_1, \latentstate_2 \in \latentstates$,
\begin{align*}
    \left|\latentrewards_{\latentpolicy}\fun{\latentstate_1} - \latentrewards_{\latentpolicy}\fun{\latentstate_2}\right| &\leq \KR{\latentpolicy} \distance_{\latentstates}\fun{\latentstate_1, \latentstate_2},\\
    \wassersteindist{\distance_{\latentstates}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{ \latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}} &\leq \KP{\latentpolicy} \distance_{\latentstates}\fun{\latentstate_1, \latentstate_2}.
\end{align*}
% In the discrete setting, we omit the $\distance_{\latentstates}$ terms.

%\smallparagraph{Local losses.}~%
%While global losses introduced by \cite{DBLP:conf/icml/GeladaKBNB19} are theoretically interesting, they depend on operations over the whole state-action space of $\mdp$, making them infeasible to approximate (and further be optimized).
%Moreover, when focusing on the behavior of $\mdp$ under a given a policy, it is rather interesting to focus on parts of the state space reachable when executing this policy, instead of considering the whole, possibly irrelevant, state space of $\mdp$.
\smallparagraph{Local losses.}~%
% \emph{Local losses} are measured under an expectation over a
% state-action distribution $\stationary{}$ and are defined as:% follows:
Let $\stationary{} \in \distributions{\states \times \actions}$,
\emph{local losses} are defined as:% follows:
\begin{align*}
    \localrewardloss{\stationary{}} &= \expectedsymbol{\state, \latentaction \sim \stationary{}}\left| \rewards\fun{\state, \latentaction} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right|, \\
    \localtransitionloss{\stationary{}} &= \expectedsymbol{\state, \latentaction \sim \stationary{}} \wassersteindist{\distance_{\latentstates}}{\embed\probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}
\end{align*}
where (i) $\rewards\fun{\state, \latentaction}$, (ii)
$\probtransitions\fun{\sampledot \mid \state, \latentaction}$, and (iii)
$\embed\probtransitions\fun{\sampledot \mid \state, \latentaction}$ are
shorthand for (i) $\rewards\fun{\state, \embeda\fun{\state, \latentaction}}$,
(ii) $\probtransitions\fun{\sampledot \mid \state, \embeda\fun{\state,
\latentaction}}$, and (iii) the distribution over $\latentstates$ of sampling
$\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}$ and
then embedding $\latentstate' = \embed\fun{\state}$. %
% where $\rewards(\state, \latentaction) = \rewards(\state, \embeda(\state, \latentaction))$,
% $\probtransitions(\sampledot \mid \state, \latentaction) = \probtransitions(\sampledot \mid \state, \embeda(\state,
% \latentaction))$, and
% $\embed\probtransitions(\latentstate' \mid \state, \latentaction) = \condition{=}(\embed(\state'), \latentstate') \cdot \probtransitions(\state' \mid \state, \latentaction)$ for all $\latentstate' \in \latentstates$.%
% The expectation term enables the use of stochastic gradient descent methods to optimize the two losses, which make them particularly interesting in practice.
%These losses allow bounding the difference between values of the original MDP $\mdp$ and those of its latent abstraction $\latentmdp$.

Henceforth, we make the following assumptions.
%From now on, we restrict our attention to the following setting.
\begin{assumption}\label{assumption:ergodicity}
MDP $\mdp$ is ergodic.
\end{assumption}
\begin{assumption}\label{assumption:rewards}
Rewards of $\mdp$ are scaled in the interval $\mathopen[ -\frac{1}{2}, \frac{1}{2}\mathclose]$, i.e., $\rewards \colon \states \times \actions \to \mathopen[ -\frac{1}{2}, \frac{1}{2}\mathclose]$.
\end{assumption}
\begin{assumption}\label{assumption:labeling}
The embedding function preserves the labels, i.e., $\embed\fun{\state} = \latentstate \implies \labels\fun{\state} = \latentlabels\fun{\latentstate}$ for $\state \in \states$, $\latentstate \in \latentstates$. 
\end{assumption}
The first assumption amounts to considering a reset of the environment is part of $\mdp$ (see \citealt{DBLP:conf/nips/Huang20} for details).
Assuming $\latentmdp$ is discrete, all $\wassersteinsymbol{\distance_{\latentstates}}$ terms can be replaced by $\dtvsymbol$ %we have $\localtransitionloss{\stationary{}} = \dtv{\embed\probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}$
since Wasserstein coincides with TV when using the discrete metric.
In that case, (optimal) constants $\KR{\latentpolicy}$ and
$\KP{\latentpolicy}$ can be computed in polynomial time in $\latentmdp$ for any $\latentpolicy \in \latentmpolicies$.

Proofs of the claims made in the following two subsections are provided in supplementary material (Appendix~\ref{appendix:section:latent-space-model}).
% Moreover, w.l.o.g., $\KR{}$ allows us to scale the rewards of $\latentmdp$ in any desired interval.


\subsection{Bisimulation and Value Difference Bounds}

%With the end-goal of enabling the model checking
%and synthesis
%of $\mdp$ given a discrete latent space model $\tuple{\latentmdp, \embed,
%\embeda}$ of $\mdp$, 
We aim now at formally checking
%and 
%quantifying 
whether
the latent space model offers a good abstraction of the original MDP $\mdp$.
%or not.
To do so, we present bounds that link the two MDPs.
We extend the bounds from \citet{DBLP:conf/icml/GeladaKBNB19} to discrete spaces while additionally taking into account state
labels and discounted reachability events.
Moreover, we present new \emph{bisimulation} bounds in the local setting.
%We start with the notion of \emph{bisimulation}.

\smallparagraph{Bisimulation.}
A \emph{(probabilistic) bisimulation}
is a behavioral equivalence between states. 
Formally, a bisimulation on $\mdp$ is an equivalence relation $B_{\Phi}$ such
that for all $\state_1, \state_2 \in \states$ and $\Phi \subseteq
\set{\rewards, \labels}$, $\state_1 B_{\Phi} \state_2$ iff
$\probtransitions\fun{T \mid \state_1, \action} = \probtransitions\fun{T \mid
\state_2, \action}$,
$\labels\fun{\state_1} = \labels\fun{\state_2}$ if  $\labels
    \in \Phi$,  and $\rewards\fun{\state_1, \action} = \rewards\fun{\state_2, \action}$ if $\rewards \in \Phi$,
% $\labels\fun{\state_1} = \labels\fun{\state_2}$, $\rewards\fun{\state_1, \action} = \rewards\fun{\state_2, \action}$ and $\probtransitions\fun{T \mid \state_1, \action} = \probtransitions\fun{T \mid \state_2, \action}$
for each action $\action \in \actions$, and (Borel measurable) equivalence class $T \in \states / B_{\Phi}$.
Properties of bisimulation include trace, trajectory, and value equivalence \citep{DBLP:conf/popl/LarsenS89,DBLP:journals/ai/GivanDG03}.
%Of particular interest is the maximal bisimulation relation which defines the partition with the fewest elements.
The relation can be extended to compare two MDPs (in our case $\mdp$ and $\latentmdp$) by considering the disjoint union of their state space.
We denote the largest bisimulation relation by $\sim_{\Phi}$.

\smallparagraph{Pseudometrics.}
%Bisimulation relations are often too conservative when applied over uncountable state spaces.
%Intuitively, this is due to their ``all-or-nothing'' nature: two states having nearly identical but slight numerical difference in their rewards or probability transitions are treated as completely different. %, leading to different bisimulation partitions.
\citet{DBLP:journals/tcs/DesharnaisGJP04} introduced \emph{bisimulation pseudometrics} for continuous Markov processes, generalizing the notion of bisimilariy by assigning a \emph{bisimilarity distance} between states. % to quantify their behavioral similarity.
A \emph{pseudometric} $\bidistance$ satisfies symmetry % ($\bidistance\fun{x, y} = \bidistance\fun{y, x}$)
and the triangle inequality. %($\bidistance\fun{x, y} + \bidistance\fun{y, z} \geq \bidistance\fun{x, z}$)
%but not necessarily the identity of indiscernibles.
%, meaning that a zero distance does not imply that elements are the same ($\bidistance\fun{x, y} = 0 \centernot\iff x = y$).
%In the context of bisimulation pseudometrics, the zero distance characterizes the probabilistic bisimulation, i.e., $\bidistance\fun{x, y} \iff x \sim y$.

Probabilistic bisimilarity can be characterized by a logical family of functional expressions %\citep{DBLP:journals/tcs/DesharnaisGJP04}
derived from a logic $\logic$.
More specifically, given a policy $\policy \in \mpolicies{\mdp}$, we consider a family $\functionalexpr\fun{\policy}$ of real-valued functions $f$, parameterized by the discount factor $\discount$ and defining the semantics of $\logic$ in $\mdp_\policy$.
%Such a logic allows formalizing discounted properties, including reachability (e.g., \citealt{DBLP:conf/fsttcs/ChatterjeeAMR08}).
The related pseudometric $\bidistance_{\policy}$ is defined as: $\bidistance_\policy\fun{\state_1, \state_2} = \sup_{f \in \functionalexpr\fun{\policy}} \left| f\fun{\state_1} - f\fun{\state_2} \right|$, for all $\state_1,\state_2 \in \states$.
\iffalse
\begin{align*}
    && \bidistance_\policy\fun{\state_1, \state_2} =& \sup_{f \in \functionalexpr\fun{\policy}} \left| f\fun{\state_1} - f\fun{\state_2} \right|, & \forall \state_1, \state_2 \in \states.
\end{align*}
\fi
We distinguish between pseudometrics $\bidistance^{\rewards}_\policy$, characterized by functional expressions including rewards,
%(e.g., \citealt{DBLP:conf/birthday/FernsPK14}), 
and $\bidistance^{\labels}_\policy$, whose functional expressions are based on state labels.
%(e.g., \citealt{DBLP:conf/fossacs/ChenBW12}).
Let $\tilde{P}$ be the space of pseudometrics on $\states$ and $\varphi \in \set{\rewards, \labels}$.
Define $\Delta\colon \tilde{P} \to \tilde{P}$ so that $\Delta\fun{\distance^{\varphi}_\policy}\fun{\state_1, \state_2}$ is $\fun{1 - \discount} \left| \rewards_\policy\fun{\state_1} - \rewards_\policy\fun{\state_2} \right| \cdot \condition{\set{\rewards}}\fun{\varphi} + M$ where:
\[
M = \max \begin{cases}
\discount
    \wassersteindist{\distance_{\policy}^{\varphi}}{\probtransitions_\policy\fun{\sampledot
  \mid \state_1}}{\probtransitions_\policy\fun{\sampledot \mid \state_2}},\\
  \condition{\neq}\fun{\labels\fun{\state_1},
  \labels\fun{\state_2}} \cdot \condition{\set{\labels}}\fun{\varphi},
\end{cases}
\]
\iffalse
\begin{align*}
    \Delta\fun{\distance^{\varphi}_\policy}\fun{\state_1, \state_2} =& \fun{1 - \discount} \left| \rewards_\policy\fun{\state_1} - \rewards_\policy\fun{\state_2} \right| \cdot \condition{\set{\rewards}}\fun{\varphi} \\
    &+ \max \{ \discount
    \wassersteindist{\distance_{\policy}^{\varphi}}{\probtransitions_\policy\fun{\sampledot
  \mid \state_1}}{\probtransitions_\policy\fun{\sampledot \mid \state_2}},\\
    &\phantom{+ \max \{\} }\condition{\neq}\fun{\labels\fun{\state_1},
  \labels\fun{\state_2}} \cdot \condition{\set{\labels}}\fun{\varphi}\}
\end{align*}
\fi
then $\bidistance^{\varphi}_\policy$ is its unique fixed point whose kernel is $\sim_{\{\varphi\}}$, i.e., $\bidistance^{\varphi}_{\latentpolicy}(\state_1, \state_2) = 0$ iff
$\state_1 \!\! \sim_{\{\varphi\}} \! \! \state_2$
%$\state_1~\sim_{\{\varphi\}}~\state_2$
\citep{DBLP:conf/icalp/BreugelW01,DBLP:conf/birthday/FernsPK14},
% When considering rewards, \citet{DBLP:conf/uai/FernsPP05} showed that
% $ | \values{\policy}{}{\state_1} - \values{\policy}{}{\state_2} | \leq \nicefrac{\bidistance^{\rewards}_{\policy}\fun{\state_1, \state_2}}{1 - \discount}.
% $
and
% \begin{equation*}
%     \left| \values{\policy}{}{\state_1} - \values{\policy}{}{\state_2} \right| \leq \frac{\bidistance^{\rewards}_{\policy}\fun{\state_1, \state_2}}{1 - \discount}. \label{eq:reward-bisimulation}
% \end{equation*}
$ | \values{\policy}{}{\state_1} - \values{\policy}{}{\state_2} | \leq \nicefrac{\bidistance^{\rewards}_{\policy}\fun{\state_1, \state_2}}{1 - \discount}
$ \cite{DBLP:conf/uai/FernsPP05}.


%based on the modal logic of \cite{DBLP:conf/popl/LarsenS89}.
% More specifically, given a policy $\policy \in \mpolicies{\mdp}$, we consider a family $\functionalexpr\fun{\policy}$ of real-valued functions $f \colon \states \to [0, 1]$ which define the semantic of $\logic$ in $\mdp_\policy$, parameterized by the discount factor $\discount$.
% Such a logic allows formalizing discounted properties, including reachability.
% For any pair of states $\state_1, \state_2 \in \states$ and policy $\policy \in \mpolicies{\mdp}$, the related pseudometric $\logicbidistance_{\policy} \colon \states \times \states \to \mathopen[0, 1\mathclose]$ is defined as
% \[
%     \logicbidistance_\policy\fun{\state_1, \state_2} = \sup_{f \in \functionalexpr\fun{\policy}} \left| % f\fun{\state_1} - f\fun{\state_2} \right|.
% \]
% When focusing on discounted return values involving general measurable reward function $\rewards$, we further consider the pseudometric $\bidistance_\policy \colon \states \times \states \to \R$ introduced by \cite{DBLP:journals/siamcomp/FernsPP11}, with a characterization based on the value difference: % for any pair of states $\state_1, \state_2 \in \states$ and policy $\policy \in \mpolicies{\mdp}$,
% \[
%     \left| \values{\policy}{}{\state_1} - \values{\policy}{}{\state_2} \right| \leq \frac{\bidistance_{\policy}\fun{\state_1, \state_2}}{1 - \discount}.
% \]
%
% In this work, we distinguish two bisimulation pseudometrics.
% First, we consider the pseudometric $\bidistance \colon \states \times \states \to \R$ introduced by \cite{DBLP:conf/uai/FernsPP05}, with a characterization based on the discounted return value difference: for any pair of states $\state_1, \state_2 \in \states$ and policy $\policy \in \mpolicies{\mdp}$,
% \[
% \left| \values{\policy}{}{\state_1} - \values{\policy}{}{\state_2} \right| \leq \frac{\bidistance_{\policy}\fun{\state_1, \state_2}}{1 - \discount}.
% \]
% Second, we consider the logical characterization introduced by \cite{DBLP:journals/tcs/DesharnaisGJP04}, based on a family of functional expressions derived from the modal logic $\logic$ of \cite{DBLP:conf/popl/LarsenS89}.
% More specifically, given a policy $\policy \in \mpolicies{\mdp}$, we consider a family $\functionalexpr\fun{\policy}$ of real-valued functions $f \colon \states \to [0, 1]$ which define the semantic of $\logic$ in $\mdp_\policy$, parameterized by the discount factor $\discount$.
% Such a logic allows formalizing discounted properties, including reachability (e.g., \citealt{DBLP:conf/fsttcs/ChatterjeeAMR08}).
%  the related pseudometric $\logicbidistance_{\policy} \colon \states \times \states \to \mathopen[0, 1\mathclose]$ is defined as
% \[
%     \logicbidistance_\policy\fun{\state_1, \state_2} = \sup_{f \in \functionalexpr\fun{\policy}} \left| f\fun{\state_1} - f\fun{\state_2} \right|.
% \]
% for any pair of states $\state_1, \state_2 \in \states$ and policy $\policy \in \mpolicies{\mdp}$.
%usually expressed with the notion of trajectory, execution trace or value equality.

%connect bisimulation metrics with latent space models by showing 
%We now show %that 
\smallparagraph{Bisimulation distance bounds.}~We state that
the expected bisimulation distance between states and their latent abstraction is bounded by local losses.
%
%Let $\latentpolicy \in \latentmpolicies$, assume $\latentmdp$ is discrete and $\langle\KR{\latentpolicy}, \KP{\latentpolicy}\rangle$-Lipschitz.
%Let $\varphi = \set{\rewards, \labels}$, then given the induced stationary distribution $\stationary{\latentpolicy}$ in $\mdp$, let
Fix
$\latentpolicy \in \latentmpolicies$ and assume $\latentmdp$ is discrete and $\langle\KR{\latentpolicy}, \KP{\latentpolicy}\rangle$-Lipschitz.
%then
Given the induced stationary distribution $\stationary{\latentpolicy}$ in $\mdp$,
\begin{align}
    % \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}} \leq  \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \localtransitionloss{\stationary{\latentpolicy}} \frac{\fun{\KR{\latentpolicy} \cdot  \condition{\set{\rewards}}\fun{\varphi} + \discount \cdot \condition{\set{\labels}}\fun{\varphi}}}{1 - \discount \fun{\KP{\latentpolicy}\condition{\set{\rewards}}\fun{\varphi} + \condition{\set{\labels}}\fun{\varphi}}}.
    \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\rewards}_{\latentpolicy}\fun{\state, \embed\fun{\state}} & \leq  \localrewardloss{\stationary{\latentpolicy}} + \discount \localtransitionloss{\stationary{\latentpolicy}} \frac{\KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}, \notag \\
    \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\labels}_{\latentpolicy}\fun{\state, \embed\fun{\state}} & \leq \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount}. \label{eq:bidistance-bound}
\end{align}
%
The result provides us a general way to asses the quality of our latent
abstraction: the bisimulation distance between states and their embedding is
guaranteed to be small in average whenever local losses are small.
% Notice that bounds of Lemma~\ref{lemma:qvalues-diff-bound} and Lemma~\ref{lemma:bidistance-embedding} are further the same (modulo the discount scaling of Eq.~\ref{eq:reward-bisimulation}).
% This justifies the choice of using local losses to evaluate the quality of the latent model as an abstraction of $\mdp$.
% In addition, it also means that this bound on the expected bisimulation distance can be checked from samples using Theorem~\ref{thm:pac-qvaluedif}.
%
% We additionally provide abstraction quality bounds in terms of bisimulation metrics.
% This allows formalizing the quality of the latent space model as an abstraction of $\mdp$ as follows.
%
%We further formalize the quality of the abstraction by showing that the bisimulation distance between states with same representation can be upper-bounded by local losses:
%
This allows us formalizing the quality of the abstraction by bounding the bisimulation distance between states with same representation by local losses:
%
%\begin{lemma}\label{lemma:bidistance-abstraction-quality}
% Let $\latentpolicy \in \latentmpolicies$, assume $\latentmdp$ is discrete and $\langle\KR{\latentpolicy}, \KP{\latentpolicy}\rangle$-Lipschitz.
% Let $\varphi = \set{\rewards, \labels}$ and $\stationary{\latentpolicy}$ be the stationary distribution of $\mdp$ induced by $\latentpolicy$.
%for any pair of states $\state_1, \state_2 \in \states$ such that $\embed\fun{\state_1} = \embed\fun{\state_2}$,
for any states $\state_1, \state_2 \in \states$ with $\embed\fun{\state_1} = \embed\fun{\state_2}$,
\begin{align}
    \bidistance^{\rewards}_{\latentpolicy}\fun{\state_1, \state_2} \leq& \left[\localrewardloss{\stationary{\latentpolicy}} + \frac{
    \discount \localtransitionloss{\stationary{\latentpolicy}} \KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}\right] \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} + \stationary{\latentpolicy}^{-1}\fun{\state_2}}, \notag \\
    \bidistance^{\labels}_{\latentpolicy}\fun{\state_1, \state_2} \leq&  \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount} \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} + \stationary{\latentpolicy}^{-1}\fun{\state_2}}. \label{eq:bidistance-abstraction-quality}
\end{align}
%\end{lemma}


\smallparagraph{Value difference bounds.}~%
Considering discounted returns or a specific event, the quality of the latent abstraction induced by $\embed$ and $\embeda$ can be in particular formalized by means of \emph{value difference bounds}.
%as demonstrated by the theoretical bounds from \cite{DBLP:conf/icml/GeladaKBNB19}.
% Given any policy in $\latentmpolicies$, such bounds link the values of the original MDP $\mdp$ and those of its latent abstraction $\latentmdp$.
% In the following, we show that we can check them to any degree of accuracy with high probability by means of simulations.
%We adapt these bounds \cite{DBLP:conf/icml/GeladaKBNB19} in the discrete setting for discounted return, and we derive new ones in the case of discounted reachability.
These bounds can be intuitively derived by taking the value function as a
real-valued function from $\functionalexpr\fun{\policy}$.
% \begin{lemma}\label{lemma:qvalues-diff-bound}
Let $\labelset{C}, \labelset{T} \subseteq \atomicprops$, $\varphi \in \set{\until{\labelset{C}}{\labelset{T}}, \eventually \labelset{T}}$ and $\KV = \min\fun{\nicefrac{\Rmax{\latentpolicy}}{1 - \discount}, \nicefrac{\KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}}$,
then, %given the induced stationary distribution $\stationary{\latentpolicy}$ in $\mdp$,
\begin{align}
    \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{}{\embed\fun{\state}}{\latentaction} \right| & \leq \frac{\localrewardloss{\stationary{\latentpolicy}} + \discount \KV \localtransitionloss{\stationary{\latentpolicy}}}{1 - \gamma}, \notag \\ %\tag{\citealt{DBLP:conf/icml/GeladaKBNB19}} \\
    \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| & \leq \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount}. \label{eq:value-dif-bound}
\end{align}
% \end{lemma}
%
% \begin{lemma}\label{lem:quality-latent-space}
    % Let $\latentpolicy \in \latentmpolicies$ and assume $\latentmdp$ is discrete and $\langle \KR{\latentpolicy}, \KP{\latentpolicy} \rangle$-Lipschitz.
    % Let $\labelset{C}, \labelset{T} \subseteq \atomicprops$, $\varphi = \set{\until{\labelset{C}}{\labelset{T}}, \eventually \labelset{T}}$, $\KV = \min\fun{\nicefrac{\Rmax{\latentpolicy}}{1 - \discount}, \nicefrac{\KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}}$, and $\stationary{\latentpolicy}$ be the induced stationary distribution in $\mdp$.
    Moreover, for any states $\state_1, \state_2 \in \states$ with $\embed\fun{\state_1} = \embed\fun{\state_2}$,
    \begin{align}
      &\left| \values{\latentpolicy}{}{\state_1} {-}
      \values{\latentpolicy}{}{\state_2} \right| \leq
      \frac{\localrewardloss{\stationary{\latentpolicy}} {+} \discount \KV
      \localtransitionloss{\stationary{\stationary{\latentpolicy}}}}{1 {-}
      \discount} \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} {+}
      \stationary{\latentpolicy}^{-1}\fun{\state_2}}, \notag\\
      %
      &\left| \values{\latentpolicy}{\varphi}{\state_1} {-}
      \values{\latentpolicy}{\varphi}{\state_2} \right| \leq \frac{\discount
      \localtransitionloss{\stationary{\latentpolicy}}}{1 {-} \discount}
      \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} {+}
      \stationary{\latentpolicy}^{-1}\fun{\state_2}}. \label{eq:value-diff-abstraction-quality}
    \end{align}
% \end{lemma}
%
Intuitively, when local losses are sufficiently small, then (i) the expected value difference of states and their embeddings that are likely to be seen under a latent policy is also small, and (ii) states with the same embedding have close values. 

\subsection{Checking the Quality of the Abstraction}
While bounding the difference between values offered by $\latentpolicy \in \latentmpolicies$ in $\mdp$ and $\latentmdp$ is theoretically possible using $\localrewardloss{\stationary{\latentpolicy}}$ and $\localtransitionloss{\stationary{\latentpolicy}}$, we need to accurately approximate these losses from samples to further offer practical guarantees (recall that $\mdp$ is unknown).
%
Although the agent is able to produce execution traces by
interacting with $\mdp$,
%In a BSCC of $\mdp_{\latentpolicy}$, this means the agent produces $\state, \latentaction \sim \stationary{\latentpolicy}$ at each step in the limit,
%as well as a reward $\reward$ resulting from the transition to the next state.
%================================================================
%Two issues arise: First, the reward obtained does not necessarily come from a function defined over state-action pairs.
%Second,
%================================================================
estimating the expectation over the Wasserstein is intractable.
Intuitively, even if approximating Wasserstein from samples is possible (e.g., \citealp{DBLP:conf/aistats/GenevayCBCP19}), 
this would require access to a generative model for $\probtransitions\fun{\sampledot \mid \state, \action}$ (e.g., \citealp{DBLP:journals/ml/KearnsMN02}) from which we would have to draw a sufficient number of samples for each $\state, \action$ drawn from $\stationary{\latentpolicy}$ to then be able to estimate the expectation. %of $\localtransitionloss{\stationary{\latentpolicy}}$.
\citet{DBLP:conf/icml/GeladaKBNB19} overcome this issue by assuming a deterministic MDP%
% (i.e., $\probtransitions({\sampledot \mid \state, \action})$ is Dirac)
, which allows optimizing an approximation of $\localtransitionloss{\stationary{\latentpolicy}}$ through gradient descent.
%
To deal with general MDPs, we study
%lower and
an upper bound on $\localtransitionloss{\stationary{\latentpolicy}}$ that can be efficiently approximated from samples:
%\begin{lemma}\label{lemma:local-loss-upper-bounds}
%Let $\stationary{\latentpolicy}$ be a stationary distribution of $\mdp$ under $\latentpolicy \in \latentmpolicies$, then
\begin{align*}
    %&\localrewardloss{\stationary{\latentpolicy}} \leq \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}\left| \rewards\fun{\state, \latentaction, \state'} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right| = \localrewardlossupper{\stationary{\latentpolicy}}, \\ %\label{eq:rewardloss-upperbound} \\
    %\wassersteindist{\distance_{\latentstates}}{\embed\stationary{\latentpolicy}}{\latentprobtransitions_{\embed}\stationary{\latentpolicy}} \leq \,
    &\localtransitionloss{\stationary{\latentpolicy}} \leq \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}} \wassersteindist{\distance_{\latentstates}}{\embed\fun{\sampledot \mid \state'}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} = \localtransitionlossupper{\stationary{\latentpolicy}}, \label{eq:transitionloss-bounds}
\end{align*}
where $\stationary{\latentpolicy}(\state, \latentaction, \state')=  \stationary{\latentpolicy}(\state, \latentaction) \cdot \probtransitions(\state' \mid \state, \latentaction)$
and $\embed(\latentstate \mid \state) = \condition{=}(\embed\fun{\state}, \latentstate)$. %$\embed\stationary{\latentpolicy}\fun{\latentstate} = \expectedsymbol{\state \sim \stationary{\latentpolicy}}{\embed\fun{\latentstate \mid \state}}$, and
% $\latentprobtransitions_\embed\steadystate{\policy}\fun{\latentstate} = \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}{\latentprobtransitions\fun{\latentstate \mid \embed\fun{\state}, \latentaction}}$.
%\end{lemma}
%
We now provide \emph{probably approximately correct} (PAC) guarantees for estimating local losses for discrete latent models, derived from 
%the Hoeffding's inequalities \citep{10.2307/2282952:hoeffding}.
the \citeauthor{10.2307/2282952:hoeffding}'s inequalities. %(\citeyear{10.2307/2282952:hoeffding}).
%
\begin{lemma}\label{lemma:pac-loss}
Suppose $\latentmdp$ is discrete and the agent interacts with $\mdp$ by executing $\latentpolicy \in \latentpolicies$, thus producing $ \tuple{\seq{\state}{T}, \seq{\latentaction}{T - 1}, \seq{\reward}{T - 1}} \sim \stationary{\latentpolicy}$.
Let $\error, \proberror \in \mathopen]0, 1\mathclose[$ and denote by
\begin{align*}
    \localrewardlossapprox{\stationary{\latentpolicy}} &= \frac{1}{T} \sum_{t = 0}^{T - 1} \left| \reward_t - \latentrewards\fun{\embed\fun{\state_t}, \latentaction_t}  \right|, \\
    % \localtransitionlossapprox{\stationary{\latentpolicy}} &= \frac{1}{2T} \sum_{t = 0}^{T - 1} \sum_{\latentstate' \in \latentstates} \left| \embed\fun{\latentstate' \mid \state_{t + 1}} - \latentprobtransitions\fun{\latentstate' \mid \embed\fun{\state_t}, \latentaction_t} \right|.
    \localtransitionlossapprox{\stationary{\latentpolicy}} &= \frac{1}{T} \sum_{t = 0}^{T - 1} \left[ 1 - \latentprobtransitions\fun{\embed\fun{\state_{t + 1}} \mid \embed\fun{\state_t}, \latentaction_t} \right].
\end{align*}
Then after $T \geq \left\lceil \nicefrac{- \log\fun{\frac{\proberror}{4}}}{2
  \error^2} \right\rceil$ steps,
    %$\left| \localrewardlossupper{\stationary{\latentpolicy}} -
    $\left| \localrewardloss{\stationary{\latentpolicy}} -
    \localrewardlossapprox{\stationary{\latentpolicy}}  \right| \leq \error$,
    $\left| \localtransitionlossupper{\stationary{\latentpolicy}} -
    \localtransitionlossapprox{\stationary{\latentpolicy}} \right| \leq
    \error$
with probability at least $1 - \proberror$.
\end{lemma}
%
%
%As a direct consequence of Lem.~\ref{lemma:local-loss-upper-bounds} and Lem.~\ref{lemma:pac-loss}, 
%$\localrewardloss{\stationary{\latentpolicy}} \leq \localrewardlossapprox{\stationary{\latentpolicy}} + \error$  and
%$\localtransitionloss{\stationary{\latentpolicy}} \leq \localtransitionlossapprox{\stationary{\latentpolicy}} + \error$ with probability at least $1 - \proberror$ when a sufficient number of simulation steps has been performed.
%The conjunction of Lemma~\ref{lemma:qvalues-diff-bound} and Lemma~\ref{lemma:pac-loss}
This yields the following Theorem, finally allowing to check the  abstraction quality as a bounded value difference.
\begin{theorem}\label{thm:pac-qvaluedif}
    Let $\latentpolicy \in \latentmpolicies$ and assume $\latentmdp$ is discrete and $\langle \KR{\latentpolicy}, \KP{\latentpolicy} \rangle$-Lipschitz.
    Let $\labelset{C}, \labelset{T} \subseteq \atomicprops$, $\varphi \in \set{\until{\labelset{C}}{\labelset{T}}, \eventually \labelset{T}}$ and $\KV = \min\fun{\nicefrac{\Rmax{\latentpolicy}}{1 - \discount}, \nicefrac{\KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}}$.
    Let $\error, \proberror \in \mathopen]0, 1\mathclose[$ and $\stationary{\latentpolicy}$ be the stationary distribution of $\mdp_{\latentpolicy}$.
    %Assume the agent executes $\latentpolicy$ in $\mdp$, then
    Then, after $T \geq \left\lceil \nicefrac{- \log\fun{\frac{\proberror}{4}} \fun{1 +
    \discount \KV}^2}{2\error^2\fun{1 - \discount}^2}\right\rceil$ interaction steps through $\stationary{\latentpolicy}$,
    \begin{align*}
        \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}
        \left| \qvalues{\latentpolicy}{}{\state}{\latentaction} -
        \latentqvalues{\latentpolicy}{}{\embed\fun{\state}}{\latentaction}
        \right| & \leq
        \frac{\localrewardlossapprox{\stationary{\latentpolicy}} + \discount
        \KV \localtransitionlossapprox{\stationary{\latentpolicy}}}{1 -
      \gamma} + \error, \\
        \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| & \leq \frac{\discount \localtransitionlossapprox{\stationary{\latentpolicy}}}{1 - \discount} + \frac{\discount \error}{1 + \discount \KV}
    \end{align*}
    with probability at least $1 - \proberror$.
\end{theorem}
%


==> hyperparameters.tex <==
\begin{tabular}{llllll}
\toprule
{} &           CartPole &        MountainCar &            Acrobot &           Pendulum &        LunarLander \\
\midrule
activation                                             &  leaky relu &  leaky relu &  relu &  relu &  relu \\
learning rate                                          & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & $10^{-4}$ & $10^{-4}$ \\
RL policy                                              &  DQN &  DQN &  DQN (robust) &  SAC (robust) &  SAC \\
$\log_2 \left | \latentstates \right|$                 &  9 &  10 &  13 &  13 &  16 \\
$\left| \latentactions \right|$                        &  / &  / &  / &  3 &  5 \\
$\temperature_{1}^{\scriptscriptstyle \latentstates}$  & $\nicefrac{2}{3}$ & $\nicefrac{2}{3}$ & $\nicefrac{2}{3}$ & $\nicefrac{2}{3}$ & $\nicefrac{2}{3}$ \\
$\temperature_{2}^{\scriptscriptstyle \latentstates}$  & $\nicefrac{1}{2}$ & $\nicefrac{1}{2}$ & $\nicefrac{1}{2}$ & $\nicefrac{1}{2}$ & $\nicefrac{1}{2}$ \\
$\temperature_{1}^{\scriptscriptstyle \latentactions}$ &  / &  / &  / & $\nicefrac{1}{2}$ & $\nicefrac{1}{4}$ \\
$\temperature_{2}^{\scriptscriptstyle \latentactions}$ &  / &  / &  / & $\nicefrac{1}{3}$ & $\nicefrac{1}{6}$ \\
$\tau_{\temperature_{1}}$                              & $10^{-6}$ & $10^{-6}$ & $10^{-6}$ & $10^{-6}$ & $10^{-6}$ \\
$\tau_{\temperature_{2}}$                              & $2\cdot 10^{-6}$ & $2\cdot 10^{-6}$ & $2\cdot 10^{-6}$ & $2\cdot 10^{-6}$ & $2\cdot 10^{-6}$ \\
$\alpha$                                               & $10^{1}$ & $10^{1}$ & $10^{1}$ & $10^{1}$ & $10^{1}$ \\
$\alpha_{\scriptscriptstyle \actions}$                                             &  / &  / &  / & $1$ & $10^{-1}$ \\
$\tau_{\alpha}$                                        & $10^{-5}$ & $10^{-5}$ & $7.5\cdot 10^{-5}$ & $7.5\cdot 10^{-5}$ & $10^{-5}$ \\
$\tau_{\beta}$                                         & $5\cdot 10^{-5}$ & $5\cdot 10^{-5}$ & $7.5\cdot 10^{-5}$ & $7.5\cdot 10^{-5}$ & $5\cdot 10^{-5}$ \\
prioritized experience replay                          &  bucket &  bucket &  bucket &  loss &  loss \\
$\varsigma$                                      & $\nicefrac{1}{3}$ & $\nicefrac{1}{3}$ & $3\cdot 10^{-1}$ & $3\cdot 10^{-1}$ & $3\cdot 10^{-1}$ \\
$\tau_{\omega}$                                        & $7\cdot 10^{-5}$ & $7.5\cdot 10^{-5}$ & $7\cdot 10^{-5}$ & $10^{-5}$ & $10^{-5}$ \\
$\varepsilon$                                          & $0$ & $0$ & $\nicefrac{1}{2}$ & $\nicefrac{1}{2}$ & $0$ \\
$\tau_{\varepsilon}$                                   &  / &  / & $10^{-5}$ & $10^{-5}$ &  / \\
\bottomrule
\end{tabular}


==> key_papers.tex <==
\begin{itemize}
    \item \textbf{Variational Autoencoders (VAEs)}: \cite{DBLP:journals/corr/KingmaW13,DBLP:conf/icml/RezendeMW14}.
    \item \textbf{Discrete latent representations}:
        \begin{itemize}
            \item \textit{Concrete distributions and Gumble-softmax trick:} \cite{DBLP:conf/iclr/JangGP17, DBLP:conf/iclr/MaddisonMT17}.
            \item via vectorization of the latent space, \cite{DBLP:conf/nips/OordVK17}; and clustering, \cite{DBLP:conf/ijcai/JiangZTTZ17}.
        \end{itemize}
    \item \textbf{Learn abstract latent states of an unknown MDP}:
        \begin{itemize}
            \item Learn discrete states via GANs for planning purposes: \cite{DBLP:conf/nips/KurutachTYRA18}.
            \item Learn continuous abstract states for reinforcement learning: \cite{DBLP:conf/nips/FreemanHM19}.
            \item Learn discrete states via VAEs and finite sequences of observations for planning purposes (prioritized sweeping): \cite{DBLP:conf/icml/CorneilGB18}.
        \end{itemize}
    \item \textbf{Deep reinforcement learning with continuous states and actions via stochastic policies}: REINFORCE, \cite{DBLP:books/lib/SuttonB98}; soft actor-critic \cite{DBLP:conf/icml/HaarnojaZAL18}.
    \item \textbf{The posterior collapse problem}:
    \begin{itemize}
        \item Analysis of the posterior collapse problem, \cite{DBLP:conf/icml/AlemiPFDS018, DBLP:conf/iclr/LucasTGN19}.
        \item Cross-entropy regularization, \cite{DBLP:conf/corl/BurkeHR19, DBLP:journals/corr/abs-1910-09588}.
    \end{itemize}
    
\end{itemize}

==> labels.tex <==
\begin{table}
\centering
\small
\begin{tabular}{l|l|l|l|l}
\hline
Environment &
  $\states \subseteq$ &
  Description, for $\vect{\state} \in \states$ &
  Labeling function $\labels\fun{\vect{\state}}$ &
  $\atomicprops = \set{p_1, \dots, p_n}$ \\ \hline
CartPole &
  $\R^4$ &
  \begin{tabular}[c]{@{}l@{}}\tabitem $\vect{\state}_1$: cart position\\ \tabitem $\vect{\state}_2$: cart velocity\\ \tabitem $\vect{\state}_3$: pole angle (rad)\\ \tabitem $\vect{\state}_4$: pole velocity at tip\end{tabular} &
  $\begin{aligned}\langle &\condition{<}\fun{\vect{\state}_1, 1.5},\\& \condition{<}\fun{\vect{\state}_3, 0.15} \rangle \end{aligned}$ &
  \begin{tabular}[c]{@{}l@{}}\tabitem $p_1$: safe cart position\\ \tabitem $p_2$: safe pole angle\end{tabular} \\ \hline
MountainCar &
  $\R^2$ &
  \begin{tabular}[c]{@{}l@{}}\tabitem $\vect{\state}_1$: position\\ \tabitem $\vect{\state}_2$: velocity\end{tabular} &
  $\begin{aligned}\langle &\condition{\geq}\fun{\vect{\state}_1, \nicefrac{1}{2}}, \\ & \condition{\geq}\fun{\vect{\state}_1, \nicefrac{-1}{2}}, \\ & \condition{\geq}\fun{\vect{\state}_2, 0}\rangle \end{aligned}$ &
  \begin{tabular}[c]{@{}l@{}}\tabitem $p_1$: target position\\ \tabitem $p_2$: right-hand side of the mountain\\ \tabitem $p_3$: car going forward\end{tabular} \\ \hline
Acrobot &
  $\R^6$ &
  \begin{tabular}[c]{@{}l@{}}Let $\theta_1, \theta_2 \in \mathopen[0, 2\pi \mathclose]$ be the angles\\ of the two rotational joints,\\ \tabitem $\vect{\state}_1 = \cos\fun{\theta_1}$\\ \tabitem $\vect{\state}_2 = \sin\fun{\theta_1}$\\ \tabitem $\vect{\state}_3 = \cos\fun{\theta_2}$\\ \tabitem $\vect{\state}_4 = \sin\fun{\theta_2}$\\ \tabitem $\vect{\state}_5$: angular velocity 1\\ \tabitem $\vect{\state}_6$: angular velocity 2\end{tabular} &
  $\begin{aligned}\langle &\condition{>}\fun{-\vect{\state}_1 -\vect{\state}_3 \cdot \vect{\state}_1 + \vect{\state}_4 \cdot \vect{\state}_2, 1}, \\ & \condition{\geq}\fun{\vect{\state}_1, 0}, \\ & \condition{\geq}\fun{\vect{\state}_2, 0} \\ & \condition{\geq}\fun{\vect{\state}_3, 0} \\ & \condition{\geq}\fun{\vect{\state}_4, 0}\\ & \condition{\geq}\fun{\vect{\state}_5, 0}\\ & \condition{\geq}\fun{\vect{\state}_6, 0}\rangle \end{aligned}$ &
  \begin{tabular}[c]{@{}l@{}}\tabitem $p_1$: RL agent target \\\tabitem $p_2$: $\theta_1 \in [0, \nicefrac{\pi}{2}] \cup [\nicefrac{3\pi}{2}, 2\pi]$ \\
  \tabitem $p_3$: $\theta_1 \in [0, \pi]$\\
  \tabitem $p_4$: $\theta_2 \in [0, \nicefrac{\pi}{2}] \cup [\nicefrac{3\pi}{2}, 2\pi]$\\
  \tabitem $p_5$: $\theta_2 \in [0, \pi]$\\
  \tabitem $p_6$: positive angular velocity (1)\\
  \tabitem $p_7$: positive angular velocity (2)\\
  \end{tabular} \\\hline
Pendulum &
  $\R^3$ &
  \begin{tabular}[c]{@{}l@{}}Let $\theta \in \mathopen[0, 2\pi \mathclose]$ be the joint angle\\ \tabitem $\vect{\state}_1 = \cos\fun{\theta}$\\ \tabitem $\vect{\state}_2 = \sin\fun{\theta}$\\ \tabitem $\vect{\state}_3$: angular velocity\end{tabular} &
  $\begin{aligned}\langle &\condition{\geq}\fun{\vect{\state}_1, \cos\fun{\nicefrac{\pi}{3}}}, \\ & \condition{\geq}\fun{\vect{\state}_1, 0}, \\ & \condition{\geq}\fun{\vect{\state}_2, 0} \\ & \condition{\geq}\fun{\vect{\state}_3, 0} \rangle \end{aligned}$ &
    \begin{tabular}[c]{@{}l@{}}
    \tabitem $p_1$: safe joint angle \\
    \tabitem $p_2$: $\theta \in [0, \nicefrac{\pi}{2}] \cup [\nicefrac{3\pi}{2}, 2\pi]$ \\
  \tabitem $p_3$: $\theta \in [0, \pi]$\\
  \tabitem $p_4$: positive angular velocity\\
  \end{tabular} \\\hline
LunarLander &
  $\R^8$ &
  \begin{tabular}[c]{@{}l@{}}\tabitem $\vect{\state}_1$: horizontal coordinates\\ \tabitem $\vect{\state}_2$: vertical coordinates\\ \tabitem $\vect{\state}_3$: horizontal speed\\ \tabitem $\vect{\state}_4$: vertical speed\\ \tabitem $\vect{\state}_5$: ship angle\\ \tabitem $\vect{\state}_6$: angular speed\\ \tabitem $\vect{\state}_7$: left leg contact\\ \tabitem $\vect{\state}_8$: right leg contact\end{tabular} &
  based on the heuristic function &
  \begin{tabular}[c]{@{}l@{}}
  \tabitem $p_1$: unsafe angle\\
  \tabitem $p_2$: leg ground contact\\
  \tabitem $p_3$: lands too rapidly\\
  \tabitem $p_4$: left inclination\\
  \tabitem $p_5$: right inclination\\
  \tabitem $p_6$: motors shut down
  \end{tabular}
\end{tabular}
\caption{Labeling functions used in our experiments.
We provide a short description of the state space and the meaning of the atomic propositions forming the labels.
Recall that labels and $\atomicprops$ are respectively binary and one-hot encoded.
Let $n = |\atomicprops|$ with $\atomicprops = \set{p_1, \dots, p_n}$, we write $p_{i}$ for the one-hot vector of size $n$ with the $i^{\text{th}}$ entry set to $1$, with $i \in [n] \setminus \set{0}$.
The LunarLander labeling function is based on the heuristic function of the OpenAI's implementation \citep{DBLP:journals/corr/BrockmanCPSSTZ16}.}
\label{appendix:table:labels}
\end{table}

==> new_vae.tex <==
We now provide a framework based on \emph{variational autoencoders} \citep{DBLP:journals/corr/KingmaW13} that allows us to learn a discrete latent space model of $\mdp$ through the interaction of the agent executing a pre-learned RL policy $\policy \in \mpolicies{\mdp}$ with the environment.
Concretely, we seek a discrete latent space model $\tuple{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}}$ such that $ \latentmdp_{\decoderparameter} = \tuple{\latentstates, \latentactions, \latentprobtransitions_{\decoderparameter}, \latentrewards_{\decoderparameter}, \latentlabels_{\decoderparameter}, \atomicprops, \zinit}$.
We propose to learn the parameters $\tuple{\encoderparameter, \decoderparameter}$ of an \emph{encoder} $\encoder$ and a \emph{behavioral model} $\decoder$ from which we can retrieve
(i) the embedding functions
$\embed_{\encoderparameter}$ and $\embeda_{\encoderparameter, \decoderparameter}$,
(ii) the latent MDP components $\latentprobtransitions_{\decoderparameter}$, $\latentrewards_{\decoderparameter}$, and $\latentlabels_{\decoderparameter}$,
and (iii) a latent policy $\latentpolicy_\decoderparameter \in \latentmpolicies$, via
$
    \min_{\decoderparameter} \divergence{\mdp_\policy}{\decoder},
$
where $\divergencesymbol$ is a discrepancy measure.
Intuitively, the end goal is to learn
(i) a discrete representation of $\states$ and $\actions$
(ii) to mimic the behaviors of the original MDP over the induced latent spaces, thus yielding a latent MDP with a bisimulation distance close to $\mdp$, and
(iii) to \emph{distill} $\policy$ into $\latentpolicy_{\decoderparameter}$. %\todo{Removed the sentence about compressing, it gives the wrong intuition I feel (it is actually an abstraction)}
%, i.e., to \emph{compress} $\policy$ over these latent spaces.
In the following, we distinguish the case where we only learn $\latentstates$, with $\latentactions = \actions$ (in that case, $\actions$ is assumed to be discrete), and the one where we additionally need to discretize the set of actions and learn $\latentactions$.

\subsection{Evidence Lower Bound}
In this work, we focus on the case where $\dklsymbol$ is used as discrepancy measure: the goal is optimizing $\min_{\decoderparameter}
\dklsymbol(\mdp_{\policy} \parallel \decoder)$ or equivalently maximizing the marginal
% \emph{log-likelihood of traces} of the original MDP, given by 
% $\expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}}$ such that:
\emph{log-likelihood of traces} of $\mdp$, i.e.,
$\expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}}$, where
% \begin{equation}
%     \expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}} 
%     \text{ s.t. }
%     \decoder\fun{\trace} =
%         \begin{cases}
%             \int_{\inftrajectories{\latentmdp_{\decoderparameter}}} \decoder\fun{\trace \mid \seq{\latentstate}{T}} \, d\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentstate}{T}} & \text{if } \latentactions = \actions, \\ 
%             \int_{\inftrajectories{\latentmdp_{\decoderparameter}}} \decoder\fun{\trace \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \, d\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} & \text{else.} 
%         \end{cases} \label{eq:maximum-likelihood}
% \end{equation}
\begin{equation}
    \decoder\fun{\trace} =
            \int_{\inftrajectories{\latentmdp_{{\decoderparameter}}}} \decoder\fun{\trace \mid \seq{\latentvariable}{T}} \, d\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentvariable}{T}}, \label{eq:maximum-likelihood}
\end{equation}
%such that
%$\trace = \defaulttrace$,
$\trace = \langle \seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \rangle$,
$\latentvariable \in \latentvariables$ with $\latentvariables = \latentstates$ if $\latentactions = \actions$ and $\latentvariables = \latentstates \times \latentactions$ otherwise,
$\latentprobtransitions_{\latentpolicy_{\decoderparameter}}(\seq{\latentstate}{T}) = \prod_{t = 0}^{T - 1} \latentprobtransitions_{\latentpolicy_{\decoderparameter}}(\latentstate_{t + 1} \mid \latentstate_t)$, and $\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}(\seq{\latentstate}{T}, \seq{\latentaction}{T-1}) = \prod_{t = 0}^{T - 1} {\latentpolicy_{\decoderparameter}}(\latentaction_t \mid \latentstate_t) \cdot \latentprobtransitions_{\decoderparameter}(\latentstate_{t + 1} \mid \latentstate_t, \latentaction_t)$.
%Note that
The dependency of $\trace$ on $\latentvariables$ in Eq.~\ref{eq:maximum-likelihood}
is made explicit by the law of total probability.

Optimizing $\expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}}$ through Eq.~\ref{eq:maximum-likelihood} is typically intractable \citep{DBLP:journals/corr/KingmaW13}.
To overcome this, we use an encoder $\encoder\fun{\seq{\latentvariable}{T} \mid \trace}$ to set up
a \emph{lower bound} on the log-likelihood of produced traces,
%on the $\log$-values of Eq.~\ref{eq:maximum-likelihood}
often referred to as \emph{evidence lower bound} (ELBO, \citealp{DBLP:journals/jmlr/HoffmanBWP13}):
\begin{align*}
    &\log \decoder\fun{\trace} - \dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{\sampledot \mid \trace}}} \notag \\
    % = & \expectedsymbol{\seq{\latentvariable}{T} \sim \encoder\fun{\sampledot \mid \trace}} \log \fun{\nicefrac{\decoder\fun{\trace \mid \seq{\latentvariable}{T}} \cdot \latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentvariable}{T}}}{\encoder\fun{\seq{\latentvariable}{T} \mid \trace}}}
    = & \expected{\seq{\latentvariable}{T} \sim \encoder\fun{\sampledot \mid \trace}}{\log \decoder\fun{\trace \mid \seq{\latentvariable}{T}}}  - \dkl{\encoder\fun{\sampledot \mid \trace}}{\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}}
\end{align*}
The purpose of optimizing the ELBO is twofold.
First, this allows us learning $\embed_{\encoderparameter}$ via (i) $\encoder(\seq{\latentstate}{T} \mid \trace) = \prod_{t = 0}^{T} \embed_{\encoderparameter}(\latentstate_{t} \mid \state_t)$ or (ii) $\encoder(\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \mid \trace) = \encoder(\seq{\latentaction}{T-1} \mid \seq{\latentstate}{T}, \trace) \cdot \encoder(\seq{\latentstate}{T} \mid \trace)$, where $\encoder\fun{\seq{\latentaction}{T-1} \mid \seq{\latentstate}{T}, \trace} = \prod_{t = 0}^{T - 1} \latentembeda_{\encoderparameter}(\latentaction_t \mid \latentstate_t, \action_t)$, $\latentembeda_\encoderparameter$
%playing the role of an %stochastic
being an
action encoder.
We assume here that
%the encoding of states and actions to latent spaces is independent of rewards.
encoding states and actions to latent spaces is independent of rewards.
We additionally make them independent of $\seq{\labeling}{T}$ by assuming that
%the labeling function $\labels$ is known.
$\labels$ is known.
This allows $\embed_\encoderparameter$ to encode states and their labels directly into the latent space (cf. Sect.~\ref{subsec:discrete-latent-distr}).

% Second, we assume that the behavioral model $\decoder$ can be decomposed into reward and label models of $\latentmdp_{\decoderparameter}$, as well as a \emph{generative model} $\decoder^{\generative}$, enabling the reconstruction of states and actions.
%Therefore, states, actions, rewards, and labels can be made independent given the latent sequence:
Second, we assume the existence of latent reward and label models, i.e., $\decoder^{\rewards}$ and $\decoder^{\labels}$, allowing to recover respectively $\latentrewards_{\decoderparameter}$ and $\latentlabels_{\decoderparameter}$, as well as a \emph{generative model} $\decoder^{\generative}$, enabling the reconstruction of states and actions.
This allows decomposing the behavioral model $\decoder$ into:
%\todo{Can you triple check this? I feel like some intuition might help the reader be convinced without checking the equations --- and if we can let's use display equations}
% We thus argue that
% We thus argue that sequences (i) $\seq{\state}{T}$, $\seq{\action}{T}$ $\seq{\reward}{T - 1}$, and $\seq{\labeling}{T}$ can be made independent given $\tuple{\seq{\latentstate}{T}, \seq{\action}{T - 1}}$, while .
\begin{multline*}
\quad \quad \begin{aligned}
    &\decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentvariable}{T}} \\
    =& \decoder^{\generative}(\seq{\state}{T} \mid \seq{\latentstate}{T}) 
    \cdot \decoder^{\generative}(\seq{\action}{T - 1} \mid \seq{\latentvariable}{T}) \\
    & \cdot \decoder^{\rewards}(\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}) \cdot \decoder^{\labels}(\seq{\labeling}{T} \mid \seq{\latentstate}{T}),
\end{aligned}\\
% where (i)
% $\decoder^{\generative}(\seq{\state}{T} \mid \seq{\latentstate}{T}) = \prod_{t = 0}^{T} \decoder^{\generative}(\state_t \mid \latentstate_t)$,
% (ii) $\decoder^{\generative}(\seq{\action}{T - 1} \mid \seq{\latentstate}{T - 1}, \seq{\latentaction}{T - 1})$ is $\prod_{t = 0}^{T - 1} \latentpolicy_{\decoderparameter}(\latentaction_t \mid \latentstate_t)$ if $\latentactions = \actions$ and $\prod_{t = 0}^{T - 1} \embeda_{\decoderparameter}(\action_t \mid \latentstate_t, \latentaction_t)$ otherwise,
% (iii) $\decoder^{\rewards}(\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}) = \prod_{t = 0}^{T - 1} \decoder^{\rewards}(\reward_{t} \mid \latentstate_t, \latentaction_t)$,
% (iv) $\decoder^{\labels}(\seq{\labeling}{T} \mid \seq{\latentstate}{T}) = \prod_{t = 0}^{T}\decoder^{\labels}(\labeling_t \mid {\latentstate}_{t})$.
%The generative model (ii)
\begin{aligned}
    \text{where }\decoder^{\generative}(\seq{\state}{T} \mid \seq{\latentstate}{T}) &= \textstyle{\prod_{t = 0}^{T}} \, \decoder^{\generative}(\state_t \mid \latentstate_t), \\
    \decoder^{\generative}(\seq{\action}{T - 1} \mid \seq{\latentvariable}{T - 1}) &=
    \begin{cases}
        \textstyle{\prod_{t = 0}^{T - 1}}\, \latentpolicy_{\decoderparameter}(\action_t \mid \latentstate_t) \text{ if } \latentactions = \actions \\
        \prod_{t = 0}^{T - 1}\, \embeda_{\decoderparameter}(\action_t \mid \latentstate_t, \latentaction_t) \text{ else,}
    \end{cases} \\
    \decoder^{\rewards}(\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}) &= \textstyle{\prod_{t = 0}^{T - 1}} \, \decoder^{\rewards}(\reward_{t} \mid \latentstate_t, \latentaction_t), \text{and} \\
    \decoder^{\labels}(\seq{\labeling}{T} \mid \seq{\latentstate}{T}) &= \textstyle{\prod_{t = 0}^{T}} \, \decoder^{\labels}(\labeling_t \mid {\latentstate}_{t}).
\end{aligned}
\end{multline*}
Model $\embeda_{\decoderparameter}$
allows learning the action embedding function via $\embeda_{\encoderparameter, \decoderparameter}\fun{\action \mid \state, \latentaction} = \expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction}$ for all $\state \in \states, \action \in \actions, \latentaction \in \latentactions$.
We also argue that a \emph{perfect reconstruction} of labels is possible, i.e., $\decoder^{\labels}\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}} = 1$, due to the labels being encoded into the latent space.
%Intuitively, this can be done by encoding labels directly into the latent space. Details are given below.
From now on, we thus omit the label term.

% Deterministic embedding functions
% %$\embed_{\encoderparameter}\colon \states \! \to \latentstates$, $\embeda_{\encoderparameter, \decoderparameter} \colon \states \times \latentactions \to \actions$ and and reward function 
% $\latentrewards_{\decoderparameter} \colon \latentstates \times \latentactions \to \R$
%$\embed_{\encoderparameter}\fun{\state} = \mode{\embed_{\encoderparameter}\fun{\sampledot \mid \state}}$, $\embeda_{\encoderparameter, \decoderparameter}\fun{\state, \latentaction} = \mode{\embeda_{\decoderparameter}\fun{\sampledot \mid \embed_{\encoderparameter}\fun{\state}, \latentaction}}$, and $\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction} = \expectedsymbol{\reward \sim \decoder^{\rewards}\fun{\sampledot \mid \latentstate, \latentaction}} \reward$ for $\state \in \states, \latentaction \in \latentactions$.

Deterministic embedding functions $\embed_{\encoderparameter}$, $\embeda_{\encoderparameter, \decoderparameter}$
and $\latentrewards_{\decoderparameter}$
can finally be obtained by
taking the mode of their distribution.%

\smallparagraph{Back to the local setting.}~Taking Assumption~\ref{assumption:ergodicity} into account, drawing multiple finite traces $\trace \sim \mdp_{\policy}$ can be seen as a continuous interaction with $\mdp$ along an infinite trace \citep{DBLP:conf/nips/Huang20}.
This observation allows us to formulate the ELBO in the local setting\footnote{The expert reader might note this is not the standard definition of ELBO, we prove in Appendix (Corollary~\ref{cor:elbo-local}) that this reformulation is valid because of developments in Sect.~\ref{section:deepmdp}.}
and connect to local losses:
%and connect to local losses introduced in Sect.~\ref{section:deepmdp}:
%
% \begin{Lemma}\label{lem:elbo-local}
% Let  $\stationary{\policy}$ be the stationary distribution of $\mdp_\policy$, $f \colon \states \times \actions \times \images{\rewards} \times \states \to \R$ be a continuous function, and $\embed\fun{\latentstate, \latentstate' \mid \state, \state'} = \embed\fun{\latentstate \mid \state} \embed\fun{\latentstate' \mid \state'}$.
% Assume $\states, \actions$ are compact, then
% \begin{align*}
%     & \lim_{T \to \infty} \frac{1}{T} \expectedsymbol{}_{\substack{\trace \sim \mdp_{\policy}[T] \\ \seq{\latentvariable}{T} \sim \encoder\fun{\sampledot \mid \trace}}}
%     \begin{aligned}[t]
%     [&\log \decoder\fun{\trace \mid \seq{\latentvariable}{T}} \\ & \quad \quad  - \dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{ \sampledot \mid \trace}}} ] \end{aligned}\\
%     =&
%     \left\lbrace\begin{array}{@{}r@{\quad}l@{}}
%     \displaystyle \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy}\\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}} \big[
%     \begin{aligned}[t]
%         & \log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \latentpolicy_{\decoderparameter}\fun{\action \mid \latentstate} + \\
%         & \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action} - \\
%         & \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\sampledot\mid \latentstate}} \big] \text{ if } \latentactions = \actions \hfill \\
%     \end{aligned} \hfill \\[30pt]
%     \displaystyle \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy}\\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'} \\ \latentaction \sim \latentembeda_{\encoderparameter}\fun{\sampledot \mid \latentstate, \action}}}\big[
%     \begin{aligned}[t]
%         & \log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log\embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction} + \\
%         & \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \latentaction} - \\
%         & \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot\mid \latentstate}} - \\
%         & \dkl{\latentembeda_{\encoderparameter}\fun{\sampledot\mid\latentstate, \action}}{\latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \big]
%         \text{ else},
%     \end{aligned}\hfill
%     \end{array}
%     \right.
% \end{align*}
% %where $\trace = \defaulttrace$, $\seq{\latentvariable}{T} = \seq{\latentstate}{T}$ if $\latentactions = \actions$ and $\seq{\latentvariable}{T} = \tuple{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}$ otherwise.
% where $\mdp_{\policy}[T]$ denotes the distribution over $\traces{\mdp_\policy}$ of size $T$ and $ \stationary{\policy}(\state, \action, \reward, \state') = \stationary{\policy}(\state, \action, \state') \cdot \condition{=}(\reward,  \rewards\fun{\state, \action, \state'})$.
% \end{Lem.}
%
%We formulate the maximization of the \emph{local} ELBO\footnote{The expert reader might note this is not the standard definition of ELBO, we prove in Appendix that this reformulation is valid because of developments in Section~\ref{section:deepmdp}.} as
\[
%\begin{align*}
    \max_{\encoderparameter, \decoderparameter}\; \elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}} = - \min_{\encoderparameter, \decoderparameter} \left\{\distortion_{\encoderparameter, \decoderparameter} + \rate_{\encoderparameter, \decoderparameter} \right\},
%\end{align*}
\]
where $\distortion$ and $\rate$ denote respectively the \emph{distortion} and \emph{rate} of the variational model  \citep{DBLP:conf/icml/AlemiPFDS018}, given by
\begin{equation*}
    \distortion_{\encoderparameter, \decoderparameter} = -
    \left\lbrace\begin{array}{@{}r@{\quad}l@{}}
        \displaystyle \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy} \\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}} \big[
        \begin{aligned}[t]
        & \log \decoder^{\generative}(\state' \mid \latentstate') + \log \latentpolicy_{\decoderparameter}(\action \mid \latentstate) +
        \\
        & \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action}\big]
        \text{ if } \latentactions = \actions,
        \end{aligned} \hfill \\
        \displaystyle \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy} \\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'} \\ \latentaction \sim \latentembeda_{\encoderparameter}\fun{\sampledot \mid \latentstate, \action}}}
        \big[
        \begin{aligned}[t]
        & \log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \\
        & \log \embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction} + \\
        & \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \latentaction}\big] \text{ else, and}
        \end{aligned} \hfill
        \end{array}
    \right.
\end{equation*}
\begin{equation*}
    \rate_{\encoderparameter, \decoderparameter} =
    \left\lbrace\begin{array}{@{}r@{\quad}l@{}}
        \displaystyle \expectedsymbol{}_{\substack{\state, \action, \state' \sim \stationary{\policy} \\ \latentstate \sim \embed_{\encoderparameter}(\sampledot \mid \state)}}  \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\latentpolicy_{\decoderparameter}}(\sampledot \mid \latentstate)} \text{ if } \latentactions = \actions, \hfill \\
        \displaystyle \expectedsymbol{}_{\substack{\state, \action, \state' \sim \stationary{\policy} \\ \latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state} \\ \latentaction \sim \latentembeda_{\encoderparameter}\fun{\sampledot \mid \latentstate, \action} }}
        \big[
        \begin{aligned}[t]
        & \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} + \\
        & \dkl{\latentembeda_{\encoderparameter}\fun{\sampledot\mid\latentstate, \action}}{\latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \big] \text{ else.}
        \end{aligned} \hfill
    \end{array}
    \right.
\end{equation*}
%
We omit the subscripts when the context is clear.
The optimization of $\elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}}$ allows for an indirect optimization of the local losses through their variational versions:
(i) $\localrewardloss{\stationary{\latentpolicy}}$ via the log-likelihood of rewards produced, and % by taking $\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction} = \expectedsymbol{\reward \sim \decoder^{\rewards}\fun{\sampledot \mid \latentstate, \latentaction}} \reward$, and
(ii) $\localtransitionlossupper{\stationary{\latentpolicy}}$ where we change the Wasserstein term to the KL divergence.
Note that this last change means we do not necessarily obtain the theoretical guarantees on the quality of the abstraction via its optimization. Nevertheless, our experiments indicate KL divergence is a good proxy of the Wasserstein term in practice.
%it \todo{odd way to end the section, why is this loss of guarantees not a problem?} (cf.\todo{The right way to write it is cf. not c.f., check the whole doc.} Eq.~\ref{eq:bidistance-abstraction-quality} and Eq.~\ref{eq:value-diff-abstraction-quality}).

\subsection{VAE Distributions}\label{subsec:discrete-latent-distr}
\smallparagraph{Discrete distributions.}~We aim at learning \emph{discrete} latent spaces $\latentstates$ and $\latentactions$, the distributions $\embed_{\encoderparameter}$, $\encoder^{\actions}$, $\latentprobtransitions_{\decoderparameter}$, and $\latentpolicy_{\decoderparameter}$ are thus supposed to be discrete.
Two main challenges arise:
%by learning the parameters of discrete distributions via
% stochastic computation graphs through %optimization techniques such as
%\emph{gradient descent} and \emph{Monte-Carlo sampling} methods:
%\todo{F: cut here}
(i) gradient descent is not applicable to learn $\encoderparameter$ and $\decoderparameter$ due to the discontinuity of $\latentstates$ and $\latentactions$, and (ii) sampling from these distributions must be a \emph{derivable operation}.
We overcome these by using \emph{continuous relaxation of Bernoulli distributions} to learn a binary representation of the latent states, and the \emph{Gumbel softmax trick} for the latent action space \citep{DBLP:conf/iclr/JangGP17,DBLP:conf/iclr/MaddisonMT17}.
% Intuitively, they rely on a temperature parameter $\temperature$ that makes the continuous distributions converging to their discrete variant when $\temperature$ converges to $0$.

\smallparagraph{Labels.}~To enable $\log \decoder^\labels\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}} = 0$, we encode $\labels\fun{\state_t} = \labeling_t$ into each $\latentstate_t$ via $\embed_{\encoderparameter}$.
Recall each label is given in binary. We thus allocate $|\atomicprops|$ bits in $\latentstates$ for the labels.
Then, $\embed_{\encoderparameter}\fun{\latentstate \mid \state} > 0$ implies $\labels\fun{\state} = \latentlabels_\decoderparameter\fun{\latentstate}$, for all $\state \in \states, \latentstate \in \latentstates$,
\iffalse
This enforces the following property of $\embed_{\encoderparameter}$:
\[
\forall \state \in \states, \, \forall \latentstate \in \latentstates,\, \embed_{\encoderparameter}\fun{\latentstate \mid \state} > 0 \implies \labels\fun{\state} = \latentlabels_\decoderparameter\fun{\latentstate},
\]
\fi
satisfying Assumption~\ref{assumption:labeling} if $\embed_{\encoderparameter}$ is deterministic.

\smallparagraph{Decoders.}~For $\decoder^{\generative}$, $\embeda_{\decoderparameter}$, and $\decoder^{\rewards}$, we learn the parameters of multivariate normal distributions.
%Models $\decoder^{\generative}$, $\embeda_{\encoderparameter, \decoderparameter}$ thus allow generating grounded states or actions %from the environment
%based on their latent embedding.
%While our approach allows learning a meaningful representation of the input model and policy through latent state and action spaces,
This further allows linking all $\latentstate \in \latentstates$ to the parameters of $\decoder^{\generative}(\sampledot \mid \latentstate)$ for explainability.
%This allows each $\latentstate \in \latentstates$ to be linked to the normal parameters of $\decoder^{\generative}(\sampledot \mid \latentstate)$ for explainability purposes.

% \smallparagraph{Deterministic functions.}~%
% % Deterministic embedding functions
% $\embed_{\encoderparameter}$, $\embeda_{\encoderparameter, \decoderparameter}$ and and
% %reward function 
% $\latentrewards_{\decoderparameter}$
% %$\latentrewards_{\decoderparameter}$
% can be obtained by
% taking the mode of their learned distribution.%

\subsection{Posterior Collapse}\label{sec:posterior-collapse}
A common issue encountered while optimizing variational models via the ELBO is %so called
\emph{posterior collapse}.
Intuitively, this results in a degenerate local optimum where the model learns to ignore the latent space.
%while the generative model alone is used to optimize the ELBO.
With a discrete encoder, this translates into a deterministic mapping to a single latent state, regardless of the input.
%From a formal-abstraction point of view,
%From a model-checking standpoint, this means 
%the VAE derives this coarse abstraction by ``learning a BSCC decomposition of $\mdp$'', consisting in a unique absorbing state since $\mdp$ is ergodic.
%
%
From an information-theoretic point of view, optimizing the ELBO gives way to a trade-off between the minimization of
%the rate and the distortion
$\rate$ and $\distortion$, where the feasible region is a convex set \citep{DBLP:conf/icml/AlemiPFDS018}.
%Posterior collapse happens when the rate is close to zero
Posterior collapse occurs when $\rate \approx 0$
%(referred to as the \emph{auto-decoding limit} of the variational model).
(\emph{auto-decoding limit}).
%, which can be achieved by the optimizer by merging all states to the same embedding.
%$\expected{\trace \sim \mdp_\policy}{\sum_{t=0}^{T - 1}\dkl{\encoder^\transitions\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \action_t}}} \approx 0$, meaning
% $\encoder^\transitions\fun{\seq{\latentstate}{T} \mid \seq{\state}{T}, \seq{\action}{T - 1}} \approx \latentprobtransitions_{\decoderparameter}\fun{\seq{\latentstate}{T} \mid \seq{\action}{T - 1}}$.
%$\log \embed_{\encoderparameter}\fun{\latentstate' \mid \state'} \approx \expected{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}{\log \latentprobtransitions_{\decoderparameter}\fun{{\latentstate}' \mid \latentstate, {\action}}}$ for any $\latentstate' \in \latentstates$ by definition of the KL divergence.
%This means (i) the embedding distribution is nearly independent of ${\state' \in \states}$, and (ii) the latent  transition distribution tends to ignore $\action \in \actions$.
% The latent representation is thus not encoding information about input transitions, meaning that it fails to create a useful representation.
%On the other hand, one can achieve a distortion close to zero
On the other hand, one can achieve $\distortion \approx 0$
%(referred to as the \emph{auto-encoding limit})
(\emph{auto-encoding limit})
at the price of a higher rate.

% As already mentioned, posterior collapse is a consequence of the KL divergence here replacing the Wasserstein in the rate minimization: when the latter is used, Lem.~\ref{Lem.:local-loss-upper-bounds} and Lem.~\ref{Lem.:bidistance-abstraction-quality} ensure that a value close to zero implies a bisimilarity between states embedded to the same representation.

% \smallparagraph{Regularization terms.}
% Various solutions have been proposed in the litterature to prevent posterior collapse.
% They include \emph{KL-scaling} % and \emph{KL-annealing}
% consisting in changing $\elbo$ to $\beta\text{-}\elbo = -(\distortion + \beta \cdot \rate)$, with $\beta \in \mathopen[0, 1\mathclose]$.
% This allows to interpolate between auto-encoding and auto-decoding behavior, which is not possible with the standard ELBO objective.

% Another method consists in adding an \emph{entropy regularizer} $\alpha \in \mathopen[0, \infty\mathclose[$ to $\elbo$, i.e.,
% $
%     \alpha\text{-}\elbo = \elbo + \alpha \cdot \entropy{\encoder},
% $
% and anneal $\alpha$ to 0 during training \citep{DBLP:conf/icml/HaarnojaZAL18,DBLP:conf/corl/BurkeHR19}, where 
% $\entropy{\encoder}$ denotes the entropy of an encoding distribution.
% We choose to measure the entropy of the \emph{marginal} encoder, given by $\encoder\fun{\latentstate} = \expectedsymbol{\state \sim \stationary{\policy}} \embed_{\encoderparameter}\fun{\latentstate \mid \state}$. 
% Intuitively, this encourages the encoder to learn to make plenty use of the latent space. % to represent the input data.

% A drawback of these methods is that we are no longer optimizing a lower bound on the log-likelihood of the input while optimizing
% % $\tuple{\alpha, \beta}\text{-}\elbo(\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}) = - (\distortion_{\encoderparameter, \decoderparameter} + \beta \cdot \rate_{\encoderparameter, \decoderparameter}) + \alpha \cdot \entropy{\embed_{\encoderparameter}}$.
% $\tuple{\alpha, \beta}\text{-}\elbo = - (\distortion + \beta \cdot \rate) + \alpha \cdot \entropy{\encoder}$.
% In practice, setting up annealing schemes for $\alpha$ and $\beta$ allows to eventually recover $\elbo$ and avoid posterior collapse ($\alpha=0$ and $\beta=1$ matches $\elbo$).
\smallparagraph{Regularization terms.}~%
Various solutions have been proposed in the literature to prevent posterior collapse.
They include \emph{entropy regularization} (via $\alpha \in \mathopen[ 0, \infty \mathclose[$, \citealt{DBLP:conf/icml/HaarnojaZAL18,DBLP:conf/corl/BurkeHR19}) and
\emph{KL-scaling} (via $\beta \in \mathopen[0, 1\mathclose]$, e.g., \citealt{DBLP:conf/icml/AlemiPFDS018}),
consisting in changing $\elbo$ to
$\tuple{\alpha, \beta}\text{-}\elbo = - (\distortion + \beta \cdot \rate) + \alpha \cdot \entropy{\encoder}$, where 
$\entropy{\encoder}$ denotes the entropy of an encoding distribution.
We choose to measure the entropy of the \emph{marginal} encoder, given by $\encoder\fun{\latentstate} = \expectedsymbol{\state \sim \stationary{\policy}} \embed_{\encoderparameter}\fun{\latentstate \mid \state}$. 
Intuitively, this encourages the encoder to learn to make plenty use of the latent space. % to represent the input data.
The parameter $\beta$ allows to interpolate between auto-encoding and auto-decoding behavior, which is not possible with the standard ELBO objective.

A drawback of these methods is that we no longer optimize a lower bound on the log-likelihood of the input while optimizing
% $\tuple{\alpha, \beta}\text{-}\elbo(\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}) = - (\distortion_{\encoderparameter, \decoderparameter} + \beta \cdot \rate_{\encoderparameter, \decoderparameter}) + \alpha \cdot \entropy{\embed_{\encoderparameter}}$.
$\tuple{\alpha, \beta}\text{-}\elbo$.
In practice, setting up annealing schemes for $\alpha$ and $\beta$ allows to eventually recover $\elbo$ and avoid posterior collapse ($\alpha=0$ and $\beta=1$ matches $\elbo$).

% \cite{DBLP:conf/iclr/HeSNB19} introduced a method only based on the training process of the variational model, which allows to overcome this problem.
% It consists in an aggressive training schedule which iterates between multiple updates of $\encoderparameter$ and one update of $\decoderparameter$, based on the observation that the inference model often lags behind the reconstruction model during training when posterior collapse occurs.
% In our experiments, we also noticed that posterior collapse is even more difficult to handle when the entropy of the produced traces is low, in particular when rewards and states produced by executing $\policy$ have low variance.
%This can be explained by an auto-encoding behavior: \cite{DBLP:conf/icml/AlemiPFDS018} showed that $\dataentropy - \rate$ is an upper bound on the distortion $\distortion$ that can be achieved, with $\dataentropy$ being the entropy of the input distribution (in our case $\dataentropy = \entropy{\stationary{\policy}}$).
% When $\entropy{\stationary{\policy}}$ is low, the optimizer may tend to minimize the distortion by pushing the rate close to zero and achieve this way the low entropy of the input distribution.
% \begin{figure*}[t]
%     \begin{subfigure}{0.495\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{ressources/cartpole_histogram.pdf} \\
%         \caption{CartPole}
%     \end{subfigure}
%     \begin{subfigure}{0.495\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{ressources/mountain_car_histogram.pdf} \\
%         \caption{MountainCar}
%     \end{subfigure}
%     \caption{Latent space distribution along training steps. The intensity of the blue hue corresponds to the frequency of latent states produced by $\embed$ during training. We compare a bucket-based prioritized against a simple uniform experience replay. The latent space learned with transitions sampled from the uniform replay buffer collapses to (a) two and (b) a single latent state(s).}
%     \label{fig:prioritized-replay}
% \end{figure*}
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{ressources/cartpole_histogram.pdf}
    \caption{Latent space distribution along training steps for the CartPole environment. The intensity of the blue hue corresponds to the frequency of latent states produced by $\embed_{\encoderparameter}$ during training. We compare a bucket-based prioritized against a simple uniform experience replay.
    % The latent space learned with transitions sampled from the uniform replay buffer collapses to two latent states.}
    The latent space learned via the uniform buffer collapses to two latent states.}
    \label{fig:prioritized-replay}
\end{figure}
\smallparagraph{Prioritized replay buffers.}~%
To enable meaningful use of latent space to represent input state-actions pairs,
%states that are reached under $\policy$ but not seen often should not be ignored during the learning process.
$\encoder$ should learn to (i) exploit the entire latent space, and (ii) encode wisely states and actions of transitions yielding poor ELBO, being generally sensitive to bad representation embedding.
%This motivates us to use a \emph{prioritized replay buffer} \citep{DBLP:journals/corr/SchaulQAS15} to store and sample environment transitions.
This motivates us to use a \emph{prioritized replay buffer} \citep{DBLP:journals/corr/SchaulQAS15} to store transitions and sample them when optimizing $\elbo$.
Draw $\tuple{\state, \action, \reward, \state'} \sim \stationary{\policy}$ and let $p_{\tuple{\state, \action, \reward, \state'}}$ be its priority, we introduce the following priority functions.

\begin{itemize}
    % \item \emph{Bucket-based priority:}~the replay buffer is partitioned in $|\latentstates|$ \emph{buckets}.
    % Each bucket $b \colon \latentstates \to \N$ is a latent state counter that is incremented each time a latent state is drawn from $\embed_{\encoderparameter}$.
    % We also maintain a training step counter $N$.
    % At each step, let $\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}$, we assign $p_{\tuple{\state, \action, \reward, \state'}}$ to $\nicefrac{N}{b\fun{\latentstate}}$, then increment $N$ and $b\fun{\latentstate}$ of $1$.
    % This allows the encoder to learn from transitions for which the embedding of their incident state is not seen often under $\policy$ and fairly distribute the latent space.
    \item \emph{Bucket-based priority:}~we partition the buffer in $|\latentstates|$ \emph{buckets}.
    Let $N \in \N$ and $b \colon \latentstates \to \N$ be respectively step and latent state counters.
    At each step, let $\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}$, we assign $p_{\tuple{\state, \action, \reward, \state'}}$ to $\nicefrac{N}{b\fun{\latentstate}}$, then increment $N$ and $b\fun{\latentstate}$ of one.
    This allows $\embed_\encoderparameter$ to process states being infrequently visited under $\policy$ and learn to fairly distribute $\latentstates$.
    % This allows $\embed_\encoderparameter$ to consider transitions for which the embedding of their incident state is infrequently visited under $\policy$, and learn to fairly distribute $\latentstates$.
    % and learn to make plenty use of the latent space.
    \item \emph{Loss-based priority:}~we set $p_{\tuple{\state, \action, \reward, \state'}}$ to its individual transition loss,
    %$- \loss_{\elbo}$, i.e., for $\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}$ and $\latentaction \sim \encoder^\actions\fun{\sampledot \mid \latentstate, \action}$ if $\latentactions \neq \actions$ and $\latentaction = \action$ else,
    % \begin{align*}
    %     & \loss_{\elbo}\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentaction, \latentstate'}} \\
    %     =&  - \log \decoder^\generative\fun{\state' \mid \latentstate'} - \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \latentaction} - \log \latentpolicy_{\decoderparameter}\fun{\latentaction \mid \latentstate} + \log \embed_{\encoderparameter}\fun{\latentstate' \mid \state'} \\
    %     & - \condition{=}\fun{\latentactions, \actions} \cdot \log \latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\latentstate' \mid \latentstate} \\
    %     & - \condition{\neq}\fun{\latentactions, \actions} \cdot \fun{\log \embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction} + \log \latentprobtransitions_{\decoderparameter}\fun{\latentstate' \mid \latentstate, \latentaction} - \log \encoder^{\actions}\fun{\latentaction \mid \latentstate, \action}}.
    % \end{align*}
    which enables to learn improving the representation of states and actions that yield poor ELBO.
\end{itemize}
%

==> pomdp_formulation.tex <==
\todo[inline]{F: {\color{red} DEPRECATED}}
\smallparagraph{Partially observable MDPs.} A \emph{partially observable MDP} (POMDP) is a tuple $\pomdp = \pomdptuple$ where $\mdp$ is the underlying MDP modeling the environment, $\observations$ is a set of \emph{observations}, and $\observe \colon \actions \times \states \to \distributions{\observations}$ is an \emph{observation function}.
Intuitively, $\observe(\observation \mid \action, \state')$ is the probability of observing $\observation$ when $\action$ is chosen and the resulted state in $\mdp$ is $s'$.

In POMDP $\pomdp$, the agent does not directly perceive states from $\mdp$ but perceives observations of the environment instead.
Therefore, a \emph{history} of $\pomdp$ is a sequence of actions and observations $\historytuple{\action}{\observation}{T}$ such that $\exists \trajectorytuple{\state}{\action}{T} \in \trajectories{\mdp}$ with $\observe\left(\observation_{t+1} \mid \action_t, \state_{t+1}\right) > 0$ for $t \in \set{0, \dots, T-1}$, $T \in \N$. The set of histories of $\pomdp$ is $\histories{\pomdp}$.
According to an observed history, a \emph{belief} $\belief \in \distributions{\states}$ can be maintained, giving the probability for the agent of being in each particular state of $\mdp$ \citep{DBLP:conf/aaai/CassandraKL94}.
Agent policies do not depend on trajectories of $\mdp$ since they are not observable, but rather on observed histories in $\pomdp$ or (sequences of) such beliefs.

The initial belief $\belief_I(\state)$ is equal to $1$ if $\state = \sinit$, and $0$ otherwise. Then, the belief can be updated
%via the \emph{state estimator distribution}
according to $\stateestimator\colon \distributions{\states} \times \actions \times \observations \to \distributions{\states}$, $\stateestimator\fun{\state' \mid \belief, \action, \observation}$ being the probability of transitioning to state $\state'\in \states$ when the current belief is $\belief$, the action $\action \in \actions$ is executed, and $\observation \in \observations$ is perceived afterwards.
By Bayes' rule, we have
\begin{equation*}
    \stateestimator\left(\state' \mid \belief, \action, \observation\right) = \frac{\stateestimator(\observation \mid \belief, \action, \state') \cdot \stateestimator(\state'\mid\belief, \action)}{\stateestimator(\observation \mid \belief, \action)}
\end{equation*}
with
$\stateestimator\left(\observation \mid \belief, \action, \state'\right) = \observe\left(\observation \mid \action, \state'\right)$,
$\stateestimator(\state'\mid\belief, \action) = \sum_{\state \in \states} \transitions\left(\state, \action, \state'\right) \cdot \belief(\state)$,
and $\stateestimator\left(\observation \mid \belief, \action\right) = \sum_{\state' \in \states} \stateestimator\left(\observation \mid \belief, \action, \state'\right) \cdot \stateestimator(\state'\mid\belief, \action)$.
Therefore, the belief update for state $\state'$ is given by
\begin{equation*}
    \belief^{\action, \observation}(\state') = \stateestimator\left(\state' \mid \belief, \action, \observation\right) = \frac{\observe\left(\observation \mid \action, \state'\right) \cdot \sum_{\state \in \states} \transitions\left(\state, \action, \state'\right) \cdot \belief(\state)}{\sum_{\state' \in \states} \observe\left(\observation \mid \action, \state'\right) \cdot \sum_{\state \in \states} \transitions\left(\state, \action, \state'\right) \cdot \belief\fun{\state}}
\end{equation*}
%\todo{G: I don't understand this part, it is looks very complicated whereas belief updates are very intuitive, maybe it's $\sigma$ that has to be better explained?}
The set of reachable beliefs $\beliefs$ constructed this way allows $\pomdp$ to be formulated as an equivalent (infinite) MDP $\beliefmdp$ with state space $\beliefs$, same action space $\actions$, transition probability distribution $\probtransitions{\beliefs}$ such that $\probtransitions{\beliefs}\left(\belief' \mid \belief, \action \right)$ is equal to $\stateestimator\left(\observation \mid \belief, \action \right)$ if $\belief'=\belief^{\action, \observation}$ and $0$ otherwise, and reward function $\beliefrewards{\beliefs}\left(\belief, \action\right) = \sum_{\state \in \states} \belief\left(\state\right) \cdot \rewards(\state, \action)$.
%\todo{G: continuous is a vague word here, in fact a countably infinite state space is enough. No need for real numbers here right? Or did you start with a partially observable continuous space MDP?}

We assume the environment being modeled by an unknown continuous-space MDP $\mdp_\states = \statesmdptuple{\states}{\state}$, where $\states$ is a continuous state space.
In order to recover a policy with formal guarantees in $\mdp_\states$, we learn a finite abstraction of the environment in which model-checking techniques can be applied.
Specifically, we learn a new MDP $\mdp_\latentstates = \statesmdptuple{\latentstates}{\latentstate_I}$ with finite state space $\latentstates$ via a stochastic encoder $\encoder \colon \states \times \actions \times \rewards \times \states \times 2^{\atomicprops} \to \distributions{\latentstates}$.
We assume $\encoder\fun{\latentstate' \mid \state, \action, \reward, \state', \labels_{\scriptscriptstyle\states}\fun{\state'}} > 0 \iff \labels_{\scriptscriptstyle\states}\fun{\state'} = \labels_{\scriptscriptstyle\latentstates}\fun{\latentstate'}$.
Intuitively, $\encoder\fun{\latentstate' \mid \state, \action, \reward, \state', \labeling'}$ gives the probability of being in state $\latentstate$ in $\mdp_\latentstates$ after observing transition $\tuple{\state, \action, \reward, \state', \labeling'}$ in $\mdp_\states$.
Such an encoder allows producing discrete states that share similar labels, transition dynamics and rewards.

\smallparagraph{POMDP formulation.} Let $\encoder\fun{\latentstate' \mid \state, \action, \state'} = \encoder\fun{\latentstate' \mid \state, \action, \rewards_{\scriptscriptstyle \states}\fun{\state, \action, \state'}, \state', \labels_{\scriptscriptstyle \states}\fun{\state'}}$.
From $\tracetuple{\state}{\action}{\reward}{\labeling}{T} \in \traces{\mdp_\states}$, one can recover $\tracetuple{\latentstate}{\action}{\reward}{\labeling}{T} \in \traces{\mdp_\latentstates}$ by sampling $\sample{\latentstate_{t+1}}{\encoder}\fun{\sampledot \mid \state_t, \action_t, \state_{t+1}}$ for $t \in \set{0, \dots, T - 1 }$.
Precisely, after observing sequence $\historytuple{\action}{\state}{t}$, the agent executes an action ${\action}_{t} \in \act{\state_t}$, observes ${\state}_{t+1} \in \states$ and goes to state $\latentstate_{t + 1} \in \latentstates$ with probability $\encoder\fun{\latentstate_{t + 1} \mid {\state}_{t}, {\action}_{t}, {\state}_{t+1}}$. 
In the following, we show that an agent acting this way is equivalent to acting in a POMDP where the belief state over $\latentstates$ is induced by $\encoder$.

Let POMDP $\pomdp_\latentstates = \tuple{\mdp_\latentstates, \states, \observe}$ with $\observe\colon \states \times \actions \times \latentstates \to \distributions{\states}$ such that $\observe\fun{\state' \mid \state, \action, \latentstate'}$ is the probability of observing $\state'$ when the last observation was $\state$, then $\action$ is executed and the resulted state in $\mdp_\latentstates$ is $\latentstate'$.
% Notice that $\observe$ is slightly different from the general definition. In the following, we will see this is not a problem due to the belief space being induced by $\encoder$.
By Bayes' rule, we have
$\observe\fun{\state' \mid \state, \action, \latentstate'} = {\encoder\fun{\latentstate' \mid \state, \action, \state'} \cdot \probtransitions{\states}\fun{\state' \mid \state, \action}}/{\transitiontolatent\fun{\latentstate' \mid \state, \action}}$.
Intuitively, $\transitiontolatent\fun{\latentstate' \mid \state, \action}$ is the probability of transitioning to $\latentstate'$ in $\mdp_\latentstates$ when $\action \in \actions$ is chosen.
By construction, $\transitiontolatent\fun{\latentstate' \mid \state, \action} = \sum_{\state' \in \states} \encoder\fun{\latentstate' \mid \state, \action, \state'} \cdot \probtransitions{\states}\fun{\state' \mid \state, \action}$.
\begin{lemma}\label{belief-independent}
Let $\tuple{\action_{\scriptscriptstyle 0:t}, \state_{\scriptscriptstyle 1:t+1}} \in \histories{\pomdp_\latentstate}$ and $\belief_t$ be the belief of $\pomdp_\latentstates$ after observing $\historytuple{\action}{\state}{t}$,
then (i) $\stateestimator\fun{\state_{t + 1} \mid \belief_t, \action_t} = \probtransitions{\states}\fun{\state_{t + 1} \mid \state_t, \action_t}$, , (ii) $\indexof{\rewards}{\distributions{\latentstates}}\fun{\belief_t, \action_t} = \indexof{\rewards}{\states}\fun{\state_t, \action_t}$, and (iii) for all $\latentstate' \in \latentstates$, $\stateestimator\fun{\latentstate' \mid \belief_t, \action_t} = \probtransitions{\states, \latentstates}\fun{\latentstate' \mid \state_t, \action_t}$.
\end{lemma}
\begin{proof}
The belief space of any POMDP is a \emph{sufficient information state space process} \citep{DBLP:journals/jair/Hauskrecht00} that preserves the probability of being in each particular state of the underlying MDP and the probability of the new observation when an action in executed.
In $\pomdp_\latentstates$, that means $\stateestimator\fun{\state_{t + 1} \mid \tuple{\action_{\scriptscriptstyle 0:t-1}, \state_{\scriptscriptstyle 1:t}}, \action_t} = \stateestimator\fun{\state_{t + 1} \mid \belief_t, \action_t}$.
The results follow then from the fact that the history $\historytuple{\action}{\state}{t}$ associated with $\belief_t$ corresponds to the trajectory $\tuple{\sinit, \state_{\scriptscriptstyle 1:t}, \action_{\scriptscriptstyle 0:t-1}}$ in $\mdp_\states$.
By the Markov property, the probability distribution and reward obtained by choosing $\action_t$ in $\state_t$ do not depend on the past history, so we have (i) $\stateestimator\fun{\state_{t + 1} \mid \belief_t, \action_t} = \stateestimator\fun{\state_{t + 1} \mid \tuple{\action_{\scriptscriptstyle 0:t-1}, \state_{\scriptscriptstyle 1:t}}, \action_t} = \probtransitions{\states}\fun{\state_{t + 1 } \mid \sinit, \state_{\scriptscriptstyle 1:t}, \seq{\action}{t}} = \probtransitions{\states}\fun{{\state_{t+1} \mid \state_t, \action_t}}$, (ii) $\indexof{\rewards}{\distributions{\latentstates}}\fun{\belief_t, \action_t} = \indexof{\rewards}{\states}\fun{\tuple{\sinit, \indexof{\state}{1:t-1}, \indexof{\action}{0:t-1}}, \state_t, \action_t} = \indexof{\rewards}{\states}\fun{\state_t, \action_t}$, and (iii) $\stateestimator\fun{\latentstate' \mid \belief_t, \action_t} =
\sum_{\state' \in \states} \encoder\fun{\latentstate' \mid \state_t, \action_t, \state'} \cdot \stateestimator\fun{\state' \mid \tuple{\action_{\scriptscriptstyle 0:t-1}, \state_{\scriptscriptstyle 1:t}}, \action_t} = 
\sum_{\state' \in \states} \encoder\fun{\latentstate' \mid \state_t, \action_t, \state'} \cdot \probtransitions{\states}\fun{\state' \mid \state_t, \action_t} = \transitiontolatent\fun{\latentstate' \mid \state_t, \action_t}$.
\end{proof}
%
As a consequence, for any belief $\belief$ of $\pomdp_\latentstates$ and $\action \in \actions$, $\stateestimator\fun{\sampledot \mid \belief, \action}$ can be made independent of $\belief$ provided that the last observation is known.
%
\begin{corollary}
The belief space of $\pomdp_\latentstates$ is $\latentbeliefspace = \set{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \state, \state' \in \states, \, \action \in \act{\state} } \cup \set{\encoder^I}$ with $\encoder^I \in \distributions{\latentstates}$ such that $\encoder^I\fun{\latentstate} \text{ is equal to } 1 \text{ if } \latentstate = \latentstate_I, \, 0 \text{ else}$.
\end{corollary}
%
\begin{proof}
Let $\tuple{\action_{\scriptscriptstyle 0:t}, \state_{\scriptscriptstyle 1:t+1}} \in \histories{\pomdp_\latentstate}$ and $\belief_t$ be the belief of $\pomdp_\latentstates$ after observing $\historytuple{\action}{\state}{t}$.
Assume $\belief_t \in \set{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \state, \state' \in \states, \, \action \in \act{\state} } \cup \set{\encoder^I}$.
By definition, the next belief $\belief_{t + 1}$ after executing $\action_t$ and observing $\state_{t + 1}$ thereafter is given by $\belief_{t}^{\action_t, \state_{t + 1}}$ where for all $\latentstate_{t + 1} \in \latentstates$,
\begin{align*}
    \belief_{t}^{\action_t, \state_{t + 1}}&\fun{\latentstate_{t + 1}} = \stateestimator\fun{\latentstate_{t + 1} \mid \encoder\fun{\sampledot \mid \state_{t - 1}, \action_{t - 1}, \state_{t}}, \action_t, \state_{t + 1}}\\
    &= \frac{\stateestimator(\state_{t + 1} \mid \encoder\fun{\sampledot \mid \state_{t - 1}, \action_{t - 1}, \state_{t}}, \action_t, \latentstate_{t + 1}) \cdot \stateestimator(\latentstate_{t + 1} \mid \encoder\fun{\sampledot \mid \state_{t - 1}, \action_{t - 1}, \state_{t}}, \action_t)}{\stateestimator(\state_{t + 1} \mid \encoder\fun{\sampledot \mid \state_{t - 1}, \action_{t - 1}, \state_{t}}, \action_t)}\\
    &= \frac{\stateestimator(\state_{t + 1} \mid \encoder\fun{\sampledot \mid \state_{t - 1}, \action_{t - 1}, \state_{t}}, \action_t, \latentstate_{t + 1}) \cdot \probtransitions{\states, \latentstates}\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\probtransitions{\states}\fun{\state_{t + 1} \mid \state_t, \action_t}} \tag{by Lemma~\ref{belief-independent}}\\
    &= \frac{\fun{\sum_{\state \in \states} \stateestimator\fun{\state \mid \encoder\fun{\sampledot \mid \state_{t - 1}, \action_{t - 1}, \state_{t}}} \cdot \observe\fun{\state_{t + 1} \mid \state, \action_t, \latentstate_{t + 1}}} \cdot \probtransitions{\states, \latentstates}\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\probtransitions{\states}\fun{\state_{t + 1} \mid \state_t, \action_t}}\\
    &= \frac{\observe\fun{\state_{t + 1} \mid \state_{t}, \action_t, \latentstate_{t + 1}} \cdot \probtransitions{\states, \latentstates}\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\probtransitions{\states}\fun{\state_{t + 1} \mid \state_t, \action_t}}\tag{$\stateestimator\fun{\state \mid \encoder\fun{\sampledot \mid \state_{t - 1}, \action_{t - 1}, \state_{t}}}$ is $1$ if $\state = \state_t$, $0$ else}\\
    &= \frac{\encoder\fun{\latentstate_{t + 1} \mid \state_t, \action_t, \state_{t + 1}} \cdot \probtransitions{\states}\fun{\state_{t + 1} \mid \state_t, \action_t} \cdot \probtransitions{\states, \latentstates}\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\transitiontolatent\fun{\latentstate_{t + 1} \mid \state_t, \action_t} \cdot \probtransitions{\states}\fun{\state_{t + 1} \mid \state_t, \action_t}}\\
    &= \encoder\fun{\latentstate_{t + 1} \mid \state_t, \action_t, \state_{t + 1}}
\end{align*}
The result is then obtained by induction over histories of $\pomdp_\latentstates$.
\end{proof}
%
Contrarily to general POMDPs, the beliefs over the states of the underlying MDP thus only depend on a limited history of $\pomdp_\latentstates$,  namely the last observation, the last action executed and the new observation.
%In the following, we show that there is an equivalence between $\mdp_\states$ and $\pomdp_\latentstates$ that preserves the probability of trajectories and their return.
We formally define the belief MDP as follows.

\smallparagraph{Belief MDP.} The \emph{belief MDP} of $\pomdp_\latentstates$ is $\mdp_\latentbeliefspace = \statesmdptuple{\latentbeliefspace}{\encoder^I}$.
Let $\previousstate, \state \in \states \cup \set{{\scriptstyle\top}}$, $\previousaction \in \act{\previousstate}$, $\action \in \act{\state}$ and $\belief' \in \latentbeliefspace$.
The components of $\mdp_\latentbeliefspace$ are defined as follows.
From the initial belief, we assume that $\mdp_\states$ is in $\state = \sinit \in \states$.
Therefore, we formulate the initial belief as $\encoder^I = \encoder\fun{\sampledot \mid {\scriptstyle\top}, \indexof{\action}{\top}, \sinit}$ for some dummy state $\scriptstyle\top$ and action $\indexof{\action}{\top} \in \act{{\scriptstyle\top}}$.
Then, for belief $\encoder\fun{\sampledot \mid \previousstate, \previousaction, \state} \in \latentbeliefspace$, $\act{\encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}} = \act{\state}$, and
$\probtransitions{\latentbeliefspace}\fun{\belief' \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}, \action} = 0$ if $\belief' \neq \encoder\fun{\sampledot \mid \state, \action, \state'}$ for all $\state' \in \states$.
Otherwise,
\begin{align*}
    \probtransitions{\latentbeliefspace}&\fun{\encoder\fun{\sampledot\mid\state, \action, \state'} \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}, \action} = \stateestimator\fun{\state'\mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}, \action} = \probtransitions{\states}\fun{\state'\mid \state, \action}%\tag{by Lemma~\ref{belief-independent}}
%    &= \probtransitions{\states}\fun{\state'\mid \state, \action} \cdot \sum_{\latentstate'\in\latentstates} \encoder\fun{\latentstate' \mid \state, \action, \state'} = \probtransitions{\states}\fun{\state'\mid \state, \action}
\end{align*}
The state-action reward function is given by $\indexof{\rewards}{\latentbeliefspace}\fun{\encoder(\sampledot \mid \previousstate, \previousaction, \state), \action} = \indexof{\rewards}{\states}\fun{\state, \action}$.
%
Finally, $\indexof{\labels}{\latentbeliefspace}\fun{\encoder\fun{\sampledot \mid \state, \action, \state'}} = \indexof{\labels}{\states}\fun{\state'}$ since for all $\latentstate' \in \latentstates$, $\encoder\fun{\latentstate' \mid \state, \action, \state'} > 0 \iff \labels_{\scriptscriptstyle\states}\fun{\state'} = \labels_{\scriptscriptstyle\latentstates}\fun{\latentstate'}$.

One can easily show there is a bisimulation \citep{DBLP:journals/ai/GivanDG03} between $\mdp_\states$ and $\mdp_\latentbeliefspace$ (and consequently between $\mdp_\states$ and $\pomdp_\latentstates$):
%via the equivalence relation $\set{\tuple{\state, \belief} \in \states \times \latentbeliefspace \mid \belief = \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state} \text{ for } \previousstate \in \states, \, \previousaction \in \act{\previousstate}}$.
intuitively, $\mdp_\latentbeliefspace$ refines $\mdp_\states$ by recording the last state and action visited.
In the following we show that we can benefits from this link between $\pomdp_\latentstates$ and $\mdp_\states$ to recover some guarantees in $\mdp_\states$ using the underlying MDP $\mdp_\latentstates$ of $\pomdp_\latentstates$.

\smallparagraph{Upper bound guarantees.} Given $\policy \in \mpolicies{\mdp_\latentstates}$, one can recover a finite-memory policy $\policy'\in\policies{\mdp_\states}$ in a natural way using $\encoder$:
for all $\previousstate, \state \in \states$, $\previousaction, \action \in \actions$, $\policy'\fun{\action \mid \previousstate, \previousaction, \state} = \sum_{\latentstate \in \latentstates} \policy\fun{\action \mid \latentstate} \cdot \encoder\fun{\latentstate \mid \previousstate, \previousaction, \state}$.
We say that two such policies are equivalent under relation $\policyequiv$.\todo{G: is this a definition or a claim?}

\begin{theorem}
Let $T \subseteq \atomicprops$, $\discount \in [0, 1]$, $\policy \in \mpolicies{\mdp_\latentstates}$ and $\policy' \in \policies{\mdp_\states}$ such that $\policy \policyequiv \policy'$,
then $\Prob^{\mdp_\latentstates}_{\pi}\fun{\eventually T} \geq \Prob^{\mdp_\states}_{\policy'}\fun{\eventually T}$, and
$\expectmdp{\policy}{\mdp_\latentstates}{\discountedreturn{\discount}} \geq \expectmdp{\policy'}{\mdp_\states}{\discountedreturn{\discount}}$.
\end{theorem}
%
\begin{proof}
The result follows from the fact that the \emph{value function} (giving the optimal expected return) of the underlying MDP of a POMDP is an upper bound on the value function of this POMDP \citep[Theorems~6 and 9]{DBLP:journals/jair/Hauskrecht00}.
Precisely, we fix $\policy$ in $\mdp_\latentstates$.
From policy $\policy$ in $\mdp_\latentstates$, we recover policy $\indexof{\policy}{\latentbeliefspace} \colon \latentbeliefspace \to \distributions{\actions}$ in $\pomdp_\latentstates$ such that $\indexof{\policy}{\latentbeliefspace}\fun{\action \mid \belief} = \sum_{\latentstate \in \latentstates} \policy\fun{\action \mid \latentstate} \cdot \belief\fun{\latentstate}$.
The POMDP $\pomdp_\latentstates$ under $\indexof{\policy}{\latentbeliefspace}$ is itself a POMDP such that the underlying MDP is the Markov Chain induced by $\mdp_\latentstates$ and $\policy$\todo{F: prove that? {\color{red}wrong}},
and the belief MDP is defined by the Markov Chain $\mdp_{\latentbeliefspace, \policy} = \tuple{\latentbeliefspace, \indexof{\transitions}{\latentbeliefspace, {\scriptstyle \policy}}, \indexof{\rewards}{\latentbeliefspace, {\scriptstyle \policy}}, \indexof{\labels}{\latentbeliefspace}, \atomicprops, \encoder^I}$ (we ignore the action space since there is only one enabled action in each state).
The probability transition distribution is defined as follows.
Let $\previousstate, \state, \state' \in \states$, $\previousaction\in\act{\previousstate}, \action \in \act{\state}$,
\begin{align*}
&\probtransitions{\latentbeliefspace, {\scriptstyle\policy}}\fun{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}}\\
& \quad = \sum_{\action^\star \in \act{\state}} \indexof{\policy}{\latentbeliefspace}\fun{\action^\star \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}} \cdot \probtransitions{\latentbeliefspace}\fun{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}, \action^\star}\\
& \quad = \sum_{\action^\star \in \act{\state}} \sum_{\latentstate \in \latentstates} \policy\fun{\action^\star \mid \latentstate} \cdot \encoder\fun{\latentstate \mid \previousstate, \previousaction, \state} \cdot \probtransitions{\latentbeliefspace}\fun{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}, \action^\star}.
\end{align*}
By definition, $\probtransitions{\latentbeliefspace}\fun{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}, \action^\star} = 0$ if $\action^\star \neq \action$. Therefore,
\begin{align*}
\probtransitions{\latentbeliefspace, {\scriptstyle\policy}}&\fun{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}}\\
&= \sum_{\latentstate \in \latentstates} \policy\fun{\action \mid \latentstate} \cdot  \encoder\fun{\latentstate \mid \previousstate, \previousaction, \state} \cdot \probtransitions{\latentbeliefspace}\fun{\encoder\fun{\sampledot \mid \state, \action, \state'} \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}, \action}\\
&= \sum_{\latentstate \in \latentstates} \policy\fun{\action \mid \latentstate} \cdot  \encoder\fun{\latentstate \mid \previousstate, \previousaction, \state} \cdot \probtransitions{\states}\fun{\state' \mid \state, \action}.
\end{align*}
We define the reward function as $\indexof{\rewards}{\latentbeliefspace, {\scriptstyle \policy}} \colon \latentbeliefspace \to \R$ such that \todo{G: are you redefining it or recalling its definition?}
\begin{align*}
\indexof{\rewards}{\latentbeliefspace, {\scriptstyle \policy}}&\fun{\encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}}\\
&= \sum_{\action \in \act{\state}} \indexof{\policy}{\latentbeliefspace}\fun{\action \mid \encoder\fun{\sampledot \mid \previousstate, \previousaction, \state}} \cdot \indexof{\rewards}{\latentbeliefspace}\fun{\encoder\fun{\sampledot\mid\previousstate, \previousaction, \state}, \action}\\
&= \sum_{\action \in \act{\state}} \sum_{\latentstate \in \latentstates} \policy\fun{\action \mid \latentstate} \cdot \encoder\fun{\latentstate \mid \previousstate, \previousaction, \state} \cdot \indexof{\rewards}{\states}\fun{\state, \action}.
\end{align*}
%
On the other hand, in $\mdp_\states$, one can see $\policy'$ as a finite memory policy encoded by a Mealy machine with memory $\states \times \actions$, recording the last $\previousstate \in \states$ and $\previousaction \in \act{\previousstate}$ visited.
By construction, since $\policy \policyequiv \policy'$, the Markov chain induced by $\mdp_\states$ and $\policy'$ is exactly the Markov chain $\mdp_{\latentbeliefspace, \policy}$ modulo the state equivalence relation
$\set{\tuple{\belief, \rightarrow} \in \latentbeliefspace \times \states \times \actions \times \states \mid \belief = \encoder\fun{\sampledot \mid \state, \action, \state'} \text{ and } \rightarrow = \tuple{\state, \action, \state'} \text{ for } \state, \state' \in \states, \action \in \act{\state}}$.

By \cite{DBLP:journals/jair/Hauskrecht00}, we thus have 
$\expectmdp{\policy}{\mdp_\latentstates}{\discountedreturn{\discount}} \geq \expectmdp{\indexof{\policy}{\latentbeliefspace}}{\pomdp_{\latentstates}}{\discountedreturn{\discount}} = \expectmdp{\indexof{\policy}{\latentbeliefspace}}{\mdp_\latentbeliefspace}{\discountedreturn{\discount}} = \expectmdp{\policy'}{\mdp_\states}{\discountedreturn{\discount}}$.
Moreover, one can reduce a reachability objective of the form $\Prob^{\mdp_\latentstates}_{\policy}\fun{\eventually T}$ to an expected (un)discounted return objective of the form $\expectmdp{\policy}{\mdp'_\latentstates}{\discountedreturn{\discount}}$ with $\discount = 1$, in a modified MDP $\mdp'_\latentstates$ where states $t \in \set{\latentstate \in \latentstates \mid \indexof{\labels}{\latentstates}\fun{\latentstate} \cap T \neq \emptyset}$ are made absorbing (i.e., $\transitions'_\latentstates\fun{t, \action, t} = 1$ for all $\action \in \act{t}$), and where each transition has $0$ reward except for transitions entering a state $t$, giving a reward of $1$ \citep{DBLP:journals/lmcs/EtessamiKVY08}.
This yields the result for the reachability objective.
\end{proof}

==> proofs.tex <==
% \todo[inline]{Make sure to reshuffle sections to have the right ordering}
\section{Details on Discrepancy Measures}
Let $P, Q \in
\distributions{\measurableset}$ be probability distributions over $\measurableset$ with density functions $p$ and $q$.

\smallparagraph{Wasserstein.}~The Kantorovich-Rubinstein duality allows formulating the Wasserstein distance between $P$ and $Q$ as
    \[
        %\wassersteindist{\distance}{P}{Q} = \sup_{\tuple{f_1, f_2} \in \Lipschf{\distance}^2} \int_X f_1\fun{x} \, dP\fun{x} + \int_X f_2\fun{y} \, dQ\fun{y}
        \wassersteindist{\distance}{P}{Q} = \sup_{f \in \Lipschf{\distance}} \left|{\expectedsymbol{x \sim P} f\fun{x} - \expectedsymbol{y \sim Q} f\fun{y}}\right|,
    \]
    % where $\Lipschf{\distance}^2 = \set{\tuple{f_1, f_2} \mid f_1\fun{x} + f_2\fun{y} \leq \distance\fun{x, y}}$.
    where $\Lipschf{\distance}$ is the set of 1-Lipschitz functions, i.e.,
    $\Lipschf{\distance} = \set{f : \left|f\fun{x} - f\fun{y}\right| \leq
    \distance\fun{x, y}}$.
    %

\smallparagraph{Total Variation.}~One can reformulate the total variation distance between $P$ and $Q$ as
\begin{align*}
\dtv{P}{Q} ={} & \sup_{A \in \borel{\measurableset}} |P\fun{A} - Q\fun{A}|\\
{}={} & \frac{1}{2} \int_{\measurableset} |p\fun{x} - q\fun{x}|\, dx.
\end{align*}
When $\measurableset$ is continuous, TV might thus give an overly strong measure of the numerical differences across probability distributions to all measurable sets since the distance between two point masses $dx, dy$ is $1$ unless $x = y$ \citep{DBLP:conf/uai/FernsPP05}.

\section{Latent Space Models}\label{appendix:section:latent-space-model}
From now on, fix MDP $\mdp = \mdptuple$ with latent space model $\tuple{\latentmdp, \embed, \embeda}, \, \latentmdp = \latentmdptuple$.
\subsection{DeepMDPs}
In the following, we recall DeepMDPs notions (from \citealt{DBLP:conf/icml/GeladaKBNB19}) that are useful to prove bisimumation distance (Lem.~\ref{lemma:bidistance-embedding}, Lem.~\ref{lemma:bidistance-abstraction-quality}) and value difference bounds (Lem.~\ref{lemma:qvalues-diff-bound}, Lem.~\ref{lem:quality-latent-space}).  

\smallparagraph{Smooth-valuations.}
A policy $\latentpolicy \in \latentmpolicies$ is said to be \emph{$\KV$-($\dtvsymbol$-)smooth-valued} if
$\sup_{\latentstate \in \latentstates} \left| \latentvalues{\latentpolicy}{}{\latentstate}\right| \leq \KV$ and if for all $\latentaction \in \latentactions$, $\sup_{\latentstate \in \latentstates} \left| \latentqvalues{\latentpolicy}{}{\latentstate}{\latentaction} \right| \leq \KV.$
Observe that all policies $\latentpolicy \in \latentmpolicies$ are
$(\nicefrac{\Rmax{\latentpolicy}}{1 - \discount})$-smooth-valued, where $\Rmax{\latentpolicy} = \sup_{\latentstate \in \latentstates} \left| \latentrewards_{\latentpolicy}\fun{\latentstate} \right|$.

\smallparagraph{Lipschitzness.}
%Let $\latentmdp$ be a latent MDP with metric $\distance_\latentstates$,
A policy $\latentpolicy \in \latentmpolicies$ is $\KV$-Lipschitz-valued if for
all $\latentstate_1, \latentstate_2 \in \states$,
\(
    \left|\latentvalues{\latentpolicy}{}{\latentstate_1} - \latentvalues{\latentpolicy}{}{\latentstate_2} \right| \leq \KV\distance_{\latentstates}\fun{\latentstate_1, \latentstate_2}
\)
and for all $\latentaction \in \latentactions$,
\(
    \left|\latentqvalues{\latentpolicy}{}{\latentstate_1}{\latentaction} - \latentqvalues{\latentpolicy}{}{\latentstate_2}{\latentaction} \right| \leq \KV\distance_{\latentstates}\fun{\latentstate_1, \latentstate_2}.
\)
The MDP $\latentmdp$ is \emph{$\langle \KR{\latentpolicy}, \KP{\latentpolicy}\rangle$-Lipschitz} if for all $\latentstate_1, \latentstate_2 \in \latentstates$,
\begin{align*}
    \left|\latentrewards_{\latentpolicy}\fun{\latentstate_1} - \latentrewards_{\latentpolicy}\fun{\latentstate_2}\right| &\leq \KR{\latentpolicy} \distance_{\latentstates}\fun{\latentstate_1, \latentstate_2},\\
    \wassersteindist{\distance_{\latentstates}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{ \latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}} &\leq \KP{\latentpolicy} \distance_{\latentstates}\fun{\latentstate_1, \latentstate_2}.
\end{align*}
Moreover, all latent policies $\latentpolicy \in \latentmpolicies$ with $\KP{\latentpolicy} \leq \frac{1}{\discount}$ are $(\nicefrac{\KR{\latentpolicy}}{1 - \discount
\KP{\latentpolicy}})$-Lipschitz-valued \citep[Lem.~1]{DBLP:conf/icml/GeladaKBNB19}.
In the discrete setting, we replace the Wasserstein term by TV and we omit the $\distance_{\latentstates}$ terms.

\subsection{Bounded Bisimulation Distance}
\begin{lemma}\label{lemma:bidistance-embedding}
Let $\latentpolicy \in \latentmpolicies$, assume $\latentmdp$ is discrete and $\langle\KR{\latentpolicy}, \KP{\latentpolicy}\rangle$-Lipschitz.
Then, given the induced stationary distribution $\stationary{\latentpolicy}$ in $\mdp$,
\begin{align*}
    % \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}} \leq  \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \localtransitionloss{\stationary{\latentpolicy}} \frac{\fun{\KR{\latentpolicy} \cdot  \condition{\set{\rewards}}\fun{\varphi} + \discount \cdot \condition{\set{\labels}}\fun{\varphi}}}{1 - \discount \fun{\KP{\latentpolicy}\condition{\set{\rewards}}\fun{\varphi} + \condition{\set{\labels}}\fun{\varphi}}}.
    \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\rewards}_{\latentpolicy}\fun{\state, \embed\fun{\state}} & \leq  \localrewardloss{\stationary{\latentpolicy}} + \discount \localtransitionloss{\stationary{\latentpolicy}} \frac{\KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}, \\
    \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\labels}_{\latentpolicy}\fun{\state, \embed\fun{\state}} & \leq \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount}.
\end{align*}
\end{lemma}
\begin{proof}
% Let us first state a property derived from Wasserstein: let $\distance_1, \distance_2 \in \tilde{P}_\measurableset$ such that $\distance_1\fun{x, y} \leq K \distance_2\fun{x, y}$ for all $x, y \in \measurableset$ and some $K \in \R_{\geq 0}$, then for all $P, Q \in \distributions{\measurableset}$, $\wassersteindist{\distance_1}{P}{Q} \leq K \wassersteindist{\distance_2}{P}{Q}$.
% A proof of the statement is provided by \citealp[Lemma~A.4]{DBLP:conf/icml/GeladaKBNB19}, where they showed that a Lipschitz norm of $\bidistance_{\latentpolicy}^{\rewards}$ in $\latentstates$ is given by $\frac{(1 - \discount) \KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}$.
% Let $=_{\labels}$ be the relation $\set{\latentstate_1, \latentstate_2 \mid \labels\fun{\latentstate_1} = \labels\fun{\latentstate_2}} \subseteq \latentstates^2$, we similarly show that $\bidistance^{\labels}_{\latentpolicy}\fun{\latentstate_1, \latentstate_2} \leq \discount \KP{\latentpolicy}$ whenever $\latentstate_1 =_{\labels} \latentstate_2$.
% \cite{DBLP:conf/fossacs/ChenBW12} showed that the sequence given by $\bidistance^{\labels}_{\latentpolicy, 0}\fun{\latentstate_1, \latentstate_2} = \condition{\neq_{\labels}}$ and $\bidistance^{\labels}_{\latentpolicy, n + 1} = \Delta(\bidistance^{\labels}_{\latentpolicy, n})$ converges to $\bidistance^{\labels}_{\latentpolicy}$ as $n \to \infty$.
% Let $K_n = \sup_{\latentstate_1 =_{\labels} \latentstate_2} \bidistance^{\labels}_{\latentpolicy, n}$ for $n \geq 1$.
% When $n = 1$, we have
% \begin{align*}
%     K_1 &= \sup_{\latentstate_1 =_{\labels} \latentstate_2} \discount \wassersteindist{\condition{\neq_{\labels}}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}} \\
%     & \leq \discount \sup_{\latentstate_1 =_{\labels} \latentstate_2} \wassersteindist{\condition{\neq}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}} \tag{by the property stated above} \\ % \tag{$\forall \latentstate_1, \latentstate_2 \in \latentstates$, $\condition{\neq_{\labels}}\fun{\latentstate_1, \latentstate_2} \leq \condition{\neq}\fun{\latentstate_1, \latentstate_2}$} \\
%     & \leq \discount \sup_{\latentstate_1 \neq \latentstate_2} \dtv{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}} \\
%     & \leq \discount \KP{\latentpolicy}
% \end{align*}
% Assume $K_n \leq \discount \KP{\latentpolicy}$ for $n \geq 1$, then
% \begin{align*}
%     K_{n + 1} &= \discount \sup_{\latentstate_1 =_{\labels} \latentstate_2} \wassersteindist{\bidistance^{\labels}_{\latentpolicy, n}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}} \\
%     &\leq \discount \sup_{\latentstate_1 \neq \latentstate_2} \discount \KP{\latentpolicy} \wassersteindist{\condition{\neq}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}} \tag{by the property stated above} \\
%     &= \discount^2 \KP{\latentpolicy} \sup_{\latentstate_1 \neq \latentstate_2} \dtv{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_1}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \latentstate_2}}
%     \leq (\discount \KP{\latentpolicy})^2
%     \leq \discount \KP{\latentpolicy},
% \end{align*}
% which yields the desired upper bound.
% Let $K^{\rewards} = \frac{(1 - \discount) \KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}$ and $K^{\labels} = \discount \KP{\latentpolicy}$, the Wasserstein property stated above allows us to derive
% \begin{align*}
%     &\expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}{\wassersteindist{\bidistance^{\varphi}_{\latentpolicy}}{\embed\probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}}\\
%     \leq& \expected{\state, \latentaction \sim \stationary{\latentpolicy}}{K^{\varphi} \wassersteindist{\condition{\neq}}{\embed\probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}} \\
%     \leq& K^{\varphi} \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}\dtv{\embed\probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} \\
%     \leq& K^{\varphi} \localtransitionloss{\stationary{\latentpolicy}}.
% \end{align*}
\citet[Lemma~A.4]{DBLP:conf/icml/GeladaKBNB19} showed that $\bidistance_{\latentpolicy}^{\rewards}$ is $\frac{(1 - \discount) \KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}$-Lipschitz in $\latentstates$, whereas $\bidistance_{\latentpolicy}^{\labels}$ is $1$-Lipschitz since it assigns a maximal distance of one whenever states have different labels.
Let $K_{\rewards} = \frac{(1 - \discount) \KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}$, $K_{\labels} = 1$ and $\varphi \in \set{\rewards, \labels}$, this allows us deriving the following inequality:
\begin{align*}
    &\expectedsymbol{\state \sim \stationary{\latentpolicy}}{\wassersteindist{\bidistance^{\varphi}_{\latentpolicy}}{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}}} \\
    =& \expected{\state \sim \stationary{\latentpolicy}}{\inf_{\coupling \in \couplings{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}}} \sum_{\latentstate_1, \latentstate_2 \in \states} \bidistance^{\varphi}_{\latentpolicy}\fun{\latentstate_1, \latentstate_2} \coupling\fun{\latentstate_1, \latentstate_2}} \\
    \leq& \expected{\state \sim \stationary{\latentpolicy}}{ \inf_{\coupling \in \couplings{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}}} \sum_{\latentstate_1, \latentstate_2 \in \states}  K_{\varphi} \condition{\neq}\fun{\latentstate_1, \latentstate_2} \coupling\fun{\latentstate_1, \latentstate_2}} \tag{$\bidistance^{\varphi}_{\latentpolicy}$ is $K_{\varphi}$-Lipschitz in $\latentstates$} \\
    =& K_{\varphi} \expected{\state \sim \stationary{\latentpolicy}}{ \inf_{\coupling \in \couplings{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}}} \sum_{\latentstate_1 \neq \latentstate_2} \coupling\fun{\latentstate_1, \latentstate_2}} \\
    =&  K_{\varphi} \expectedsymbol{\state \sim \stationary{\latentpolicy}}{\dtv{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}}} \tag{by definition of TV; TV coincides with $\wassersteinsymbol{\condition{\neq}}$} \\
    =&  K_{\varphi} \expected{\state \sim \stationary{\latentpolicy}}{\frac{1}{2} \sum_{\latentstate' \in \latentstates} \left|\embed\probtransitions_{\latentpolicy}\fun{\latentstate' \mid \state} - \latentprobtransitions_{\latentpolicy}\fun{\latentstate' \mid \embed\fun{\state}} \right|} \\
     =&  K_{\varphi} \expected{\state \sim \stationary{\latentpolicy}}{\frac{1}{2} \sum_{\latentstate' \in \latentstates} \left|\expectedsymbol{\latentaction \sim \latentpolicy\fun{\sampledot \mid \state}}\embed\probtransitions\fun{\latentstate' \mid \state, \latentaction} - \expectedsymbol{\latentaction \sim \latentpolicy\fun{\sampledot \mid \state}}\latentprobtransitions\fun{\latentstate' \mid \embed\fun{\state}, \latentaction} \right|} \\
     =&  K_{\varphi} \expected{\state \sim \stationary{\latentpolicy}}{\frac{1}{2} \sum_{\latentstate' \in \latentstates} \left|\expectedsymbol{\latentaction \sim \latentpolicy\fun{\sampledot \mid \state}} \fun{\embed\probtransitions\fun{\latentstate' \mid \state, \latentaction} - \latentprobtransitions\fun{\latentstate' \mid \embed\fun{\state}, \latentaction}} \right|} \\
     \leq& K_{\varphi} \expectedsymbol{\state \sim \stationary{\latentpolicy}}\expected{\latentaction \sim \latentpolicy\fun{\sampledot \mid \state}}{\frac{1}{2} \sum_{\latentstate' \in \latentstates}  \left| \embed\probtransitions\fun{\latentstate' \mid \state, \latentaction} - \latentprobtransitions\fun{\latentstate' \mid \embed\fun{\state}, \latentaction} \right|} \tag{Jensen's  inequality} \\
     \leq& K_\varphi \localtransitionloss{\stationary{\latentpolicy}}.
\end{align*}
Then,
\begin{align*}
    &\expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}} \\
    =& \expected{\state \sim \stationary{\latentpolicy}}{\fun{1 - \discount} \left| \rewards_{\latentpolicy}\fun{\state} - \latentrewards_{\latentpolicy}\fun{\embed\fun{\state}} \right| \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \wassersteindist{\bidistance_{\latentpolicy}^{\varphi}}{\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}} } \tag{$\labels\fun{\state} = \labels\fun{\embed\fun{\state}}$ by Assumption~\ref{assumption:labeling}} \\
    \leq& \fun{1 - \discount} \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \expected{\state \sim \stationary{\latentpolicy}}{ \wassersteindist{\bidistance_{\latentpolicy}^{\varphi}}{\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}} } \\
    \leq& \fun{1 - \discount} \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} \\
    &+ \discount \expected{\state \sim \stationary{\latentpolicy}}{ \wassersteindist{\bidistance_{\latentpolicy}^{\varphi}}{\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid {\state}}} + \wassersteindist{\bidistance_{\latentpolicy}^{\varphi}}{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\latentpolicy}\fun{\sampledot \mid \embed\fun{\state}}} } \tag{triangular inequality} \\
    \leq& \fun{1 - \discount} \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount K_\varphi \localtransitionloss{\stationary{\latentpolicy}} + \discount \expectedsymbol{\state \sim \stationary{\latentpolicy}}{ \wassersteindist{\bidistance_{\latentpolicy}^{\varphi}}{\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid {\state}}} } \tag{by the inequality derived above} \\
    \leq& \fun{1 - \discount} \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount K_\varphi \localtransitionloss{\stationary{\latentpolicy}} + \discount \expectedsymbol{\state \sim \stationary{\latentpolicy}}{ \bidistance_{\latentpolicy}^{\varphi}\fun{\state, \embed\fun{\state}} }.
\end{align*}
To see how we pass from the penultimate to the last line, recall that 
\[\expectedsymbol{\state \sim \stationary{\latentpolicy}}\wassersteindist{\bidistance_{\latentpolicy}^{\varphi}}{\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{\embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid {\state}}} = \expectedsymbol{\state \sim \stationary{\latentpolicy}} \sup_{f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}} \left| \expectedsymbol{\state' \sim \probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\state'}} - \expectedsymbol{\latentstate' \sim \embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\latentstate'}} \right|,\]
where \[\Lipschf{\bidistance^{\varphi}_{\latentpolicy}} = \set{f \colon \states \uplus \latentstates \to \R : \left| f\fun{\state_1^\star} - f\fun{\state_2^{\star}} \right| \leq  \bidistance^{\varphi}_{\latentpolicy}\fun{\state_1^{\star}, \state_2^{\star}}}.\]
%Take $f^{\star}_s = \sup_{f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}} \left| \expectedsymbol{\state' \sim \probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\state'}} - \expectedsymbol{\latentstate' \sim \embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\latentstate'}} \right|$ for $\state \in \states$, then we have
Then, we have
\begin{align*}
    &\expectedsymbol{\state \sim \stationary{\latentpolicy}} \sup_{f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}} \left| \expectedsymbol{\state' \sim \probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\state'}} - \expectedsymbol{\latentstate' \sim \embed\probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\latentstate'}} \right| \\
    =& \expectedsymbol{\state \sim \stationary{\latentpolicy}} \sup_{f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}} \left| \expectedsymbol{\state' \sim \probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\state'}} - \expectedsymbol{\state' \sim \probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}{f\fun{\embed\fun{\state'}}} \right| \\
    =& \expectedsymbol{\state \sim \stationary{\latentpolicy}} \sup_{f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}} \left| \expectedsymbol{\state' \sim \probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}}\fun{f\fun{\state'} - f\fun{\embed\fun{\state'}}} \right| \\
    \leq& \expectedsymbol{\state \sim \stationary{\latentpolicy}} \expectedsymbol{\state' \sim \probtransitions_{\latentpolicy}\fun{\sampledot \mid \state}} \sup_{f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}} \left| {f\fun{\state'} - f\fun{\embed\fun{\state'}}} \right| \\
    =& \expectedsymbol{\state \sim \stationary{\latentpolicy}} \sup_{f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}} \left| {f\fun{\state} - f\fun{\embed\fun{\state}}} \right| \tag{by the stationary property} \\
    \leq& \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}} \tag{since $f \in \Lipschf{\bidistance^{\varphi}_{\latentpolicy}}$}.
\end{align*}
This finally yields 
\begin{align*}
     (1 - \discount) {\expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}}} &\leq \fun{1 - \discount} \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \localtransitionloss{\stationary{\latentpolicy}} K_\varphi \\
    \equiv  \expectedsymbol{\state \sim \stationary{\latentpolicy}} \bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}} &\leq \localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \localtransitionloss{\stationary{\latentpolicy}} \frac{ K_\varphi }{1 - \discount}.
\end{align*}
\end{proof}

\subsection{Abstraction Quality as Bounded Bisimulation Distance}
\begin{lemma}\label{lemma:bidistance-abstraction-quality}
Let $\latentpolicy \in \latentmpolicies$, assume $\latentmdp$ is discrete and $\langle\KR{\latentpolicy}, \KP{\latentpolicy}\rangle$-Lipschitz.
Let $\stationary{\latentpolicy}$ be the stationary distribution of $\mdp$ induced by $\latentpolicy$.
Then, for any pair of states $\state_1, \state_2 \in \states$ such that $\embed\fun{\state_1} = \embed\fun{\state_2}$,
\begin{align*}
    \bidistance^{\rewards}_{\latentpolicy}\fun{\state_1, \state_2} \leq& \left[\localrewardloss{\stationary{\latentpolicy}} + \frac{
    \discount \localtransitionloss{\stationary{\latentpolicy}} \KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}\right] \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} + \stationary{\latentpolicy}^{-1}\fun{\state_2}}, \\
    \bidistance^{\labels}_{\latentpolicy}\fun{\state_1, \state_2} \leq&  \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount} \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} + \stationary{\latentpolicy}^{-1}\fun{\state_2}}.
\end{align*}
\end{lemma}
\begin{proof}
Let $K_{\rewards} = \frac{(1 - \discount) \KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}$, $K_{\labels} = 1$, and $\varphi \in \set{\rewards, \labels}$.
We use the fact that $\bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}} \leq \stationary{\latentpolicy}^{-1}\fun{\state} \expectedsymbol{\state \sim \stationary{\latentpolicy}}{\bidistance^{\varphi}_{\latentpolicy}\fun{\state, \embed\fun{\state}}}$ for all $\state \in \states$.
Then, we have
\begin{align*}
    &\bidistance^{\varphi}_{\latentpolicy}\fun{\state_1, \state_2}\\
    \leq& \bidistance^{\varphi}_{\latentpolicy}\fun{\state_1, \embed\fun{\state_1}} + \bidistance^{\varphi}_{\latentpolicy}\fun{\embed\fun{\state_1}, \embed\fun{\state_2}} + \bidistance^{\varphi}_{\latentpolicy}\fun{\embed\fun{\state_2}, \state_2} \tag{triangular inequality} \\
    \leq& \stationary{\latentpolicy}^{-1}\fun{\state_1} \expectedsymbol{\state \sim \stationary{\latentpolicy}}{\bidistance^{\varphi}_{\latentpolicy}\fun{\state_1, \embed\fun{\state_1}}} + \stationary{\latentpolicy}^{-1}\fun{\state_2} \expectedsymbol{\state \sim \stationary{\latentpolicy}}{\bidistance^{\varphi}_{\latentpolicy}\fun{\state_2, \embed\fun{\state_2}}} + \bidistance^{\varphi}_{\latentpolicy}\fun{\embed\fun{\state_1}, \embed\fun{\state_2}} \\
    \leq& \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} + \stationary{\latentpolicy}^{-1}\fun{\state_2}} \fun{\localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \localtransitionloss{\stationary{\latentpolicy}} \frac{ K_\varphi }{1 - \discount}} + \bidistance^{\varphi}_{\latentpolicy}\fun{\embed\fun{\state_1}, \embed\fun{\state_2}} \tag{Lemma~\ref{lemma:bidistance-embedding}} \\
    =& \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} + \stationary{\latentpolicy}^{-1}\fun{\state_2}} \fun{\localrewardloss{\stationary{\latentpolicy}} \cdot \condition{\set{\rewards}}\fun{\varphi} + \discount \localtransitionloss{\stationary{\latentpolicy}} \frac{ K_\varphi }{1 - \discount}}. \tag{$\embed\fun{\state_1} = \embed\fun{\state_2}$ by assumption}
\end{align*}
\end{proof}

\subsection{Value Difference Bound}
\begin{lemma}\label{lemma:qvalues-diff-bound}
    Let $\latentpolicy \in \latentmpolicies$ and assume $\latentmdp$ is discrete and $\langle \KR{\latentpolicy}, \KP{\latentpolicy} \rangle$-Lipschitz.
    Let $\labelset{C}, \labelset{T} \subseteq \atomicprops$, $\varphi \in \set{\until{\labelset{C}}{\labelset{T}}, \eventually \labelset{T}}$ and $\KV = \min\fun{\nicefrac{\Rmax{\latentpolicy}}{1 - \discount}, \nicefrac{\KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}}$.
    Then, given the induced stationary distribution $\stationary{\latentpolicy}$ in $\mdp$,
    \begin{align*}
        \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{}{\embed\fun{\state}}{\latentaction} \right| & \leq \frac{\localrewardloss{\stationary{\latentpolicy}} + \discount \KV \localtransitionloss{\stationary{\latentpolicy}}}{1 - \gamma}, \\ %\tag{\citet{DBLP:conf/icml/GeladaKBNB19}} \\
        \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| & \leq \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount}.
    \end{align*}
\end{lemma}
%
\begin{proof}
The first result for discounted return follows directly from \citep{DBLP:conf/icml/GeladaKBNB19}.
The choice of $\KV$ is derived from the fact that $\KP{\latentpolicy} \leq \frac{1}{\discount}$ since $\latentmdp$ is discrete:
$\dtvsymbol$ is bounded by one as well as the diameter of $\latentstates$, equipped with the discrete metric.
For the reachability cases, first observe that $\qvalues{\latentpolicy}{\varphi}{\state}{\sampledot} = 1$ when $\state \in \getstates{\labelset{T}} \subseteq \states$ and $\latentqvalues{\latentpolicy}{\varphi}{\latentstate}{\sampledot} = 1$ when $\latentstate \in \getstates{\labelset{T}} \subseteq \latentstates$.
Moreover, if $\varphi = \until{\labelset{C}}{\labelset{T}}$, $\qvalues{\latentpolicy}{\varphi}{\state}{\sampledot} = 0$ when $\state \in \getstates{\labelset{\neg C}} \subseteq \states$ and $\latentqvalues{\latentpolicy}{\varphi}{\latentstate}{\sampledot} = 0$ when $\latentstate \in \getstates{\labelset{\neg C}} \subseteq \latentstates$.
By Assumption~\ref{assumption:labeling}, $\state \in \getstates{\neg \labelset{C}} \cup \getstates{\labelset{T}}$ implies that the value difference is zero since the labels of each state and those of its latent abstraction are the same. 
Therefore, let $\mathbb{I}$ be $\condition{\getstates{\labelset{C}} \cap \getstates{\neg \labelset{T}}}$ if $\varphi = \until{\labelset{C}}{\labelset{T}}$ and $\condition{\getstates{\neg \labelset{T}}}$ if $\varphi = \eventually \labelset{T}$,
\begin{align*}
    & \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| \\
    =& \expected{\state, \latentaction \sim \stationary{\latentpolicy}}{ \mathbb{I}\fun{\state} \left| \expected{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\discount \values{\latentpolicy}{\varphi}{\state'}} - \expected{\latentstate' \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}{\discount \latentvalues{\latentpolicy}{\varphi}{\latentstate'}} \right|} \\
    \leq& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\values{\latentpolicy}{\varphi}{\state'}} - \expectedsymbol{\latentstate' \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}{\latentvalues{\latentpolicy}{\varphi}{\latentstate'}}  \right| \\
    \leq& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \expected{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\values{\latentpolicy}{\varphi}{\state'} - \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}}} + \expectedsymbol{}_{\substack{\latentstate' \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction} \\ \state' \sim \probtransitions\fun{\sampledot \mid \state, \action}}}\left[{\latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}} - \latentvalues{\latentpolicy}{\varphi}{\latentstate'}}\right] \right| \\
    \leq& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \expected{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\values{\latentpolicy}{\varphi}{\state'} - \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}}} \right| + \discount  \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left|\expectedsymbol{}_{\substack{\latentstate' \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction} \\ \state' \sim \probtransitions\fun{\sampledot \mid \state, \action}}}\left[{\latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}} - \latentvalues{\latentpolicy}{\varphi}{\latentstate'}}\right] \right| \tag{triangular inequality} \\
    \leq& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \expected{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\values{\latentpolicy}{\varphi}{\state'} - \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}}} \right| \\
    & + \discount  \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left|\expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}} - \expectedsymbol{\latentstate' \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}\latentvalues{\latentpolicy}{\varphi}{\latentstate'}} \right| \\
    \leq& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \expected{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\values{\latentpolicy}{\varphi}{\state'} - \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}}} \right| + \discount  \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \wassersteindist{\condition{\neq}}{\embed\probtransitions\fun{\sampledot\mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} \tag{by definition of the Wasserstein dual} \\
    \leq& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \expected{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{\values{\latentpolicy}{\varphi}{\state'} - \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}}} \right| + \discount \localtransitionloss{\stationary{\latentpolicy}} \\
    \leq& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}} \left|\values{\latentpolicy}{\varphi}{\state'} - \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state'}} \right| + \discount \localtransitionloss{\stationary{\latentpolicy}} \tag{Jensen's inequality} \\
    \leq& \discount \expectedsymbol{\state \sim \stationary{\latentpolicy}} \left|\values{\latentpolicy}{\varphi}{\state} - \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state}} \right| + \discount \localtransitionloss{\stationary{\latentpolicy}} \tag{by the stationnary property} \\
    =& \discount \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left|\qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| + \discount \localtransitionloss{\stationary{\latentpolicy}}
\end{align*}
Therefore,
\begin{align*}
    (1 - \discount) \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left|\qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| &\leq \discount \localtransitionloss{\stationary{\latentpolicy}}, \text{ i.e.},\\
    \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left|\qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| &\leq \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount}
\end{align*}
\end{proof}

\subsection{Abstraction Quality as Value Difference Bound}
\begin{lemma}\label{lem:quality-latent-space}
    Let $\latentpolicy \in \latentmpolicies$ and assume $\latentmdp$ is discrete and $\langle \KR{\latentpolicy}, \KP{\latentpolicy} \rangle$-Lipschitz.
    Let $\labelset{C}, \labelset{T} \subseteq \atomicprops$, $\varphi \in \set{\until{\labelset{C}}{\labelset{T}}, \eventually \labelset{T}}$, $\KV = \min\fun{\nicefrac{\Rmax{\latentpolicy}}{1 - \discount}, \nicefrac{\KR{\latentpolicy}}{1 - \discount \KP{\latentpolicy}}}$, and $\stationary{\latentpolicy}$ be the induced stationary distribution in $\mdp$.
    Then, for any pair of states $\state_1, \state_2 \in \states$ such that $\embed\fun{\state_1} = \embed\fun{\state_2}$,
    \begin{align*}
      \left| \values{\latentpolicy}{}{\state_1} {-}
      \values{\latentpolicy}{}{\state_2} \right| &\leq
      \frac{\localrewardloss{\stationary{\latentpolicy}} {+} \discount \KV
      \localtransitionloss{\stationary{\stationary{\latentpolicy}}}}{1 {-}
      \discount} \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} {+}
      \stationary{\latentpolicy}^{-1}\fun{\state_2}},\\
      %
      \left| \values{\latentpolicy}{\varphi}{\state_1} {-}
      \values{\latentpolicy}{\varphi}{\state_2} \right| &\leq \frac{\discount
      \localtransitionloss{\stationary{\latentpolicy}}}{1 {-} \discount}
      \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} {+}
      \stationary{\latentpolicy}^{-1}\fun{\state_2}}.
    \end{align*}
\end{lemma}
\begin{proof}
    The discounted return case follows directly from \citet{DBLP:conf/icml/GeladaKBNB19} and Lemma~\ref{lemma:qvalues-diff-bound}.
    For the reachability cases, we similarly use the fact that $\left| \values{\latentpolicy}{\varphi}{\state} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state}} \right| \leq \stationary{\latentpolicy}^{-1}\fun{\state} \expectedsymbol{\state \sim \stationary{\latentpolicy}}\left| \values{\latentpolicy}{\varphi}{\state} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state}} \right|$, which gives us
    \begin{align*}
        & \left| \values{\latentpolicy}{\varphi}{\state_1} -  \values{\latentpolicy}{\varphi}{\state_2} \right| \\
        =& \left| \values{\latentpolicy}{\varphi}{\state_1} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_1}}  +  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_1}} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_2}}  +  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_2}} - \values{\latentpolicy}{\varphi}{\state_2} \right|\\
        \leq& \left| \values{\latentpolicy}{\varphi}{\state_1} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_1}} \right| + \left| \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_1}} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_2}} \right| + \left| \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_2}} - \values{\latentpolicy}{\varphi}{\state_2} \right| \tag{triangular inequality} \\
        \leq& \stationary{\latentpolicy}^{-1}\fun{\state_1} \expectedsymbol{\state \sim \stationary{\latentpolicy}} \left| \values{\latentpolicy}{\varphi}{\state_1} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_1}} \right| + \left| \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_1}} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_2}} \right| \\
        & + \stationary{\latentpolicy}^{-1}\fun{\state_2} \expectedsymbol{\state \sim \stationary{\latentpolicy}} \left| \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_2}} - \values{\latentpolicy}{\varphi}{\state_2} \right| \\
        =& \stationary{\latentpolicy}^{-1}\fun{\state_1} \expectedsymbol{\state \sim \stationary{\latentpolicy}} \left| \values{\latentpolicy}{\varphi}{\state_1} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_1}} \right| + \stationary{\latentpolicy}^{-1}\fun{\state_2} \expectedsymbol{\state \sim \stationary{\latentpolicy}} \left| \values{\latentpolicy}{\varphi}{\state_2} -  \latentvalues{\latentpolicy}{\varphi}{\embed\fun{\state_2}} \right| \tag{$\embed\fun{\state_1} = \embed\fun{\state_2}$ by assumption} \\
        \leq& \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount} \fun{\stationary{\latentpolicy}^{-1}\fun{\state_1} + \stationary{\latentpolicy}^{-1}\fun{\state_2}} \tag{by Lemma~\ref{lemma:qvalues-diff-bound}}
    \end{align*}
\end{proof}
\subsection{Transition-reward function}
In general RL environments, it is quite common for rewards to be generated from a reward function defined over transitions rather than over state-action pairs., i.e., $\rewards \colon \states \times \actions \times \states$.
In that case, we have $\rewards\fun{\state, \action} = \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \action}}{\rewards\fun{\state, \action, \state'}}$.
Taking transition-rewards into account, we set up an upper bound on $\localrewardloss{\stationary{\latentpolicy}}$ that can be efficiently estimated from samples (using Lemma~\ref{lemma:pac-loss}).
\begin{lemma}
Let $\stationary{\latentpolicy}$ be a stationary distribution of $\mdp$ under $\latentpolicy \in \latentmpolicies$, then
\begin{align*}
    &\localrewardloss{\stationary{\latentpolicy}} \leq \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}\left| \rewards\fun{\state, \latentaction, \state'} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right| = \localrewardlossupper{\stationary{\latentpolicy}}.
\end{align*}
\end{lemma}
\begin{proof}
The upper bound $\localrewardlossupper{\stationary{\latentpolicy}}$ on the local reward loss is given as follows:
\begin{align*}
    & \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}\left| \rewards\fun{\state, \latentaction} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right| \\
    =& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}\left| \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}\rewards\fun{\state, \latentaction, \state'} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right| \\
    \leq& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}} \left|\rewards\fun{\state, \latentaction, \state'} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right| \tag{Jensen's inequality}\\
    =& \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}} \left|\rewards\fun{\state, \latentaction, \state'} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right|
\end{align*}
\end{proof}
This ensures Lem.~\ref{lemma:pac-loss} and Thm.~\ref{thm:pac-qvaluedif} to remain valid by approximating $\localrewardlossupper{\stationary{\latentpolicy}}$ instead of $\localrewardloss{\stationary{\latentpolicy}}$.

\subsection{Local Transition Loss Upper Bound}
Recall that to deal with general MDPs, we study
an upper bound on $\localtransitionloss{\stationary{\latentpolicy}}$ (namely, $\localtransitionlossupper{\stationary{\latentpolicy}}$) that can be efficiently approximated from samples.
We derive it in the following Lemma.
\begin{lemma}\label{lemma:local-loss-upper-bounds}
Let $\stationary{\latentpolicy}$ be a stationary distribution of $\mdp$ under $\latentpolicy \in \latentmpolicies$, then
\begin{align*}
    %&\localrewardloss{\stationary{\latentpolicy}} \leq \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}\left| \rewards\fun{\state, \latentaction, \state'} - \latentrewards\fun{\embed\fun{\state}, \latentaction} \right| = \localrewardlossupper{\stationary{\latentpolicy}}, \\ %\label{eq:rewardloss-upperbound} \\
    %\wassersteindist{\distance_{\latentstates}}{\embed\stationary{\latentpolicy}}{\latentprobtransitions_{\embed}\stationary{\latentpolicy}} \leq \,
    &\localtransitionloss{\stationary{\latentpolicy}} \leq \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}} \wassersteindist{\distance_{\latentstates}}{\embed\fun{\sampledot \mid \state'}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} = \localtransitionlossupper{\stationary{\latentpolicy}} %\label{eq:transitionloss-bounds}
\end{align*}
where we write $\stationary{\latentpolicy}\fun{\state, \latentaction, \state'}  =  \stationary{\latentpolicy}\fun{\state, \latentaction} \cdot \probtransitions\fun{\state' \mid \state, \latentaction}$
and $\embed\fun{\latentstate \mid \state} = \condition{=}\fun{\embed\fun{\state}, \latentstate}$. %$\embed\stationary{\latentpolicy}\fun{\latentstate} = \expectedsymbol{\state \sim \stationary{\latentpolicy}}{\embed\fun{\latentstate \mid \state}}$, and
% $\latentprobtransitions_\embed\steadystate{\policy}\fun{\latentstate} = \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}{\latentprobtransitions\fun{\latentstate \mid \embed\fun{\state}, \latentaction}}$.
\end{lemma}
\begin{proof}
% We then prove the LHS of the inequality~\ref{eq:transitionloss-bounds}.
% We have 
% \begin{align*}
    % & \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \wassersteindist{\distance_{\latentstates}}{\embed\probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} \\
%     =& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}{\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left| \expectedsymbol{\latentstate_1 \sim \embed\probtransitions\fun{\sampledot \mid \state, \latentaction}} f\fun{\latentstate_1} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right|} \\
%     \geq & {\sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \expectedsymbol{\latentstate_1 \sim \embed\probtransitions\fun{\sampledot \mid \state, \latentaction}} f\fun{\latentstate_1} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right|} \\
%     \geq & {\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left| \expected{\state, \latentaction \sim \stationary{\latentpolicy}}{\expectedsymbol{\latentstate_1 \sim \embed\probtransitions\fun{\sampledot \mid \state, \latentaction}} f\fun{\latentstate_1} - \expectedsymbol{\latentstate_2 \sim  \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2}} \right|} \\
%     =& {\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left|  \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}\, \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}} f\fun{\embed\fun{\state'}} - \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}\,\expectedsymbol{\latentstate_2 \sim  \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right|}\\
%     =& {\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left|  \expectedsymbol{\state \sim \stationary{\latentpolicy}} f\fun{\embed\fun{\state}} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions_{\embed}\stationary{\latentpolicy}} f\fun{\latentstate_2} \right|} \tag{by the stationary property}\\
%     =& {\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left| \expectedsymbol{\latentstate_1 \sim \embed\stationary{\latentpolicy}} f\fun{\latentstate_1} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions_{\embed}\stationary{\latentpolicy}} f\fun{\latentstate_2} \right|} \\
%     =& \wassersteindist{\distance_{\latentstates}}{\embed\stationary{\latentpolicy}}{\latentprobtransitions_{\embed}\stationary{\latentpolicy}}
% \end{align*}
%The RHS inequality, i.e.,
The upper bound $\localtransitionlossupper{\stationary{\latentpolicy}}$ on the local transition loss is obtained as follows.
\begin{align*}
    & \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}{\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left| \expectedsymbol{\latentstate_1 \sim \embed\probtransitions\fun{\sampledot \mid \state, \latentaction}} f\fun{\latentstate_1} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right|} \\
    =& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}{\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left| \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}} f\fun{\embed\fun{\state'}} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right|} \\
    =& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}{\sup_{f \in \Lipschf{\distance_{\latentstates}}} \left| \expected{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}}{f\fun{\embed\fun{\state'}} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2}} \right|} \\
    \leq& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}}\sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}} \left|f\fun{\embed\fun{\state'}} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right| \tag{Jensen's inequality}\\
    \leq& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}} \sup_{f \in \Lipschf{\distance_{\latentstates}}} \left|f\fun{\embed\fun{\state'}} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right| \\
    =& \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}} \sup_{f \in \Lipschf{\distance_{\latentstates}}} \left|\expectedsymbol{\latentstate_1 \sim {\embed\fun{\sampledot \mid \state'}}} f\fun{{\latentstate_1}} - \expectedsymbol{\latentstate_2 \sim \latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}} f\fun{\latentstate_2} \right| \\
    =& \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}} \wassersteindist{\distance_{\latentstates}}{\embed\fun{\sampledot \mid \state'} }{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \latentaction}}
\end{align*}
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:pac-loss}}
\begin{proof}
Since $\mdp$ is ergodic, the agent acts in the BSCC induced by $\latentpolicy$ and each tuple $\tuple{\state_t, \action_t, \reward_t, \state_{t + 1}}$ can be considered to be drawn independently from the stationary distribution $\stationary{\latentpolicy}$ of the BSCC in the limit.
The result follows then from the Hoeffding's bound \citep{10.2307/2282952:hoeffding}:
\begin{itemize}
    \item consider the sequence of independent random variables $\seq{X^\rewards}{T - 1}$ such that \[X^{\rewards}_t = |\reward_t - \latentrewards\fun{\embed\fun{\state_t}, \latentaction_t}| \in \mathopen[0, 1\mathclose],\] then
    $\localrewardlossapprox{\stationary{\latentpolicy}} = \frac{1}{T} \sum_{t=0}^{T-1} X^\rewards_t$ and
    $\Pr\fun{ \left|\localrewardloss{\star} - \localrewardlossapprox{\stationary{\latentpolicy}} \right| \geq \error} \leq \proberror_\rewards$, with $\proberror_\rewards = 2 e^{-2T\error^2}$ and $\localrewardloss{\star} = \localrewardloss{\stationary{\latentpolicy}}$ if $\rewards$ is defined over state-action pairs and $\localrewardloss{\star} = \localrewardlossupper{\stationary{\latentpolicy}}$ if it is defined over transitions.
    \item consider the sequence of random variables $\seq{X^{\probtransitions}}{T - 1}$ such that
    \[
        X^{\probtransitions}_t =  1 - \latentprobtransitions\fun{\embed\fun{\state_{t + 1}} \mid \embed\fun{\state_t}, \latentaction_t} \in \mathopen[0, 1 \mathclose],
    \]
    The latent MDP $\latentmdp$ being discrete, we have
    \begin{align*}
        \localtransitionlossupper{\stationary{\latentpolicy}} & = \expectedsymbol{\state, \latentaction, \state' \sim \stationary{\latentpolicy}} \dtv{\embed\fun{\sampledot \mid \state'}}{\latentprobtransitions\fun{\sampledot \mid \embed\fun{\state}, \action}} \\
        & = \expected{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}{ \frac{1}{2} \sum_{\latentstate' \in \states} \left| \embed\fun{\latentstate' \mid \state'} - \latentprobtransitions\fun{\latentstate' \mid \embed\fun{\state}, \latentaction} \right|} \\
        & = \expected{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}{ \frac{1}{2} \cdot \fun{\fun{1 - \latentprobtransitions\fun{\embed\fun{\state'} \mid \embed\fun{\state}, \latentaction}} + \sum_{\latentstate' \in \states \setminus\set{\embed\fun{\state'}}} \left| 0 - \latentprobtransitions\fun{\latentstate' \mid \embed\fun{\state}, \latentaction} \right|}}
        % \tag{because $\embed\fun{\latentstate' \mid \state'} = \condition{=}\fun{\embed\fun{\state'}, \latentstate'}$}
        \tag{because $\embed\fun{\latentstate' \mid \state'} = 1$ if $ \embed\fun{\state'} = \latentstate'$ and $0$ otherwise.} \\
        & = \expected{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}{ \frac{1}{2} \cdot \fun{\fun{1 - \latentprobtransitions\fun{\embed\fun{\state'} \mid \embed\fun{\state}, \latentaction}} + \sum_{\latentstate' \in \states \setminus\set{\embed\fun{\state'}}} \latentprobtransitions\fun{\latentstate' \mid \embed\fun{\state}, \latentaction}}} \\
        & = \expected{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}{\frac{1}{2} \cdot 2 \cdot \fun{1 - \latentprobtransitions\fun{\embed\fun{\state'} \mid \embed\fun{\state}, \latentaction}}} \\
        & = \expected{\state, \latentaction, \state' \sim \stationary{\latentpolicy}}{1 - \latentprobtransitions\fun{\embed\fun{\state'} \mid \embed\fun{\state}, \latentaction}}
    \end{align*}
    then $\localtransitionlossapprox{\stationary{\latentpolicy}} = \frac{1}{T}\sum_{t = 0}^{T - 1} X^{\probtransitions}_{t}$ and $\Pr\fun{ \left| \localtransitionlossupper{\stationary{\latentpolicy}} - \localtransitionlossapprox{\stationary{\latentpolicy}} \right| \geq \error} \leq \proberror_\probtransitions$, with $\proberror_\probtransitions = 2e^{-2T\error^2}$.
\end{itemize}
Therefore,
\begin{align*}
    & \Pr\fun{\left|\localrewardloss{\star} - \localrewardlossapprox{\stationary{\latentpolicy}} \right| \geq \error \vee \left| \localtransitionlossupper{\stationary{\latentpolicy}} - \localtransitionlossapprox{\stationary{\latentpolicy}} \right| \geq \error} \\
    & \leq \proberror_{\rewards} + \proberror_{\probtransitions} \\
    & = 2 e^{-2 T \error^2} + 2e^{-2 T \error^2} \\
    & = 4 e^{-2T\error^2}.
\end{align*}
We thus consider $\proberror \geq 4e^{-2T\error^2}$, i.e., $\log\fun{\frac{\proberror}{4}} \geq -2T\error^2$ and $T \geq \frac{- \log\fun{\frac{\proberror}{4}}}{2 \error^2}$, which yields
\[ \Pr\fun{\left|\localrewardloss{\star} - \localrewardlossapprox{\stationary{\latentpolicy}} \right| \leq \error \wedge \left| \localtransitionlossupper{\stationary{\latentpolicy}} - \localtransitionlossapprox{\stationary{\latentpolicy}} \right| \leq \error} \geq 1 - \proberror.\]
\end{proof}

\subsection{Proof of Theorem~\ref{thm:pac-qvaluedif}}

\begin{proof}
Let $\error' \in \mathopen]0, 1\mathclose[$ and $T \geq \Big\lceil \frac{- \log\fun{\frac{\proberror}{4}}}{2 \error'^2} \Big\rceil$, then by applying Lemma~\ref{lemma:qvalues-diff-bound} and Lemma~\ref{lemma:pac-loss}, we have
\begin{align*}
    \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{}{\embed\fun{\state}}{\latentaction} \right| & \leq & \frac{\localrewardloss{\stationary{\latentpolicy}} + \discount \KV \localtransitionloss{\stationary{\latentpolicy}}}{1 - \gamma} &\leq \frac{\fun{\localrewardlossapprox{\stationary{\latentpolicy}} + \error'} + \discount \KV \fun{\localtransitionlossapprox{\stationary{\latentpolicy}} + \error'}}{1 - \gamma}, \text{ and} \\ 
    \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy}} \left| \qvalues{\latentpolicy}{\varphi}{\state}{\latentaction} - \latentqvalues{\latentpolicy}{\varphi}{\embed\fun{\state}}{\latentaction} \right| & \leq & \frac{\discount \localtransitionloss{\stationary{\latentpolicy}}}{1 - \discount} \quad \; \quad &\leq \frac{\discount \fun{\localtransitionlossapprox{\stationary{\latentpolicy}} + \error'}}{1 - \discount}
\end{align*}
with probability at least $1 - \proberror$.
To offer an error of at most $\error$, we need
\begin{align*}
    && \frac{\error' + \discount \KV \error'}{1 - \discount} &\leq \error& \\
    &\equiv& \error' + \discount \KV \error' &\leq \error (1 - \discount)& \\
    &\equiv& \error'(1 + \discount \KV) &\leq \error (1 - \discount)& \\
    &\equiv& \error' &\leq \frac{\error (1 - \discount)}{1 + \discount \KV}&
\end{align*}
which yields the result.
\end{proof}

\section{Details on Variational MDPs}
\smallparagraph{ELBO.} In this work, we focus on the case where
$\dklsymbol$ is used as divergence measure.
The goal is thus to optimize $\min_{\decoderparameter}
\dkl{\mdp_{\policy}}{\decoder}$, i.e., maximizing the marginal
log-likelihood of traces of the original MDP $\expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}}$.
Recall that
% \begin{equation}
%     \expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}} 
%     \text{ s.t. }
%     \decoder\fun{\trace} =
%         \begin{cases}
%             \int_{\inftrajectories{\latentmdp_{\decoderparameter}}} \decoder\fun{\trace \mid \seq{\latentstate}{T}} \, d\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentstate}{T}} & \text{if } \latentactions = \actions, \\ 
%             \int_{\inftrajectories{\latentmdp_{\decoderparameter}}} \decoder\fun{\trace \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \, d\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} & \text{else.} 
%         \end{cases} \label{eq:maximum-likelihood}
% \end{equation}
\begin{equation}
    \decoder\fun{\trace} =
            \int_{\inftrajectories{\latentmdp_{{\decoderparameter}}}} \decoder\fun{\trace \mid \seq{\latentvariable}{T}} \, d\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentvariable}{T}} \label{eq:maximum-likelihood2}
\end{equation}
where $\trace = \defaulttrace$, $\latentvariable \in \latentvariables$ such that $\latentvariables = \latentstates$ if $\latentactions = \actions$ and $\latentvariables = \latentstates \times \latentactions$ otherwise,
$\latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\seq{\latentstate}{T}} = \prod_{t = 0}^{T - 1} \latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\latentstate_{t + 1} \mid \latentstate_t}$, and $\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1}} = \prod_{t = 0}^{T - 1} {\latentpolicy_{\decoderparameter}}\fun{\latentaction_t \mid \latentstate_t} \cdot \latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \latentaction_t}$.
%Note that
The dependency of $\trace$ on $\latentvariables$ in Eq.~\ref{eq:maximum-likelihood2}
is made explicit by the law of total probability.

Optimizing $\expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}}$ through Eq.~\ref{eq:maximum-likelihood2} is typically intractable \citep{DBLP:journals/corr/KingmaW13}.
% Intuitively, one may want to make use of \emph{Monte-Carlo sampling methods} to approximate the likelihood of $\trace$ through Eq.~\ref{eq:intractable-latent}
% by generating a finite number of latent sequences $\set{\seq{\latentstate^{\,i}}{T}}_{i=1}^{N}$ from $ \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \seq{\action}{T - 1}}$, and then averaging $\frac{1}{N}\sum_{i = 1}^{N}\decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate^{\,i}}{T}, \seq{\action}{T - 1}}$ to approximate $\decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid  \seq{\action}{T - 1}}$.
% Using such methods amounts to trying to approximate an integration over elements from an infinitely uncountable space with a sum over a finite set of elements from this space, meaning that for most $\seq{\latentstate^{\, i}}{T}$, $\decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate^{\, i}}{T}, \seq{\action}{T - 1}}$ will be close to zero thus contributing almost nothing to our estimates.
To overcome this, we use an encoder $\encoder\fun{\seq{\latentvariable}{T} \mid \trace}$ to approximate the intractable true posterior
%\begin{itemize}
    %\item
    $\decoder\fun{\seq{\latentvariable}{T} \mid \trace} = \decoder\fun{\trace \mid \seq{\latentvariable}{T}} \cdot \nicefrac{{}\latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentvariable}{T}}}{\decoder\fun{\trace}}$. %if $\latentactions = \actions$, and
    %\item
    % $\decoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \mid \trace} = \decoder\fun{\trace \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \cdot \latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} / \decoder\fun{\trace}$ otherwise.
%\end{itemize}
% giving a distribution over sequences $\seq{\latentstate}{T}$ that are likely to produce $\trace$ to estimate the integration of Eq.~\ref{eq:maximum-likelihood}.
Such an encoder can be learned through the following optimization:
\begin{equation}
    %\min_{\encoderparameter, \decoderparameter} \expected{\trace \sim \mdp_\policy}{\divergence{\encoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}}{\decoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}}}
    \min_{\encoderparameter, \decoderparameter} \; \expectedsymbol{\trace \sim \mdp_\policy}{\,\divergence{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{\sampledot \mid \trace}}},}
\end{equation}
where $\divergencesymbol$ denotes a discrepancy measure.
If we let once again $\divergencesymbol$ be $\dklsymbol$, one can set a \emph{lower bound} on the log-likelihood of produced traces,
%on the $\log$-values of Eq.~\ref{eq:maximum-likelihood}
often referred to as \emph{evidence lower bound} (ELBO, \citealp{DBLP:journals/jmlr/HoffmanBWP13}) as follows:
\begin{align*}
    &&& {\dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{\sampledot \mid \trace}}}} \notag \\
    &&= \,& {\expected{\seq{\latentvariable}{T} \sim \encoder\fun{\sampledot \mid \trace}}{\log \encoder\fun{\seq{\latentvariable}{T} \mid \trace} - {\decoder\fun{\seq{\latentvariable}{T} \mid \trace}}}} \notag \\
    && \begin{aligned}
       = \\ \, \\
    \end{aligned} \;& \begin{aligned}
        \expectedsymbol{\seq{\latentvariable}{T} \sim \encoder\fun{\sampledot \mid \trace}}[&\log \encoder\fun{\seq{\latentvariable}{T} \mid \trace} - \log \decoder\fun{\trace \mid \seq{\latentvariable}{T}} - \log \latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\seq{\latentvariable}{T}}] + \log \decoder\fun{\trace}
    \end{aligned} %\tag{Bayes' rule}
    \\
    &\iff&& {\log \decoder\fun{\trace} - \dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{\sampledot \mid \trace}}}} \notag \\
    %&&= & \expectedsymbol{\trace \sim \mdp_\policy}\bigg[\expectedsymbol{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \sim \encoder}[\log \decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}\mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}]  \notag \\
    %&&& \quad\quad\quad\quad - \dkl{\encoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1} \mid \trace}}{\latentprobtransitions_{\decoderparameter}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}}\bigg] \label{eq:ground-action-elbo}
    && \begin{aligned}
        = 
    \end{aligned} \:& \begin{aligned}
        \expectedsymbol{\seq{\latentvariable}{T} \sim \encoder\fun{\sampledot \mid \trace}}[&\log \decoder\fun{\trace \mid \seq{\latentvariable}{T}}  + \log \latentprobtransitions_{\latentpolicy_{ \decoderparameter}}\fun{\seq{\latentvariable}{T}}
        - \log \encoder\fun{\seq{\latentvariable}{T} \mid \trace}]
    \end{aligned} \label{eq:ground-action-elbo}
\end{align*}

\smallparagraph{Behavioral model.} We assume that the behavioral model $\decoder$ allows recovering the latent MDP parameters (i.e., $\latentprobtransitions_\decoderparameter$  $\latentrewards_{\decoderparameter}$ and $\latentlabels_{\decoderparameter}$), by decomposing it into reward and label models, the distilled policy, as well as a generative model $\decoder^{\generative}$ allowing the reconstruction of states and actions.
%, as well as a distillation $\latentpolicy_{\decoderparameter}$ of the policy $\policy$ that allows producing the traces in $\mdp$.
Therefore, states, actions, rewards, and labels are independent given the latent sequence:
\begin{align*}
    &\decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate}{T}}\\
    = & \decoder^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}} \cdot \decoder\fun{\seq{\action}{T - 1}, \seq{\reward}{T - 1} \mid \seq{\latentstate}{T}} \cdot \decoder^{\labels}\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}} \\
    = & \decoder^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}} \cdot 
    \latentpolicy_{\decoderparameter}\fun{\seq{\action}{T - 1} \mid \seq{\latentstate}{T}} \cdot
    \decoder^{\rewards}\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} \cdot  \decoder^{\labels}\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}}, \tag{by the chain rule, $\decoder\fun{\seq{\action}{T - 1}, \seq{\reward}{T - 1} \mid \seq{\latentstate}{T}} = \latentpolicy_{\decoderparameter}\fun{\seq{\action}{T - 1} \mid \seq{\latentstate}{T}} \cdot
    \decoder^{\rewards}\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}}$}  \\
    & \text{and} \\
    &\decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}\\
    = & \decoder^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}} \cdot \decoder^{\generative}\fun{\seq{\action}{T - 1} \mid \seq{\latentstate}{T},  \seq{\latentaction}{T - 1}} \cdot \decoder^{\rewards}\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \cdot \decoder^{\labels}\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}}
\end{align*}

\smallparagraph{Local setting.} We formulate the ELBO in the local setting thanks to the following Lemma.
\begin{lemma}\label{lemma:trace-to-stationary}
Let  $\stationary{\policy}$ be the stationary distribution of $\mdp_\policy$ and $f \colon \states \times \actions \times \images{\rewards} \times \states \to \R$ be a continuous function.
Assume $\states, \actions$ are compact, then % induced by $\policy$, then 
\begin{align*}
    \lim_{T \to \infty} \frac{1}{T} \expected{\trace \sim \mdp_{\policy}[T]}{\sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}} = \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} f\fun{\state, \action, \reward, \state'}
\end{align*}
where $\traces{\mdp}\fun{T}$ denotes the set of traces in $\mdp_{\policy}$ of size $T$, $\mdp_{\policy}[T]$ denotes the distribution over $\traces{\mdp_\policy}\fun{T}$, and $ \stationary{\policy}(\state, \action, \reward, \state') = \stationary{\policy}(\state, \action, \state') \cdot \condition{=}(\reward,  \rewards\fun{\state, \action, \state'})$.
\end{lemma}
\begin{proof}
%Let $\mu_T: \distributions{\states}$, $\mu_T\fun{\state} = \Prob_\policy\fun{\set{\tuple{\seq{\state}{\infty}, \seq{\action}{\infty}} \in \inftrajectories{\mdp_{\policy}} \mid \state_T = \state}}$ be the distribution giving the probability for the agent of being in each particular state of $\mdp_{\policy}$ after exactly $T$ steps. %, and $f \colon \states \times \actions \times \rewards \times \states \to \R$ be a continuous function.
First, observe that
\begin{align*}
    & \expected{\trace \sim \mdp_{\policy}[T]}{\sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}} \\
    =&  \expectedsymbol{\action_0 \sim \policy\fun{\sampledot \mid \sinit}}\expectedsymbol{\state_1 \sim \probtransitions\fun{\sampledot \mid \sinit, \action_0}} \expectedsymbol{\action_1 \sim \policy\fun{\sampledot \mid \state_1}} \cdots \expectedsymbol{\state_T \sim \probtransitions\fun{\sampledot \mid \state_{T - 1}, \action_{T - 1}}} \left[ \sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \rewards\fun{\state_t, \action_t, \state_{t + 1}}, \state_{t + 1}}\right]\\
    =& \sum_{t = 0}^{T - 1} \expectedsymbol{\action_0 \sim \policy\fun{\sampledot \mid \sinit}}\expectedsymbol{\state_1 \sim \probtransitions\fun{\sampledot \mid \sinit, \action_0}} \expectedsymbol{\action_1 \sim \policy\fun{\sampledot \mid \state_1}} \cdots \expectedsymbol{\state_T \sim \probtransitions\fun{\sampledot \mid \state_{T - 1}, \action_{T - 1}}} f\fun{\state_t, \action_t, \rewards\fun{\state_t, \action_t, \state_{t + 1}}, \state_{t + 1}}\\
    =& \sum_{t = 0}^{T - 1} \expectedsymbol{\trace \sim \mdp_{\policy}[t + 1]} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}.
\end{align*}
Second, let $t \in \N, \state, \state' \in \states, \action \in \act{\state},$ and $\reward = \rewards\fun{\state, \action, \state'}$, also observe that
\begin{align*}
    \stationary{\policy}^t\fun{\state \mid \sinit} &= \int_{\traces{\mdp_{\policy}}\fun{t}} \condition{=}\fun{\state_t, \state} \, d\Prob_{\policy}\fun{Cyl\fun{\seq{\state}{t},\seq{\action}{t - 1}}}
    \tag{where $Cyl\fun{\seq{\state}{t}, \seq{\action}{t}} = \set{\tuple{\seq{\state^{\star}}{\infty}, \seq{\action^{\star}}{\infty}} \in \inftrajectories{\mdp_{\policy}} \mid \state^{\star}_{i + 1} = \state_{i + 1}, \action^{\star}_{i} = \action_i \; \forall i \leq t - 1}$} \\
    f\fun{\state, \action, \reward, \state'} \cdot \stationary{\policy}^t\fun{\state \mid \sinit} &=  f\fun{\state, \action, \reward, \state'} \cdot \int_{\traces{\mdp_{\policy}}\fun{t}} \condition{=}\fun{\state_t, \state} \, d\Prob_{\policy}\fun{Cyl\fun{\seq{\state}{t}, \seq{\action}{t - 1}}} \\
    \int_{\states} f\fun{\state, \action, \reward, \state'} \,d\stationary{\policy}^t\fun{\state \mid \sinit} & =  \int_{\states} \int_{\traces{\mdp_{\policy}}\fun{t}} f\fun{\state, \action, \reward, \state'} \cdot \condition{=}\fun{\state_t, \state} \, d\Prob_{\policy}\fun{Cyl\fun{\seq{\state}{t}, \seq{\action}{t - 1}}} \, d\state \\
    & = \int_{\traces{\mdp_{\policy}}\fun{t}} f\fun{\state_t, \action, \reward, \state'} \, d\Prob_{\policy}\fun{Cyl\fun{\seq{\state}{t}, \seq{\action}{t - 1}}}.
\end{align*}
Therefore, we have
\begin{align*}
    & \lim_{T \to \infty} \frac{1}{T} \expected{\trace \sim \mdp_{\policy}[T]}{\sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}} \\
    =& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \expectedsymbol{\trace \sim \mdp_{\policy}[t + 1]} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}} \\
    =& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \int_{\traces{\mdp_{\policy}}\fun{t + 1}} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}} \, d\Prob_\policy\fun{Cyl\fun{\seq{\state}{t + 1}, \seq{\action}{t}}} \\
    =& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \int_{\states} \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\stationary{\policy}^t\fun{\state\mid\sinit} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action} \\
    =& \lim_{T \to \infty} \int_{\states}  \frac{1}{T} \sum_{t = 0}^{T - 1} \stationary{\policy}^t\fun{d\state \mid \sinit}  \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action}.
    %=& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \expectedsymbol{\state \sim \mu_{t}} \expectedsymbol{\action \sim \policy\fun{\sampledot \mid \state}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \action}} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\state
\end{align*}
By definition of $\stationary{\policy}$ and Assumption~\ref{assumption:ergodicity}, $\stationary{\policy}\fun{A} = \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \stationary{\policy}^{t}\fun{A \mid \state}$ for all $\state \in \states$, $A \in \borel{\states}$, i.e., $\frac{1}{T} \sum_{t = 0}^{T - 1} \stationary{\policy}^{t}\fun{A \mid \state}$ weakly converges to $\stationary{\policy}$ (e.g., \citealtAR{DBLP:books/daglib/0020348}).
By Assumption~\ref{assumption:rewards}, the set of images of $\rewards$ is a compact space.
Therefore, $f$ has compact support and by the Portmanteau's Theorem, 
\begin{align*}
    & \lim_{T \to \infty} \int_{\states}  \frac{1}{T} \sum_{t = 0}^{T - 1} \stationary{\policy}^t\fun{d\state \mid \sinit} \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action} \\
    =& \int_{\states} \stationary{\policy}\fun{d\state} \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action} \\
    =& \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} f\fun{\state, \action, \reward, \state'}.
\end{align*}
\end{proof}

%
\begin{corollary}\label{cor:elbo-local}
Let $ \embed\fun{\latentstate, \latentstate' \mid \state, \state'} = \embed\fun{\latentstate \mid \state} \embed\fun{\latentstate' \mid \state'}$, then
\begin{align*}
    & \lim_{T \to \infty} \frac{1}{T} \expectedsymbol{}_{\substack{\trace \sim \mdp_{\policy}[T] \\ \seq{\latentvariable}{T} \sim \encoder\fun{\sampledot \mid \trace}}} \left[\log \decoder\fun{\trace \mid \seq{\latentvariable}{T}} - \dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{ \sampledot \mid \trace}}} \right] \\
    % \begin{aligned}
    % = \\ \, \\ \, \\
    % \end{aligned} & \begin{aligned} \;
    % \lim_{T \to \infty} \frac{1}{T} \expectedsymbol{\trace \sim \mdp_{\policy}[T]} \Bigg[ \sum_{t = 0}^{T - 1} \expectedsymbol{\latentstate_t, \latentstate_{t + 1} \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state_t, \state_{t + 1}}} \big[&{\log \decoder^{\generative}\fun{\state_{t+1} \mid \latentstate_{t + 1}} + \log \decoder^{\rewards}\fun{\reward_{t + 1} \mid \latentstate_t, \action_t}} \\
    % & - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state_{t + 1}}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate_t, \action_t}}\big] \Bigg]
    % \end{aligned} \\
    % --------------------------------------------------------
    % =& \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy}\\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}}\left[{\log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action}} - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot\mid \latentstate, \action}}\right].
    % --------------------------------------------------------
    =&
    \left\lbrace\begin{array}{@{}r@{\quad}l@{}l@{}}
    \displaystyle \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy}\\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}} \big[ \log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \latentpolicy_{\decoderparameter}\fun{\action \mid \latentstate} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action}& \\[-12pt]
    \hfill - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\sampledot\mid \latentstate}} \big]
        & \text{if } \latentactions = \actions, \text{ and} \\[10pt]
    \displaystyle \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy}\\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'} \\ \latentaction \sim \latentembeda_{\encoderparameter}\fun{\sampledot \mid \latentstate, \action}}} \big[ \log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log\embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \latentaction} & \\[-25pt]
    \hfill - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot\mid \latentstate}} \quad \;\, & \\[5pt]
    \hfill - \dkl{\latentembeda_{\encoderparameter}\fun{\sampledot\mid\latentstate, \action}}{\latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \big]
        & \text{otherwise},
    \end{array}
    \right.
\end{align*}
where $\trace = \defaulttrace$, $\seq{\latentvariable}{T} = \seq{\latentstate}{T}$ if $\latentactions = \actions$ and $\seq{\latentvariable}{T} = \tuple{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}$ otherwise.
\end{corollary}
\begin{proof}
Taking 
\[f\fun{\state, \action, \reward, \state'} = \expectedsymbol{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}\big[ g\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentstate'}} \big]\]
with
\begin{align*}
    & g\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentstate'}}\\
    =& 
    \left\lbrace\begin{array}{@{}r@{\quad}l@{}l@{}}
    \log \fun{\decoder^{\generative}\fun{\state' \mid \latentstate'} \cdot \decoder^{\rewards}\fun{\reward \mid \latentstate, \action} \cdot \latentpolicy_{\decoderparameter}\fun{\action \mid \latentstate}} - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\sampledot\mid \latentstate}} & \text{if } \latentactions = \actions, \text{ and} \\[5pt]
    \expectedsymbol{\latentaction \sim \encoder^\actions\fun{\sampledot \mid \latentstate, \action}} \Big[ \log \fun{\decoder^{\generative}\fun{\state' \mid \latentstate'} \cdot \embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction} \cdot \decoder^{\rewards}\fun{\reward \mid \latentstate, \latentaction}} \hfill & \\[3pt]
    - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot\mid \latentstate, \latentaction}} \Big] - \dkl{\latentembeda_{\encoderparameter}\fun{\sampledot\mid\latentstate, \action}}{\latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} & \text{otherwise}
    \end{array}
    \right.
\end{align*}
yields the result.
\end{proof}

\subsection{Latent Distributions}
\smallparagraph{Discrete latent state space.} W.l.o.g., we assume latent states to have a binary representation, we further see each bit as a Bernoulli random variable.
Let $\logit \in \R$ and $\temperature \in \mathopen]0, 1 \mathclose]$, $\latentstate_\temperature \in \mathopen[0, 1\mathclose]$ has a \emph{relaxed Bernoulli distribution} $\latentstate_\temperature \sim \relaxedbernoulli{\logit}{\temperature}$ with logit $\logit$ and temperature parameter $\temperature$ iff
(a) if $l$ is a logistic sample with location parameter $\logit\temperature^{-1}$ and scale parameter $\temperature^{-1}$, i.e., $l \sim \logistic{\logit\temperature^{-1}}{\temperature^{-1}}$, then $\latentstate_\temperature = \sigmoid\fun{l}$, $\sigmoid$ being the \emph{sigmoid} function,
(b) $\lim_{\temperature \to 0} \relaxedbernoulli{\logit}{\temperature} = \bernoulli{\logit}$, meaning $\Prob(\textstyle\lim_{\temperature \to 0} \latentstate_\temperature = 1) = \sigmoid\fun{\logit}$, and
(c) let $p_{\logit, \temperature}$ be the density of $\relaxedbernoulli{\logit}{\temperature}$, then $p_{\logit, \temperature}\fun{\latentstate_\temperature}$ is log-convex in $\latentstate_\temperature$.
Since the logistic distribution belongs to the location-scale family, it is fully reparameterizable, i.e., $l \sim \logistic{\logit\temperature^{-1}}{\temperature^{-1}} \equiv x \sim \logistic{0}{1} \text{ and } l = \frac{\logit + x}{\temperature}$.
In practice, we train $\embed_{\encoderparameter}$ and $\latentprobtransitions_{\decoderparameter}$ to infer and generate $\log_2 |\latentstates|$ logits, and we anneal $\temperature$ to $0$ during training while using Bernoulli distributions for evaluation.
As suggested by \citet{DBLP:conf/iclr/MaddisonMT17}, we use two different temperature parameters and we fixed their initial values to $\temperature_{\embed_{\encoderparameter}} = \nicefrac{2}{3}$ for the encoder distribution and $\temperature_{\probtransitions_{\decoderparameter}} = \nicefrac{1}{2}$ for the latent transition function.

\smallparagraph{Discrete latent action space.} We learn discrete latent distributions for $\encoder^{\actions}$ and $\latentpolicy_{\decoderparameter}$ by learning the logits of continuous relaxation of discrete distributions, through the \emph{Gumbel softmax trick}.
Let $n = |\latentactions|$, and $\latentactions = \set{\latentaction_1, \dots, \latentaction_n}$.
Drawing $\latentaction_i \sim \categorical{\logits}$  from a discrete (categorical) distribution in $\distributions{\latentactions}$ with logits parameter $\logits \in \R^n$ is equivalent to applying an $\argmax$ operator to the sum of \emph{Gumble samples} and these logits, i.e., $i = \argmax_{k} \logits_k - \log\fun{- \log \vect{\epsilon}_k}$, where $\vect{\epsilon} \in \mathopen[0, 1\mathclose]^n$ is a uniform noise.
The sampling operator being fully reparameterizable here, $\argmax$ is however not derivable, preventing the operation to be optimized through gradient descent.
The proposed solution is to replace the $\argmax$ operator by a softmax function with temperature parameter $\temperature \in \mathopen]0, \left(n - 1\right)^{-1}\mathclose]$.

Concretely, $\vect{x} \in \mathopen[0, 1\mathclose]^n$ has a \emph{relaxed discrete distribution} $\vect{x} \sim \relaxedcategorical{\logits}{\temperature}$ with logits $\logits$, temperature parameter $\temperature$ iff
(a) let $\vect{\epsilon} \in [0, 1]^n$ be a uniform noise and $\vect{G}_k = {- \log \fun{- \log \vect{\epsilon}_k}}$, then $\vect{x}_k = {\frac{\exp{\fun{\fun{\logits_k + \vect{G}_k} \temperature^{-1}}}}{\sum_{i = 1}^{n} \exp{\fun{\fun{\logits_i + \vect{G}_i} \lambda^{-1}}}}}$ for each $k \in [n]$,
(b) $\lim_{\temperature \to 0} \relaxedcategorical{\logits}{\temperature} = \categorical{\logits}$, meaning $\Prob(\textstyle\lim_{\temperature \to 0} \vect{x}_k = 1) = \frac{\exp{\logits_k}}{\sum_{i = 1}^{n}\exp{\logits_i}}$,
and (c) let $p_{\logits, \temperature}$ be the density of $\relaxedcategorical{\logits}{\temperature}$, then $p_{\logits, \temperature}\fun{\vx}$ is log-convex in $\vx$.
In practice, we train $\encoder^{\actions}$ and $\latentpolicy_{\decoderparameter}$ to infer and generate logits parameter $\logits$, and we anneal $\temperature$ from $(n - 1)^{-1}$ to $0$ during training while using discrete distributions for evaluation.
Again, as prescribed by \citet{DBLP:conf/iclr/MaddisonMT17}, we use two different temperature parameters, one for $\encoder^{\actions}$ and another one for $\latentpolicy_{\decoderparameter}$.

\subsection{Prioritized Experience Replay}
%\smallparagraph{Experience replay.}~%
Modern RL techniques allow to learn the parameters $\decoderparameter$ of a policy, model, or value function, by processing encountered experiences $\experience$ 
%encountered in the interaction loop 
via a loss function $\loss\fun{\experience, \decoderparameter}$.
If these
%such experiences 
are processed sequentially and discarded after all parameter updates, the latter are strongly correlated and rare events are quickly forgotten.
\emph{Prioritized experience replay buffers} \citep{DBLP:journals/corr/SchaulQAS15} are finite data structures $\replaybuffer$ that allow to overcome both issues by
(i) storing experiences $\experience$ with some assigned priority $p_{\experience}$, and
(ii) producing $\experience \sim \replaybuffer$ according to $P\fun{\experience} = p_\experience^\varsigma / \sum_{\experience' \in \replaybuffer} p_{\experience'}^\varsigma$, $\varsigma \in \mathopen[0, 1\mathclose]$, which allows minimizing $\expected{\experience \sim \replaybuffer}{w_{\experience} \cdot \loss\fun{\experience, \decoderparameter}}$ for \emph{importance sampling weight} $w_\experience > 0$.
%, and
%(iii) removing $\experience$ from $\replaybuffer$ (when full) according to a distribution $Q$.
%In their simpler form, $P = Q$ with $\alpha = 0$ ($P$ and $Q$ are uniform).
%However, experiences drawn from $\replaybuffer$ can be in that case more or less surprising, redundant, or not being useful for the learning process.
The replay buffer $\replaybuffer$ is \emph{uniform} if $\varsigma = 0$.
Otherwise, when $\varsigma > 0$, a bias is introduced because priorities change the real distribution of experiences and consequently the estimates of the expectation of $\loss$.
This bias is alleviated via $w_{\experience} = \fun{|\replaybuffer| \cdot P\fun{\experience}}^{-\omega}$ for each $\experience \in \replaybuffer$, $\omega \in \mathopen[0, 1\mathclose]$, where $\omega = 1$ fully corrects it.

We use prioritized replay buffers to store transitions and sample them when optimizing our loss function, i.e., $\elbo$.
This allows to alleviate the posterior collapse problem, as shown in Figure~\ref{appendix:fig:prioritized-replay}.
We introduced two priority functions, yielding a bucket-based and a loss-based prioritized replay buffer.
In the following, we elaborate how precisely we assign priorities via the loss-based priority function.

\smallparagraph{Loss-based priorities.}~Draw $\tuple{\state, \action, \reward, \state'} \sim \stationary{\policy}$, we aim at assigning $p_{\tuple{\state, \action, \reward, \state'}}$ to its \emph{individual transition loss}, i.e.,
$\loss_{\elbo}$:
for $\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}$, $\latentaction \sim \encoder^\actions\fun{\sampledot \mid \latentstate, \action}$ if $\latentactions \neq \actions$ and $\latentaction = \action$ else,
    \begin{align*}
        & \loss_{\elbo}\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentaction, \latentstate'}} \\
        =&  - \log \decoder^\generative\fun{\state' \mid \latentstate'} - \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \latentaction} - \log \latentpolicy_{\decoderparameter}\fun{\latentaction \mid \latentstate} + \log \embed_{\encoderparameter}\fun{\latentstate' \mid \state'} \\
        & - \condition{=}\fun{\latentactions, \actions} \cdot \log \latentprobtransitions_{\latentpolicy_{\decoderparameter}}\fun{\latentstate' \mid \latentstate} - \condition{\neq}\fun{\latentactions, \actions} \cdot \fun{\log \embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction} + \log \latentprobtransitions_{\decoderparameter}\fun{\latentstate' \mid \latentstate, \latentaction} - \log \encoder^{\actions}\fun{\latentaction \mid \latentstate, \action}}.
    \end{align*}
Notice that we cannot assign directly $p_{\tuple{\state, \action, \reward, \state'}}$ to $\loss_{\elbo}$ since priorities require to be strictly positive to compute the replay buffer distribution.
A solution is to pass $\loss_{\elbo}\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentaction, \latentstate'}}$ to the logistic function, i.e.,
\[
    p_{\tuple{\state, \action, \reward, \state'}} = x^{\star} \cdot \sigma\fun{k \cdot \fun{\loss_{\elbo}\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentaction, \latentstate'}} - x_0}}
\]
where $x^{\star} > 0$ is the scale, $k > 0$ is the growth rate, and $x_0$ is the location of the logistic.
In practice, we set $x^{\star}$ to the desired maximum priority and we maintain upper ($L^{\max}$) and lower bounds ($L^{\min}$) on the loss during learning.
Along training steps, we tune these values according to the current loss and we set $x_0 = \frac{L^{\max} - L^{\min}}{2}$ and $k = \frac{x^{\star}}{L^{\max} - L^{\min}}$.

\begin{figure}
    \begin{subfigure}{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ressources/cartpole_histogram.pdf} \\
        \caption{CartPole}
    \end{subfigure}
    \begin{subfigure}{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ressources/mountain_car_histogram.pdf} \\
        \caption{MountainCar}
    \end{subfigure}\\
    \begin{subfigure}{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ressources/acrobot_histogram.pdf} \\
        \caption{Acrobot}
    \end{subfigure}
    \begin{subfigure}{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ressources/pendulum_histogram.pdf} \\
        \caption{Pendulum}
    \end{subfigure}
    \caption{Latent space distribution along training steps. The intensity of the blue hue corresponds to the frequency of latent states produced by $\embed$ during training. We compare a bucket-based prioritized against a simple uniform experience replay. The latent space learned with transitions sampled from the uniform replay buffer collapses to (a) two, (b) a single, (c)~and~(d) few latent state(s).}
    \label{appendix:fig:prioritized-replay}
\end{figure}

\section{Details on RL Policy Distillation}
% One can see $\latentpolicy_{\decoderparameter}$ as a \emph{compression} of the input RL policy $\policy$ over $\latentstates$ and $\latentactions$.
Concretely, the goal of $\latentpolicy_{\decoderparameter}$ is to mimic the behavior of $\policy$ through the latent spaces.
However, executing $\latentpolicy_{\decoderparameter}$ in $\mdp$ via $\embed_{\encoderparameter}$ and $\embeda_{\encoderparameter, \decoderparameter}$ as described in Sect.~\ref{section:deepmdp} to evaluate our latent space model (e.g., Lem.~\ref{lemma:pac-loss}) may
% lead the agent to parts of the state space that are not reachable when we execute the original policy $\policy$. %,
result in performance loss compared to that offered under $\policy$.
%with
%$\mdp_{\policy}$ and $\mdp_{\latentpolicy}$ not behaving exactly the same.
% This is due to our abstraction approach: we do not expect a perfect bisimulation between the two models but a suitable bisimulation distance.
This is due to the abstraction learned via the ELBO: we do not expect a zero-distortion by encoding the state-action space through the VAE (and $\mdp_{\latentpolicy_{\decoderparameter}}$ to behave exactly like $\mdp_{\policy}$), but to minimize it.
Due to this remaining distortion, decisions taken according to $\latentpolicy_{\decoderparameter}$ may result in unreachable states under $\policy$, causing $\latentpolicy_{\decoderparameter}$ to behave poorly in that particular states since the learning process only allows to learn from transitions produced via $\policy$.
We propose two approaches that can be used alone or together to alleviate this problem.

\smallparagraph{Globally-robust RL policy.}~%
In general, policies $\policy$ learned through deep-RL provide \emph{local} performance, meaning they provide good performance in states $\state \in \states$ that are likely to be reached from $\sinit$ by executing $\policy$. % (i.e., $\expectedsymbol{\state \sim \stationary{\policy}}{\values{\policy}{}{\state}}$ is good).
It is, however, often suitable to distil and verify \emph{globally-robust} RL policies, i.e., policies trained to provide good \emph{global} performance, in a wider range of states, in particular those that are likely to be reached through the distillation.
%Indeed, policies under consideration should be learned to optimize $\values{\policy}{}{\state}$ for a wider range of states $\state \in \states$ than those reachable from $\sinit$ under $\policy$ in $\mdp$, in particular those that are likely to be reached after the distillation. %perturbations (e.g., those linked to the distortion of $\latentpolicy_{\decoderparameter}$),
Training globally robust RL policies can be achieved by allowing the agent to learn (or pursuing its training) in a modified version of $\mdp$, where $\sinit$ is picked at random from $\states$.
Training $\policy$ this way will usually take longer since this may require more exploration.
The degree of randomness can be decided according to the exploration/exploitation trade-off and the additional training time allowed. %or set uniform if the environment allows it.
Moreover, we argue that this additional time is acceptable in our context since enabling and applying model checking are time-consuming tasks by nature.

\smallparagraph{$\varepsilon$-mimic.}~Assuming $\policy$ is sufficiently robust for the distillation, we allow the encoder to process states reachable under both $\latentpolicy_{\decoderparameter}$ and $\policy$ by learning from a mixture $\hat{\policy}^{\varepsilon}_{\decoderparameter}$ of the two, defined as $\hat{\policy}^{\varepsilon}_{\decoderparameter}\fun{\action \mid \state} = \policy\fun{\action \mid \state} \cdot (1 - \varepsilon) + \latentpolicy_{\decoderparameter}\fun{\action \mid \state} \cdot \varepsilon$ for all $\state \in \states$, $\action \in \actions$, given $\varepsilon \in \mathopen[0, 1 \mathclose]$.
Given the robustness assumption, states entered according to a decision $\action \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \state}$ (produced with probability $\varepsilon$) should be efficiently processed
by $\policy$.
In practice, we start with a high value of $\varepsilon$ (e.g., $\varepsilon=\nicefrac{1}{2}$) to encourage exploration of states possibly reachable under $\latentpolicy_{\decoderparameter}$ and we anneal it to $0$ during training.

\section{Experiments}\label{appendix:experiments}
%
\subsection{Setup}
We used \textsc{TensorFlow} \texttt{2.4.1} \citepAR{tensorflow2015-whitepaper} to implement the neural networks modeling our parameterized distributions constituting our variational model, optimize the loss function ($\elbo$), and running our PAC approximation schemes.
Precisely, we used \textsc{TensorFlow Probability} \texttt{0.12.2} \citepAR{dillon2017tensorflow} to handle the probabilistic components of the VAE (e.g., distributions, reparameterization tricks, etc.), as well as \textsc{TF-Agents} \texttt{0.7.1} \citepAR{TFAgents} to handle the RL parts of the framework, coupled with \textsc{Reverb} replay buffers \citepAR{cassirer2021reverb}.

The experiments have been driven on a cluster running under \texttt{CentOS Linux 7 (Core)} composed of a mix of nodes containing Intel processors with the following CPU microarchitectures:
(i) \texttt{10-core INTEL E5-2680v2}, (ii) \texttt{14-core INTEL E5-2680v4}, and (iii) \texttt{20-core INTEL Xeon Gold 6148}.
We used $8$ cores and $128$ GB of memory for each of our experiments.

\subsection{Hyper-parameters}
Each distribution parameters (locations, scales, logits) are inferred by neural networks (multilayer perceptrons) composed of two dense hidden layers and $256$ cells by layer.
For all our experiments, we used the \textsc{TensorFlow}'s implementation of the Adam optimizer \citepAR{DBLP:journals/corr/KingmaB14} to learn the neural networks weights.
We fixed the size of the prioritized experience replay to $10^{6}$.
The training starts when the agent has collected $10^{4}$ transitions in $\mdp$.
Every time a transition is added to the replay buffer, its priority is set to the maximum value.
We used minibatches of size $128$ to optimize the loss function (i.e., $\elbo$) and we applied a minibatch update every time the agent executing $\policy$ performed $16$ steps in $\mdp$.
This allows the VAE to process at least $\nicefrac{1}{8}$ of the new transitions collected by sampling from the replay buffer (more details in \citealt{DBLP:journals/corr/SchaulQAS15}).
We fixed $\omega$ to $0.4$ as suggested by \citet{DBLP:journals/corr/SchaulQAS15}.

\smallparagraph{Annealing schemes.}~During training, we anneal different hyper-parameters to $0$ or $1$ according to the following annealing schemes:
(i) we start annealing the parameters at step $t_0 = 10^{4}$, 
(ii) let $\zeta \in \mathopen[ 0, \infty \mathclose]$, we anneal $\zeta$ to $0$ via $\zeta_t = \zeta \cdot (1 - \tau_{\zeta})^{t - t_0}$, or
(iii) let $\zeta \in \mathopen[ 0, 1]$, we anneal $\zeta$ to $1$ via $\zeta_{t} = \zeta + (1 - \zeta)\cdot (1 - (1 - \tau_{\zeta})^{t - t_0})$
for step $t > t_0$ and annealing term $\tau_{\zeta}$.

\smallparagraph{Unshared parameters.}~The list of single hyper-parameters used for the different environments is given in Table~\ref{table:hyperparameters}.
The activation function of all cells of the neural networks was chosen between relu and leaky relu, the learning rate of the optimizer in $\mathopen[10^{-4}, 10^{-3}\mathclose]$, the regularizer scale factor $\alpha$ from $\set{0.1, 1, 10, 100}$, $\varsigma$ in $\mathopen[0, 1\mathclose]$, the values of each annealing term in $\mathopen[ 10^{-6}, 10^{-4} \mathclose]$, and we tested both loss- and bucket-based experience replay buffers.

\begin{table}
    \centering
    \input{hyperparameters}
    \caption{Hyper-parameter choices for the different environments.
    We write
    $\temperature^X_Y$ for the temperature parameter used for the concrete relaxation of Bernoulli distributions when $X = \latentstates$ (resp. Categorical distributions when $X = \latentactions$).
    This is the encoder distribution if $Y=1$ and the one of the latent transition function (resp. distilled policy) else, if $Y=2$. 
    Moreover, we write $\alpha_{\scriptscriptstyle \actions}$ for the scale factor of the action entropy regularizer where the final entropy regularization term is $\alpha \cdot \fun{\entropy{\encoder} + \alpha_{\scriptscriptstyle \actions} \cdot \entropy{\encoder^{\actions}}}$.}
    \label{table:hyperparameters}
\end{table}

\subsection{Labeling functions}
The labeling functions $\labels$ we used for each environment are detailed in Table~\ref{appendix:table:labels}.
%
\input{labels}
%
%
\section{Reproducibility Checklist}
\smallparagraph{Seeding.}~The code we provide allows for setting random seeds to run the experiments, making the overall shape of the Figures we present in this paper reproducible.
However, the exact values obtained in each particular instance are not: our prioritized experience replays (and those of \textsc{TF-Agents}) rely on \textsc{Reverb} replay buffers, handling randomness via the \textsc{Abseil} \texttt{C++} library{\footnote{\texttt{https://abseil.io}}} which does not allow for manual seeding.
All other libraries using randomness are seeded properly.

\clearpage
\bibliographystyleAR{aaai22}
\bibliographyAR{references}

==> related_work.tex <==
\smallparagraph{Other related work.}
%~We already mentioned the {DeepMDP} framework \citep{DBLP:conf/icml/GeladaKBNB19} 
%which introduced abstraction quality guarantees for representation learning purposes.
%
Frameworks providing formal guarantees \emph{during the RL process} include the work of \citet{DBLP:conf/tacas/Junges0DTK16}, \emph{Shielded-RL} \citep{DBLP:conf/aaai/AlshiekhBEKNT18,jansen_et_al:LIPIcs:2020:12815}, and \emph{AlwaysSafe} \citep{DBLP:conf/atal/SimaoJS21}.
These all require an abstract model of the safety aspect of the environment. Our approach is complementary in that we assume no prior knowledge and \emph{learn an abstraction}.
Notably, our goal is not the same: they aim at verifying whether the exploration is safe while our goal is to verify policies learned via \emph{any} RL technique.
The \textsc{Mosaic} approach \citep{DBLP:conf/formats/Bacci020} shares ours
% \citet{DBLP:conf/formats/Bacci020} share
%this purpose with ours
in the particular case of verifying deep-RL policies.
%They repeatedly refine an abstraction by partitioning the state space into hyperrectangles, and derive upper probability bounds on failure states.
However, they require (i) the neural network specifying the policy, (ii) the environment to be known and deterministic, and (iii) a formal description of the probability with which faults occur when attempting to execute particular actions.
%
%\todo{F: RNN paper here}
Finally, \citet{DBLP:conf/ijcai/CarrJT20} verify policies represented as recurrent neural networks (RNNs).
Although they require the environment to be discrete as well as a formal model of the environment. The authors discretize the RNN hidden states by using \emph{quantized} autoencoders%
% (another approach to learning discrete latent spaces)
, in the same spirit as our policy distillation.
%, and (iii) the hidden states of the RNN to be discretized (here, via a quantized autoencoder, another approach to learning discrete latent spaces).

VAEs have been used in the context of (model-based) RL to learn latent representations of the unknown environment and train
simpler policies
from the features extracted
%defined over the induced latent observation space
(e.g., \citealt{DBLP:conf/icml/CorneilGB18, DBLP:conf/nips/FreemanHM19, DBLP:conf/nips/LeeNAL20,ALA2021:Burden-et-al}).
In particular, \citet{DBLP:conf/icml/CorneilGB18} focused on learning discrete latent MDPs from continuous-state environments with discrete actions (without guarantees nor distilled policies) to plan via \emph{prioritized sweeping}. % \citep{DBLP:books/lib/SuttonB98}.

==> table_evaluation_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}
\centering
\caption{Formal Verification of distilled latent policies for diverse LTL properties.}
\label{table:evaluation-ltl}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllllllllll@{}}
\toprule
  & 
  Environment &
  $\states$ &
  $\actions$ &
  $\left|\latentstates\right|$ &
  $\left|\latentactions\right|$ &
  $\varphi$&
  $\latentvalues{\latentpolicy_{\decoderparameter}}{\varphi}{\zinit}$ &
  $\discount$ &
  $\localrewardloss{\stationary{\latentpolicy_{\decoderparameter}}}$ (PAC) &
  $\localtransitionloss{\stationary{\latentpolicy_{\decoderparameter}}}$ (PAC) \\ \midrule
 1 &
{CartPole} &
  $\subseteq \R^4$ &
  $\set{1, 2}$ &
  $512$ &
  $2$ &
  $\always \neg \textsf{Unsafe}$ &
  $0.958882$ &
  $0.99$ &
  $0.00499653$ &
  $0.399636$ & \\
  2&
{MountainCar} &
  $\subseteq \R^2$ &
  $\set{1, 2}$ &
  $1024$ &
  $3$ &
  $\always \eventually \textsf{Flag}$ &
  $0.999843$ &
  $1 - 10^{-4}$ &
  $0.0141763$ &
  $0.382323$ & \\
  3 &
  {Pendulum} &
  $\subseteq \R^3$ &
  $\mathopen[ -2, 2 \mathclose]$ &
  $8192$ &
  $3$ &
  $\eventually\fun{\until{\textsf{Upright}}{\textsf{Reset}}}$ &
  $0.948295$ &
  $1 - 10^{-4}$ &
  $0.0266745$ &
  $0.539508$ &\\
  4 &
  {Pendulum} &
  $\subseteq \R^3$ &
  $\mathopen[ -2, 2 \mathclose]$ &
  $8192$ &
  $3$ &
  $\always\eventually\fun{\until{\textsf{Upright}}{\textsf{Reset}}}$ &
  $0.953257$ &
  $1 - 10^{-4}$ &
  $0.0266745$ &
  $0.539508$ &\\
  5 &
  {LunarLander} &
  $\subseteq \R^8$ &
  $\mathopen[-1, 1\mathclose]^2$ &
  $16384$ &
  $3$ &
  $\always \fun{\neg \fun{\neg \textsf{SafeLanding} \wedge \ltlnext \textsf{Reset}}}$ &
  $0.908891$ &
  $0.99$ &
  $0.0207205$ &
  $0.131357$ & \\
  6 &
  {LunarLander} &
  $\subseteq \R^8$ &
  $\mathopen[-1, 1\mathclose]^2$ &
  $16384$ &
  $3$ &
  $\eventually\fun{\until{\neg \textsf{SafeAngle}}{\textsf{LegContact}}}$ &
  $0.0943765$ &
  $0.99$ &
  $0.0207205$ &
  $0.131357$ & \\
  7 &
  {LunarLander} &
  $\subseteq \R^8$ &
  $\mathopen[-1, 1\mathclose]^2$ &
  $16384$ &
  $3$ &
  $\always \fun{\until{\textsf{SafeAngle}}{\textsf{LegContact}}}$ &
  $0.888488$ &
  $0.99$ &
  $0.0207205$ &
  $0.131357$ & \\
 \bottomrule
\end{tabular}%
}
\end{table}

==> vae.tex <==
%We consider the agent interacting with an \emph{unknown} environment modeled by a continuous MDP $\mdp = \mdptuple$.
% The environment being unknown precisely means that $\transitions$, $\rewards$ and $\labels$ are unknown, preventing us to use them to compute a policy for the agent.
% However, by interacting with the environment, the latter is able to observe the current state $\state$ of the environment and its label $\labeling = \labels\fun{\state}$, as well as the outcome of executing an action $\action$ in $\state$, i.e., $\state' \sim \probtransitions\fun{\sampledot \mid \state, \action}$, and the reward $\reward = \rewards\fun{\state, \action, \state'}$ of the resulted transition.
% Furthermore, if we fix a policy $\policy \in \policies{\mdp}$ for the agent, it produces execution traces $\defaulttrace \sim \mdp_\policy$ by interacting with $\mdp$ according to $\policy$.
%in $\mdp$ with $\action_{t+1} \sim \policy\fun{\sampledot \mid \indexof{\state}{0:t}, \indexof{\action}{0:t}}$ for $t < T - 1$.
%In order to use model checking as a mean to provide a control policy for the agent, the model to be verified is required to be finite.
%Therefore, we seek for a discrete abstraction $\latentmdp$ with finite state space $\latentstates$ and action space $\latentactions$ where the agent would be able to produce and recover the set of outputs (i.e., execution traces) of $\mdp$ with same probability when a policy is fixed in $\latentmdp$.
% In the following, we describe how we tackle this problem by learning the abstraction via parameterized function approximators.
%
%
%
We now provide a framework based on \emph{variational autoencoders} \citep{DBLP:journals/corr/KingmaW13} that allows us learning a (discrete) latent space model of $\mdp$ through the interaction of the agent executing a pre-learned RL policy $\policy \in \mpolicies{\mdp}$ in the environment.
Concretely, we seek a latent space model $\tuple{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter}}$ such that $ \latentmdp_{\decoderparameter} = \tuple{\latentstates, \latentactions, \latentprobtransitions_{\decoderparameter}, \latentrewards_{\decoderparameter}, \latentlabels_{\decoderparameter}, \atomicprops, \zinit}$.
We propose to learn the parameters $\tuple{\encoderparameter, \decoderparameter}$ of a \emph{behavioral model} $\decoder$ from which we can retrieve $\latentprobtransitions_{\decoderparameter}$, $\latentrewards_{\decoderparameter}$, and $\latentlabels_{\decoderparameter}$ through the following optimization:
\begin{align}\label{eq:mdp-discrepancy}
    \min_{\decoderparameter} \divergence{\mdp_\policy}{\decoder},
\end{align}
where $\divergencesymbol$ denotes a discrepancy measure. Intuitively, the end goal is to allow $\decoder$ to learn to mimic the behavior of the original MDP by making use of an \emph{encoder} $\encoder$ (including the state embedding function), thus yielding a latent MDP bisimilar to $\mdp$.
In the following, we present two approaches that are distinguished by the discrepancy $\divergencesymbol$ chosen.

\subsection{The variational approach}
\subsubsection{State space abstraction}
We first focus on learning an abstraction of $\states$ through a latent space model $\tuple{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \sampledot}$ that shares its action space with $\mdp$ (i.e., $\latentactions = \actions$).
% equipped with a reconstruction model $\decoder$ with parameters $\decoderparameter$ from which we can retrieve models for $\transitions_\decoderparameter$, $\rewards_\decoderparameter$, and $\labels_\decoderparameter$.
Fix any policy $\policy \in \mpolicies{\mdp}$, we dedicate this Subsection to the optimization of Eq.~\ref{eq:mdp-discrepancy} through KL divergence, i.e., $\min_{\decoderparameter} \dkl{\mdp_{\policy}}{\decoder}$, or equivalently the maximization of the marginal \emph{log-likelihood of traces} of the original MDP, given by
\begin{equation}
    \expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}}} \label{eq:maximum-likelihood}
\end{equation}
where we make the dependence of $\tuple{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T}}$ on $\latentstates$ explicit by the law of total probability:
\begin{align}
    & \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\action}{T - 1}} \notag \\
    =&  \int_{\inftrajectories{\latentmdp_{\decoderparameter}}} \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} \cdot \condition{=}\fun{\seq{\action}{T - 1}, \seq{\action'}{T - 1}} \, d\latentprobtransitions_{\decoderparameter}\fun{\seq{\latentstate}{T} \mid \seq{\action'}{T - 1}} \label{eq:intractable-latent}
\end{align}
with $\trace = \defaulttrace$ and $\latentprobtransitions_{\decoderparameter}\fun{\seq{\latentstate}{T} \mid \seq{\action}{T - 1}} = \prod_{t = 0}^{T - 1} \latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \action_t}$. %, and $\tuple{\seq{\latentstate}{T}, \seq{\action}{T - 1}} \in \trajectories{{\latentmdp, \decoder}}$.
Notice that we consider the likelihood conditioned by actions chosen by $\policy$ since we do not desire to learn an MC, but rather an MDP.
Optimizing Eq.~\ref{eq:maximum-likelihood} through Eq.~\ref{eq:intractable-latent} is typically intractable.
Intuitively, given an execution trace $\trace$, one may want to make use of \emph{Monte-Carlo sampling methods} to approximate the likelihood of $\trace$ through Eq.~\ref{eq:intractable-latent}
by generating a finite number of latent sequences $\set{\seq{\latentstate^{\,i}}{T}}_{i=1}^{N}$ from $ \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \seq{\action}{T - 1}}$, and then averaging $\frac{1}{N}\sum_{i = 1}^{N}\decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate^{\,i}}{T}, \seq{\action}{T - 1}}$ to approximate $\decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid  \seq{\action}{T - 1}}$.
Using such methods amounts to trying to approximate an integration over elements from an infinitely uncountable space with a sum over a finite set of elements from this space, meaning that for most $\seq{\latentstate^{\, i}}{T}$, $\decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate^{\, i}}{T}, \seq{\action}{T - 1}}$ will be close to zero thus contributing almost nothing to our estimates.
To overcome this, we introduce a new model $\encoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}$ that we consider here as a {probabilistic encoder} giving a distribution over sequences $\seq{\latentstate}{T}$ that are likely to produce $\tuple{\seq{\state}{T}, \seq{\reward}{T-1}, \seq{\labeling}{T}}$ according to any policy sequentially producing $\seq{\action}{T-1}$.
We learn such an encoder through the following optimization:
\begin{equation}
    %\min_{\encoderparameter, \decoderparameter} \expected{\trace \sim \mdp_\policy}{\divergence{\encoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}}{\decoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}}}
    \min_{\encoderparameter, \decoderparameter} \; \expectedsymbol{\trace \sim \mdp_\policy}{\,\divergence{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{\sampledot \mid \trace}}}\,}
\end{equation}
where $\divergencesymbol$ denotes a discrepancy measure.
If we let once again $\divergencesymbol$ be the KL divergence, one can set a \emph{lower bound} on the log-likelihood of produced traces,
%on the $\log$-values of Eq.~\ref{eq:maximum-likelihood}
often referred to as \emph{evidence lower bound} (ELBO, \citealp{DBLP:journals/jmlr/HoffmanBWP13}) as follows:
\begin{align*}
    &&&\dkl{\encoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}}{\decoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}} \\
    &&=&\expectedsymbol{\seq{\latentstate}{T} \sim \encoder\fun{\sampledot \mid \trace}}\left[\log \encoder\fun{\seq{\latentstate}{T} \mid \seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}, \seq{\labeling}{T}} - \log \decoder\fun{\seq{\latentstate}{T} \mid \seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}\right] \\
    &&\begin{aligned}
        = \\ \, 
    \end{aligned}&\begin{aligned}
        \; \expectedsymbol{\seq{\latentstate}{T} \sim \encoder\fun{\sampledot \mid \trace}}&[\log \encoder\fun{\seq{\latentstate}{T} \mid \seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}, \seq{\labeling}{T}} - \log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T}, \seq{\labeling}{T} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} \\
        &\,-\log \latentprobtransitions_{\decoderparameter}\fun{\seq{\latentstate}{T} \mid \seq{\action}{T -1}}] + \log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}}
    \end{aligned} \tag{Bayes' rule}\\
    &\equiv&&\log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}} - \dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{ \sampledot \mid \trace}}} \\
    && =&\expectedsymbol{\seq{\latentstate}{T} \sim \encoder\fun{\sampledot \mid \trace}}[{\log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate}{T}, \seq{\action}{T-1}}}] \\
    &&&- \dkl{\encoder\fun{\sampledot \mid \seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T-1} \seq{\labeling}{T}}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \seq{\action}{T -1}}}
    %&& =& \; \elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}}.
\end{align*}
The purpose of optimizing the ELBO is twofold.
First, it allows us learning $\embed_{\encoderparameter}$ through $\encoder$ with $\encoder\fun{\seq{\latentstate}{T} \mid \seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T-1} \seq{\labeling}{T}} = \prod_{t = 0}^{T - 1} \embed_{\encoderparameter}\fun{\latentstate_{t + 1} \mid \state_t}$.
Second, this allows us learning transition, reward and label models for $\latentmdp$.
We thus argue that sequences $\seq{\state}{T}$, $\seq{\reward}{T - 1}$, and $\seq{\labeling}{T}$ can be made independent given $\tuple{\seq{\latentstate}{T}, \seq{\action}{T - 1}}$.
Moreover, we assume that a \emph{generative model} $\decoder^{\generative}$ enabling the reconstruction from latent states in $\latentstates$ to grounded states in $\states$ exists, which gives us
% log version
% \begin{align*}
%     & \log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}}\\
%     =\, & \log \decoder^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}} + \log \decoder^{\rewards}\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} + \log \decoder^{\labels}\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}}
% \end{align*}
\begin{align}
    \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}}
    = \decoder^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}} \cdot \decoder^{\rewards}\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} \cdot \decoder^{\labels}\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}} %\label{eq:behavioral-model-chain}
\end{align}
$\textstyle \text{with } \allowbreak \decoder^{\generative}(\seq{\state}{T} \mid \seq{\latentstate}{T}) = \prod_{t = 0}^{T} \decoder^{\generative}(\state_t \mid \latentstate_t), \, \decoder^{\rewards}(\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}) = \prod_{t = 0}^{T - 1} \decoder^{\rewards}(\reward_{t} \mid \latentstate_t, \action_t) \text{, and } 
\decoder^{\labels}(\seq{\labeling}{T} \mid \seq{\latentstate}{T}) = \prod_{t = 0}^{T}\decoder^{\labels}(\labeling_t \mid {\latentstate}_{t}).$
We also emphasize that a \emph{perfect reconstruction} of labels is possible, i.e., $\log \decoder^{\labels}\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}} = 0$.
Intuitively, this can be done by encoding labels directly into the latent space. Details are given below.
From now on, we omit the label term.

Taking Assumption~\ref{assumption:ergodicity} into account, drawing multiple finite traces $\trace \sim \mdp_{\policy}$ can be seen as a continuous interaction with $\mdp$ along an infinite trace.
This observation allows us to formulate the ELBO in the local setting and connect to local losses introduced in Section~\ref{section:deepmdp}.
%
%
\begin{lemma}\label{lemma:trace-to-stationary}
Let  $\stationary{\policy}$ be the stationary distribution of $\mdp_\policy$ and $f \colon \states \times \actions \times \rewards \times \states \to \R$ be a continuous function.
Assume $\states, \actions$ are compact, then % induced by $\policy$, then 
\begin{align*}
    \lim_{T \to \infty} \frac{1}{T} \expected{\trace \sim \mdp_{\policy}[T]}{\sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}} = \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} f\fun{\state, \action, \reward, \state'}
\end{align*}
where $\mdp_{\policy}[T]$ denotes the distribution over $\traces{\mdp_\policy}\fun{T}$ and $ \stationary{\policy}(\state, \action, \reward, \state') = \stationary{\policy}(\state, \action, \state') \cdot \condition{=}(\reward,  \rewards\fun{\state, \action, \state'})$.
\end{lemma}
\begin{proof}
Let $\mu_T: \distributions{\states}, \state \mapsto \Prob_\policy\fun{\set{\tuple{\seq{\state}{\infty}, \seq{\action}{\infty}} \in \inftrajectories{\mdp_{\policy}} \mid \state_T = \state}}$ be the distribution giving the probability for the agent of being in each particular state of $\mdp_{\policy}$ after exactly $T$ steps. %, and $f \colon \states \times \actions \times \rewards \times \states \to \R$ be a continuous function.
First, observe that
\begin{align*}
    & \expected{\trace \sim \mdp_{\policy}[T]}{\sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}} \\
    =&  \expectedsymbol{\action_0 \sim \policy\fun{\sampledot \mid \sinit}}\expectedsymbol{\state_1 \sim \probtransitions\fun{\sampledot \mid \sinit, \action_0}} \expectedsymbol{\action_1 \sim \policy\fun{\sampledot \mid \state_1}} \cdots \expectedsymbol{\state_T \sim \probtransitions\fun{\sampledot \mid \state_{T - 1}, \action_{T - 1}}} \left[ \sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \rewards\fun{\state_t, \action_t, \state_{t + 1}}, \state_{t + 1}}\right]\\
    =& \sum_{t = 0}^{T - 1} \expectedsymbol{\action_0 \sim \policy\fun{\sampledot \mid \sinit}}\expectedsymbol{\state_1 \sim \probtransitions\fun{\sampledot \mid \sinit, \action_0}} \expectedsymbol{\action_1 \sim \policy\fun{\sampledot \mid \state_1}} \cdots \expectedsymbol{\state_T \sim \probtransitions\fun{\sampledot \mid \state_{T - 1}, \action_{T - 1}}} f\fun{\state_t, \action_t, \rewards\fun{\state_t, \action_t, \state_{t + 1}}, \state_{t + 1}}\\
    =& \sum_{t = 0}^{T - 1} \expectedsymbol{\trace \sim \mdp_{\policy}[t + 1]} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}.
\end{align*}
Therefore, we have
\begin{align*}
    & \lim_{T \to \infty} \frac{1}{T} \expected{\trace \sim \mdp_{\policy}[T]}{\sum_{t = 0}^{T - 1} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}}} \\
    =& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \expectedsymbol{\trace \sim \mdp_{\policy}[t + 1]} f\fun{\state_t, \action_t, \reward_t, \state_{t + 1}} \\
    =& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \int_{\traces{\mdp_{\policy}}\fun{t + 1}} f\fun{\state_t, \action_t, \rewards\fun{\state_t, \action_t, \state_{t + 1}}, \state_{t + 1}} \, d\Prob_\policy\fun{Cyl\fun{\seq{\state}{t + 1}, \seq{\action}{t}}} \tag{where $Cyl\fun{\seq{\state}{t + 1}, \seq{\action}{t}} = \set{\tuple{\seq{\state^{\star}}{\infty}, \seq{\action^{\star}}{\infty}} \in \inftrajectories{\mdp_{\policy}} \mid \state^{\star}_i = \state_i \quad \forall i \leq t + 1}$} \\
    =& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \int_{\states} \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\mu_t\fun{\state} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action} \\
    =& \lim_{T \to \infty} \int_{\states}  \frac{1}{T} \sum_{t = 0}^{T - 1} \mu_t\fun{d\state}  \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action}.
    %=& \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \expectedsymbol{\state \sim \mu_{t}} \expectedsymbol{\action \sim \policy\fun{\sampledot \mid \state}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \action}} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\state
\end{align*}
By definition of $\stationary{\policy}$, $\stationary{\policy}\fun{A} = \lim_{T \to \infty} \frac{1}{T} \sum_{t = 0}^{T - 1} \mu_{t}\fun{A}$ for all $A \in \borel{\states}$, i.e., $\mu_t$ weakly converges to $\stationary{\policy}$.
By Assumption~\ref{assumption:rewards}, the set of images of $\rewards$ is a compact space.
Therefore, $f$ has compact support and by the Portmanteau's Theorem, 
\begin{align*}
    & \lim_{T \to \infty} \int_{\states}  \frac{1}{T} \sum_{t = 0}^{T - 1} \mu_t\fun{d\state} \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action} \\
    =& \int_{\states} \stationary{\policy}\fun{d\state} \int_{\actions} \int_{\states} f\fun{\state, \action, \rewards\fun{\state, \action, \state'}, \state'} \, d\policy\fun{\action \mid \state} \, d\probtransitions\fun{\state' \mid \state, \action} \\
    =& \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} f\fun{\state, \action, \reward, \state'}.
\end{align*}
\end{proof}
%
\begin{corollary}
Let $ \embed\fun{\latentstate, \latentstate' \mid \state, \state'} = \embed\fun{\latentstate \mid \state} \embed\fun{\latentstate' \mid \state'}$, then
\begin{align*}
    & \lim_{T \to \infty} \frac{1}{T} \expectedsymbol{\trace \sim \mdp_{\policy}[T]}\left[\log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}} - \dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{ \sampledot \mid \trace}}} \right] \\
    % \begin{aligned}
    % = \\ \, \\ \, \\
    % \end{aligned} & \begin{aligned} \;
    % \lim_{T \to \infty} \frac{1}{T} \expectedsymbol{\trace \sim \mdp_{\policy}[T]} \Bigg[ \sum_{t = 0}^{T - 1} \expectedsymbol{\latentstate_t, \latentstate_{t + 1} \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state_t, \state_{t + 1}}} \big[&{\log \decoder^{\generative}\fun{\state_{t+1} \mid \latentstate_{t + 1}} + \log \decoder^{\rewards}\fun{\reward_{t + 1} \mid \latentstate_t, \action_t}} \\
    % & - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state_{t + 1}}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate_t, \action_t}}\big] \Bigg]
    % \end{aligned} \\
    =& \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy}\\ \latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}}\left[{\log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action}} - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot\mid \latentstate, \action}}\right].
\end{align*}
\end{corollary}
\begin{proof}
Taking 
\[f\fun{\state, \action, \reward, \state'} = \expectedsymbol{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}\big[\log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action} - \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot\mid \latentstate, \action}}\big]\]
yields the result.
\end{proof}
%
Finally, our objective becomes the maximization of the following ELBO:
\begin{align*}
    \max_{\encoderparameter, \decoderparameter}\; \elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}} = - \min_{\encoderparameter, \decoderparameter} \left\{\distortion_{\encoderparameter, \decoderparameter} + \rate_{\encoderparameter, \decoderparameter} \right\}
    %= \max_{\encoderparameter, \decoderparameter} & \; \expectedsymbol{}_{\trace \sim \mdp_\policy}[\;\log \decoder\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}} - \dkl{\encoder\fun{\seq{\latentstate}{T} \mid \trace}}{{\decoder\fun{\seq{\latentstate}{T} \mid \trace}}}\;] \notag \\
    %= \max_{\encoderparameter, \decoderparameter} & \; \expectedsymbol{}_{\trace \sim \mdp_\policy} \bigg[\, \sum_{t = 0}^{T - 1} \expected{z_t, z_{t + 1} \sim \encoder^\sim}{\log \decoder^{\generative}\fun{\state_t \mid \latentstate_t} + \log \decoder^{\rewards}\fun{\reward_{t + 1} \mid \latentstate_t, \action_t, \latentstate_{t + 1}} + \log \decoder^{\labels}\fun{\labeling_t \mid {\latentstate}_{t}}} \notag \\
    %& - \dkl{\encoder^\transitions\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \action_t}}  \,\bigg]
    %= \min_{\encoderparameter, \decoderparameter} & \; \distortion_{\encoderparameter, \decoderparameter} + \rate_{\encoderparameter, \decoderparameter}
\end{align*}
where $\distortion$ and $\rate$ denote respectively the \emph{distortion} and \emph{rate} of the variational model  \citep{DBLP:conf/icml/AlemiPFDS018} such that
\begin{align*}
    \distortion_{\encoderparameter, \decoderparameter} &= - \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expected{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}}{\log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action}} \\
    %\rate_{\encoderparameter, \decoderparameter} &= \expected{\trace \sim \mdp_\policy}{\sum_{t=0}^{T - 1}\dkl{\encoder^\transitions\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \action_t}}}
    \rate_{\encoderparameter, \decoderparameter} &=  \expectedsymbol{\state, \action, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \action}}.
\end{align*}
We omit the subscripts when the context is clear.
One can see the optimization of $\elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}}$ as an indirect optimization of (i) $\localrewardloss{\stationary{\latentpolicy}}$ via the log-likelihood of rewards produced by taking $\latentrewards_{\decoderparameter}\fun{\latentstate, \action} = \expectedsymbol{\reward \sim \decoder^{\rewards}\fun{\sampledot \mid \latentstate, \action}} \reward$, and (ii) $\localtransitionlossupper{\stationary{\latentpolicy}}$ where we change the Wasserstein distance term to KL divergence.
This change has a cost though, introducing new potential problems such as \emph{posterior collapse} with the loss of theoretical guarantees on the quality of the abstraction (c.f. Lemma~\ref{lemma:bidistance-abstraction-quality}).
%

\smallparagraph{Choosing $\policy$.} Learning a discrete abstraction of the full environment model describing all the possible interactions that the agent can have with it is hardly tractable and scalable.
Consequently, $\policy$ must be wisely chosen: $\latentstates$ is learned based on sequences generated from $\mdp_\policy$, meaning ${\latentmdp_{\decoderparameter}}$ is constrained to reachable parts of the system by executing $\policy$.
The key is to make $\policy$ permissive enough to constrain the abstraction to \emph{relevant} parts of the environment, by executing \emph{promising} actions to achieve the objective.
In practice, we compute a policy $\policy$ via an RL algorithm so that (i) the set of promising actions is determined by information gathered during the learning process, and (ii) the permissiveness of $\policy$ is expressed through its entropy. 
Intuitively, the higher the entropy of $\policy$, the more permissive $\policy$ is.

\smallparagraph{Discrete latent distributions.} We aim at learning a \emph{discrete} latent space $\latentstates$, $\embed_{\encoderparameter}$ and $\latentprobtransitions_{\decoderparameter}$ are thus supposed to be \emph{discrete distributions}.
W.l.o.g., we assume latent states to have a binary representation, we further see each bit as a Bernoulli random variable.
Two main challenges arise by learning the parameters of discrete latent distributions via stochastic computation graphs through optimization techniques such as \emph{gradient descent} and Monte-Carlo sampling methods:
(i) gradient descent is not applicable to learn $\encoderparameter$ and $\decoderparameter$ due to the discontinuity of $\latentstates$, and (ii) sampling $\latentstate$ from $\embed_{\encoderparameter}$ must be a \emph{derivable operation}.
We overcome both problems by making use of \emph{continuous relaxation of Bernoulli distributions} \citep{DBLP:conf/iclr/JangGP17,DBLP:conf/iclr/MaddisonMT17}.

Concretely, let $\logit \in \R$ and $\temperature \in \mathopen]0, 1 \mathclose]$, $\latentstate_\temperature \in \mathopen[0, 1\mathclose]$ has a \emph{relaxed Bernoulli distribution} $\latentstate_\temperature \sim \relaxedbernoulli{\logit}{\temperature}$ with logit $\logit$, temperature parameter $\temperature$ iff
(a) if $l$ is a logistic sample with location parameter $\logit\temperature^{-1}$ and scale parameter $\temperature^{-1}$, i.e., $l \sim \logistic{\logit\temperature^{-1}}{\temperature^{-1}}$, then $\latentstate_\temperature = \sigmoid\fun{l}$, $\sigmoid$ being the \emph{sigmoid} function,
(b) $\lim_{\temperature \to 0} \relaxedbernoulli{\logit}{\temperature} = \bernoulli{\logit}$, meaning $\Prob(\textstyle\lim_{\temperature \to 0} \latentstate_\temperature = 1) = \sigmoid\fun{\logit}$, and
(c) let $p_{\logit, \temperature}$ be the density of $\relaxedbernoulli{\logit}{\temperature}$, then $p_{\logit, \temperature}\fun{\latentstate_\temperature}$ is log-convex in $\latentstate_\temperature$.
Since the logistic distribution belongs to the location-scale family, it is fully reparameterizable, i.e., $l \sim \logistic{\logit\temperature^{-1}}{\temperature^{-1}} \equiv x \sim \logistic{0}{1} \text{ and } l = \frac{\logit + x}{\temperature}$.
In practice, we train $\embed_{\encoderparameter}$ and $\latentprobtransitions_{\decoderparameter}$ to infer and generate $\log_2 |\latentstates|$ logits, and we anneal $\temperature$ from $1$ to $0$ during training while using Bernoulli distributions for evaluation.
As prescribed in \cite{DBLP:conf/iclr/MaddisonMT17}, we use two different temperature parameters, one for $\embed_{\encoderparameter}$ and another for $\latentprobtransitions_{\decoderparameter}$.

In order to enable $\log \decoder^\labels\fun{\seq{\labeling}{T} \mid \seq{\latentstate}{T}} = 0$, we linearly encode $\labeling_t$ into each $\latentstate_t$ via $\embed_{\encoderparameter}$.
Recall that each label is given in binary, we thus allocate $|\atomicprops|$ bits in $\latentstates$ for the labels.
This enforces the following property of the $\embed_{\encoderparameter}$:
\[
\forall \state \in \states, \, \forall \latentstate \in \latentstates,\, \embed_{\encoderparameter}\fun{\latentstate \mid \state} > 0 \implies \labels\fun{\state} = \latentlabels_\decoderparameter\fun{\latentstate},
\]
which allows satisfying Assumption~\ref{assumption:labeling} when considering a deterministic encoder.

\smallparagraph{Posterior collapse.} A common issue encountered while optimizing variational models by maximizing the ELBO is the so called \emph{posterior collapse} problem.
Intuitively, this results in a degenerated local optimum where the model learns to ignore the latent space while the reconstruction model alone is used to optimize the ELBO.
With a discrete encoder, this translates into a deterministic mapping to a single latent state, regardless of the input.

From an information-theoretic point of view, optimizing an ELBO gives way to a trade-off between the minimization of the rate and the distortion, where the feasible region is a convex set \citep{DBLP:conf/icml/AlemiPFDS018}.
Posterior collapse happens when the rate is close to zero (referred to as the \emph{auto-decoding limit} of the variational model). %, which can be achieved by the optimizer by merging all states to the same embedding.
%$\expected{\trace \sim \mdp_\policy}{\sum_{t=0}^{T - 1}\dkl{\encoder^\transitions\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \action_t}}} \approx 0$, meaning
% $\encoder^\transitions\fun{\seq{\latentstate}{T} \mid \seq{\state}{T}, \seq{\action}{T - 1}} \approx \latentprobtransitions_{\decoderparameter}\fun{\seq{\latentstate}{T} \mid \seq{\action}{T - 1}}$.
%$\log \embed_{\encoderparameter}\fun{\latentstate' \mid \state'} \approx \expected{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}{\log \latentprobtransitions_{\decoderparameter}\fun{{\latentstate}' \mid \latentstate, {\action}}}$ for any $\latentstate' \in \latentstates$ by definition of the KL divergence.
%This means (i) the embedding distribution is nearly independent of ${\state' \in \states}$, and (ii) the latent  transition distribution tends to ignore $\action \in \actions$.
% The latent representation is thus not encoding information about input transitions, meaning that it fails to create a useful representation.
On the other hand, one can achieve a distortion close to zero (referred to as the \emph{auto-encoding limit}) at the price of a higher rate.

As already mentioned, posterior collapse is a consequence of the KL divergence here replacing the Wasserstein in the rate minimization: when the latter is used, Lemma~\ref{lemma:local-loss-upper-bounds} and Lemma~\ref{lemma:bidistance-abstraction-quality} ensure that a value close to zero implies a bisimilarity between states embedded to the same representation.

Different solutions have been proposed in the literature to prevent posterior collapse.
These include \emph{KL-scaling} and \emph{KL-annealing}, that consists in changing the ELBO to $\beta\text{-}\elbo = -(\distortion + \beta \cdot \rate)$, with $\beta \in \mathopen[0, 1\mathclose]$.
This allows to interpolate between auto-encoding and auto-decoding behavior which is not possible with the standard ELBO objective.

Another method consists in adding a cross-entropy regularizer $\alpha \in \mathopen[1, \infty\mathclose[$ to the ELBO, giving
% \begin{equation*}
%     \alpha\text{-}\elbo_{\latentstates}(\encoderparameter, \decoderparameter) = \expectedsymbol{\trace \sim \mdp_\policy}[\expected{\seq{\latentstate}{T} \sim \encoder}{\log \decoder\fun{\seq{\state}{T}, \seq{\latentstate}{T}, \seq{\reward}{T-1} \mid \seq{\action}{T-1}}} + \alpha \cdot \entropy{\encoder(\sampledot \mid \trace)}]
% \end{equation*}
\begin{align*}
    %& \alpha\text{-}\elbo(\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}) \\
    \expectedsymbol{}_{\substack{\state, \action, \reward, \state' \sim \stationary{\policy} \\ \latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}}\big[{{\log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \action}} + \log \latentprobtransitions_{\decoderparameter}\fun{\latentstate' \mid \latentstate, \action}} + \alpha \cdot \entropy{\embed_{\encoderparameter}(\sampledot \mid \state')}\big]
\end{align*}
and anneal $\alpha$ to 1 during training \citep{DBLP:conf/icml/HaarnojaZAL18,DBLP:conf/corl/BurkeHR19}, where 
%$\decoder\fun{\seq{\state}{T}, \seq{\latentstate}{T}, \seq{\reward}{T-1} \mid \seq{\action}{T-1}} = \prod_{t = 0}^{T - 1} \decoder^{\generative}(\state_{t+1} \mid \latentstate_{t + 1}) \cdot \decoder^{\rewards}(\reward_{t + 1} \mid \latentstate_t, \action_t, \latentstate_{t + 1}) \cdot \latentprobtransitions_{\decoderparameter}(\latentstate_{t + 1} \mid \latentstate_t, \action_t)$, and
$\entropy{P}$ denotes the entropy of $P \in \distributions{\measurableset}$ for measurable space $\measurableset$.
Intuitively, this allows encouraging the encoder to learn to make plenty use of the latent space to represent the input data.

A drawback of these methods is that we are no longer optimizing a lower bound on the log-likelihood of the input sequences while optimizing
\begin{equation*}
\tuple{\alpha, \beta}\text{-}\elbo(\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}) = - (\distortion_{\encoderparameter, \decoderparameter} + \beta \cdot \rate_{\encoderparameter, \decoderparameter}) + (\alpha - 1) \cdot \entropy{\embed_{\encoderparameter}}
\end{equation*}
In practice, setting up annealing schemes for $\alpha$ and $\beta$ allows to eventually recover the ELBO and avoid posterior collapse ($\alpha=1$ and $\beta=1$ matches the ELBO).
\cite{DBLP:conf/iclr/HeSNB19} introduced a method only based on the training process of the variational model, which allows to overcome this problem.
It consists in an aggressive training schedule which iterates between multiple updates of $\encoderparameter$ and one update of $\decoderparameter$, based on the observation that the inference model often lags behind the reconstruction model during training when posterior collapse occurs.

In our experiments, we also noticed that posterior collapse is even more difficult to handle when the entropy of the produced traces is low, in particular when rewards and states produced by executing $\policy$ have low variance.
This can be explained by an auto-encoding behavior: \cite{DBLP:conf/icml/AlemiPFDS018} showed that $\dataentropy - \rate$ is an upper bound on the distortion $\distortion$ that can be achieved, with $\dataentropy$ being the entropy of the input distribution (in our case $\dataentropy = \entropy{\stationary{\policy}}$).
When $\entropy{\stationary{\policy}}$ is low, the optimizer may tend to minimize the distortion by pushing the rate close to zero and achieve this way the low entropy of the input distribution.

\subsubsection{Action space abstraction}
Assuming the action space $\actions$ is large or continuous, we additionally now consider learning a discrete space $\latentactions$ through the latent space model $\tuple{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}}$.
Intuitively, the trick here is to let the dynamics of $\policy$ be part of the abstraction.
Then, the log-likelihood of execution traces produced when executing $\policy$ in $\mdp$ %by making use of latent spaces $\latentstates$ and $\latentactions$
is given by
\begin{equation*}
    \expected{\trace \sim \mdp_\policy}{\log \decoder\fun{\trace}} \label{eq:maximum-likelihood-with-actions}
    \text{ such that }
    \decoder\fun{\trace} = \int_{\inftrajectories{\latentmdp_{\decoderparameter}}} \decoder\fun{\trace \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \, d\latentprobtransitions_{\latentpolicy, \decoderparameter}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} 
\end{equation*}
with $\latentprobtransitions_{\latentpolicy, \decoderparameter}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1}} = \prod_{t = 0}^{T - 1} {\latentpolicy_{\decoderparameter}}\fun{\latentaction_t \mid \latentstate_t} \cdot \latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \latentaction_t}$.
Note that $\latentpolicy_{\decoderparameter}$ can be seen as a \emph{simplified policy} embedding dynamics of $\policy$ defined over the latent spaces.
As for the state space abstraction case, we set up a lower bound on the log-likelihood of produced traces as follows:
\begin{align*}
    &&& {\dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{\sampledot \mid \trace}}}} \notag \\
    &&= \,& {\expected{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \sim \encoder\fun{\sampledot \mid \trace}}{\log \encoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1} \mid \trace} - {\decoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \mid \trace}}}} \notag \\
    && \begin{aligned}
       = \\ \, \\
    \end{aligned} \;& \begin{aligned}
        \expectedsymbol{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \sim \encoder\fun{\sampledot \mid \trace}}[&\log \encoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1} \mid \trace} - \log \decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}\mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}\\
        & - \log \latentprobtransitions_{\latentpolicy, \decoderparameter}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}] + \log \decoder\fun{\trace}
    \end{aligned} \tag{Bayes' rule} \\
    &\equiv&& {\log \decoder\fun{\trace} - \dkl{\encoder\fun{\sampledot \mid \trace}}{{\decoder\fun{\sampledot \mid \trace}}}} \notag \\
    %&&= & \expectedsymbol{\trace \sim \mdp_\policy}\bigg[\expectedsymbol{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \sim \encoder}[\log \decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}\mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}]  \notag \\
    %&&& \quad\quad\quad\quad - \dkl{\encoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1} \mid \trace}}{\latentprobtransitions_{\decoderparameter}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}}\bigg] \label{eq:ground-action-elbo}
    && \begin{aligned}
        = \\ \, \\
    \end{aligned} \:& \begin{aligned}
        \expectedsymbol{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \sim \encoder\fun{\sampledot \mid \trace}}[&\log \decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}\mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}  + \log \latentprobtransitions_{\latentpolicy, \decoderparameter}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \\
        & - \log \encoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1} \mid \trace}]
    \end{aligned} \label{eq:ground-action-elbo}
\end{align*}
We assume the existence of a decoder enabling the reconstruction of actions in $\actions$, based on the current state of $\latentmdp_{\decoderparameter}$ and the discrete action chosen in that state.
Then, we have
\begin{align*}
    & \log \decoder\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1}\mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \\
    =\, & \log \decoder^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}} + \log \decoder^{\generative}\fun{\seq{\action}{T - 1} \mid \seq{\latentstate}{T - 1}, \seq{\latentaction}{T - 1}} + \log \decoder^\rewards\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}
\end{align*}
with $\decoder^{\generative}(\seq{\action}{T - 1} \mid \seq{\latentstate}{T - 1}, \seq{\latentaction}{T - 1}) = \prod_{t = 0}^{T - 1} \embeda_{\decoderparameter}(\action_t \mid \latentstate_t, \latentaction_t)$, and $\decoder^\rewards(\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}) = \prod_{t = 0}^{T - 1} \decoder^\rewards(\reward_t \mid \latentstate_t, \latentaction_t)$.
This allows us learning our action embedding function through $\embeda_{\encoderparameter, \decoderparameter}\fun{\action \mid \state, \latentaction} = \expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction}$ for all $\state \in \states, \action \in \actions, \latentaction \in \latentactions$.
Regarding the encoder, the chain rule gives us $\encoder\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T-1} \mid \trace} = \encoder\fun{\seq{\latentaction}{T-1} \mid \seq{\latentstate}{T}, \trace} \cdot \encoder\fun{\seq{\latentstate}{T} \mid \trace}$.
We further learn an action encoder $\latentembeda_{\encoderparameter}$ through $\encoder\fun{\seq{\latentaction}{T-1} \mid \seq{\latentstate}{T}, \trace} = \prod_{t = 0}^{T - 1} \latentembeda_{\encoderparameter}\fun{\latentaction_t \mid \latentstate_t, \action_t}$.
Putting all together, our objective involves the following brand new ELBO measured in the local setting using Lemma~\ref{lemma:trace-to-stationary}:
\begin{align*}
    \max_{\encoderparameter, \decoderparameter}\, \elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}} = - \min_{\encoderparameter, \decoderparameter} \left\{ \distortion_{\encoderparameter, \decoderparameter} + \rate_{\encoderparameter, \decoderparameter} \right\},
\end{align*}
such that
\begin{align*}
    \distortion_{\encoderparameter, \decoderparameter} =& - \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{}_{\substack{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'} \\ \latentaction \sim \latentembeda_{\encoderparameter}\fun{\sampledot \mid \latentstate, \action}}}\left[{\log \embeda_{\decoderparameter}\fun{\action \mid \latentstate, \latentaction} + \log \decoder^{\generative}\fun{\state' \mid \latentstate'} + \log \decoder^{\rewards}\fun{\reward \mid \latentstate, \latentaction}}\right] \\
    % \rate_{\encoderparameter, \decoderparameter} =& \expectedsymbol{\trace \sim \mdp_\policy}\Big[\sum_{t=0}^{T - 1}\dkl{\encoder^\transitions\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \latentaction_t}} \notag \\
    % & \quad\quad\quad\quad\quad\;\, + \dkl{\embeda_{\encoderparameter}\fun{\latentaction_t \mid \latentstate_t, \action_t}}{\latentpolicy_{\decoderparameter}\fun{\latentaction_t \mid \latentstate_t}}\Big]
    % \begin{aligned}
    %     \rate_{\encoderparameter, \decoderparameter} = \\ \phantom{\rate_{\encoderparameter, \decoderparameter} = }
    % \end{aligned}& \;
    % \begin{aligned}
    %     \expectedsymbol{\trace \sim \mdp_\policy}\Big[\sum_{t=0}^{T - 1} \expectedsymbol{\latentstate_t \sim \encoder^\transitions} \big[&\dkl{\encoder^\transitions\fun{\latentstate_{t + 1} \mid \state_t, \action_t}}{\latentprobtransitions_{\decoderparameter}\fun{\latentstate_{t + 1} \mid \latentstate_t, \latentaction_t}} \\
    %     + & \dkl{\embeda_{\encoderparameter}\fun{\latentaction_t \mid \latentstate_t, \action_t}}{\latentpolicy_{\decoderparameter}\fun{\latentaction_t \mid \latentstate_t}}\big]\Big]
    % \end{aligned}
    \rate_{\encoderparameter, \decoderparameter} =& \expectedsymbol{\state, \action, \state' \sim \stationary{\policy}} \, \expectedsymbol{}_{\substack{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state} \\ \latentaction \sim \latentembeda_{\encoderparameter}\fun{\sampledot \mid \latentstate, \action}}}\left[ \dkl{\embed_{\encoderparameter}\fun{\sampledot \mid \state'}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} + \dkl{\latentembeda_{\encoderparameter}\fun{\sampledot\mid\latentstate, \action}}{\latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \right].
\end{align*}
 %where we consider the local setting under $\stationary{\policy}$ using Lemma~\ref{lemma:trace-to-stationary}.
%and executing $\latentaction$ in state $\latentstate$ can be seen as executing $\action \sim \decoder^{\generative}\fun{\sampledot \mid \latentstate, \latentaction}$ in the real environment.
%

\smallparagraph{Two-phase learning.} Optimizing $\elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter}}$ and learning both latent spaces at once might be a difficult task.
One can split this ELBO in two to better control the optimization and prevent this way (i) high-variance loss, (ii) the optimizer to fall in bad local optima, and (iii) posterior collapse.
Therefore, we re-write the ELBO as follows.
\begin{proposition}
Let $\tuple{\encoderparameter_1, \encoderparameter_2}$, $\tuple{\decoderparameter_1, \decoderparameter_2}$ be respectively encoder and behavior model parameters such that $\encoderparameter = \encoderparameter_1 \cup \encoderparameter_2$, $\decoderparameter = \decoderparameter_1 \cup \decoderparameter_2$, and $\tuple{\latentmdp_{\decoderparameter_1}, \embed_{\encoderparameter_1}}, \tuple{\latentmdp_{\decoderparameter_2}, \embed_{\encoderparameter_2}, \embeda_{\encoderparameter_{1}, \decoderparameter_2}}$ be latent space models of $\mdp$ such that $\latentmdp_{\decoderparameter_1}$ shares its action space with $\mdp$, then
\begin{align*}
    \elbo\fun{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}} =& \,\elbo\fun{\latentmdp_{\decoderparameter_1}, \embed_{\encoderparameter_1}} + \elbo\fun{\latentmdp_{\decoderparameter_2}, \embeda_{\encoderparameter_2, \decoderparameter_2}},
\end{align*}
if and only if
\begin{align*}
    & \elbo\fun{\latentmdp_{\decoderparameter_2}, \embeda_{\encoderparameter_2, \decoderparameter_2}} \\
    =& \lim_{T \to \infty} \frac{1}{T} \expected{\trace \sim \mdp_\policy[T]}{\log \decodersymbol_{\decoderparameter_2}^{\policy}\fun{\seq{\action}{T - 1} \mid \seq{\state}{T - 1}}  - \!\!\!\! \expectedsymbol{\seq{\latentstate}{T} \sim \encodersymbol_{\encoderparameter_{1}}\fun{\sampledot \mid \trace}} \! \dkl{\encodersymbol_{\encoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}{\decoder\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}} \\
    =& - \fun{\distortion_{\encoderparameter_2, \decoderparameter_2} + \rate_{\encoderparameter_2, \decoderparameter_2} }
\end{align*}
where $\expected{\trace \sim \mdp_\policy[T]}{\log \decodersymbol_{ \decoderparameter_2}^\policy\fun{\seq{\action}{T - 1} \mid \seq{\state}{T - 1}}}$ denotes the log-likelihood of $\policy$, and
\begin{align*}
    \distortion_{\encoderparameter_2, \decoderparameter_2} &= - \expectedsymbol{\state, \action \sim \stationary{\policy}}\expectedsymbol{}_{\substack{\latentstate \sim \embed_{\encoderparameter_1}\fun{\sampledot \mid \state} \\ \latentaction \sim \latentembeda_{\encoderparameter_2}\fun{\sampledot \mid \latentstate, \action}}}\left[\log \embeda_{\decoderparameter_2}\fun{\action \mid \latentstate, \latentaction}\right] - \Delta \latentprobtransitions_{\decoderparameter} - \Delta\decodersymbol_{\decoderparameter}^\rewards, \\
    \Delta\latentprobtransitions_{\decoderparameter} &= \expectedsymbol{\state, \action, \state' \sim \stationary{\policy}}\, \expectedsymbol{}_{\substack{\latentstate, \latentstate' \sim \embed_{\encoderparameter_1}\fun{\sampledot \mid \state, \state'} \\ \latentaction \sim \latentembeda_{\encoderparameter_2}\fun{\sampledot \mid \latentstate, \action}}}\left[\log \latentprobtransitions_{\decoderparameter_2}\fun{\latentstate' \mid \latentstate, \latentaction} - \log \latentprobtransitions_{\decoderparameter_1}\fun{\latentstate' \mid \latentstate, \action}\right],\\
    \Delta\decoder^\rewards &= \expectedsymbol{\state, \action, \reward, \sampledot \sim \stationary{\policy}}\expectedsymbol{}_{\substack{\latentstate \sim \embed_{\encoderparameter_1}\fun{\sampledot \mid \state} \\ \latentaction \sim \latentembeda_{\encoderparameter_2}\fun{\sampledot \mid \latentstate, \action}}} \left[ \log \decodersymbol_{\decoderparameter_2}^\rewards\fun{\reward \mid \latentstate, \latentaction} - \log \decodersymbol_{\decoderparameter_1}^\rewards\fun{\reward \mid \latentstate, \action} \right], \\
    \rate_{\encoderparameter_2, \decoderparameter_2} &= \expectedsymbol{\state, \action \sim \stationary{\policy}} \, \expectedsymbol{\latentstate \sim \embed_{\encoderparameter_1}\fun{\sampledot \mid \state}} \dkl{\latentembeda_{\encoderparameter_2}\fun{\sampledot \mid \latentstate, \action}}{\latentpolicy_{\decoderparameter_2}\fun{\sampledot \mid \latentstate}}.
\end{align*}
\end{proposition}
\begin{proof} First, observe that we can re-write the log-likelihood of traces as
\begin{align*}
    \log \decoder\fun{\seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}}
    &= \log \fun{\decodersymbol_{\decoderparameter_1}\fun{\seq{\state}{T}, \seq{\reward}{T-1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}} \prod_{t = 0}^{T - 1} \decodersymbol^\policy_{\decoderparameter_2}\fun{\action_t \mid \state_t}}\\
    &= \log \decodersymbol_{\decoderparameter_1}\fun{\seq{\state}{T}, \seq{\reward}{T-1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}} + \log \decodersymbol_{\decoderparameter_2}^{\policy}\fun{\seq{\action}{T - 1} \mid \seq{\state}{T - 1}}
    \end{align*}
     and the KL divergence between encoder and behavioral distributions over latent sequences as
    \begin{align*}
    &\dkl{\encoder\fun{\sampledot \mid \trace}}{\decoder\fun{\sampledot \mid \trace}} \\
    \begin{aligned}
    = \\ \, \\ \,
    \end{aligned}& \; \begin{aligned}
        \expectedsymbol{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1} \sim \encoder\fun{\sampledot \mid \trace}}[&\log \encodersymbol_{\encoderparameter_1}\fun{\seq{\latentstate}{T} \mid \trace} + \log \encodersymbol_{\encoderparameter_2}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \trace}\\
        &- \log \decodersymbol_{\decoderparameter_1}\fun{\seq{\latentstate}{T} \mid \trace} - \log \decodersymbol_{\decoderparameter}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \trace}]
    \end{aligned} \tag{by definition of KL divergence and chain rule} \\
    \begin{aligned}
    = \\ \, \\ \,
    \end{aligned}& \; \begin{aligned}
        \expectedsymbol{\seq{\latentstate}{T} \sim \encodersymbol_{\encoderparameter_1}\fun{\sampledot \mid \trace}}\Big[& \log \encodersymbol_{\encoderparameter_1}\fun{\seq{\latentstate}{T} \mid \trace} - \log \decodersymbol_{\decoderparameter_1}\fun{\seq{\latentstate}{T} \mid \trace} \\
        &+ \expected{\seq{\latentaction}{T - 1} \sim \encodersymbol_{\encoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}{ \log \encodersymbol_{\encoderparameter_2}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \trace} - \decodersymbol_{\decoderparameter}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \trace}}\Big]
    \end{aligned}\\
    =& \dkl{\encodersymbol_{\encoderparameter_1}\fun{\sampledot \mid \trace}}{\decodersymbol_{\decoderparameter_1}\fun{\sampledot \mid \trace}} + \expectedsymbol{\seq{\latentstate}{T} \sim \encodersymbol_{\encoderparameter_1}} \dkl{\encodersymbol_{\encoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}{\decoder\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}.
\end{align*}
This gives us
\begin{align*}
     &\log \decoder\fun{\seq{\state}{T}, \seq{\action}{T-1}, \seq{\reward}{T-1}, \seq{\labeling}{T}} - \dkl{\encoder\fun{\sampledot \mid \trace}}{\decoder\fun{\sampledot \mid \trace}} \\
     =& \log \decodersymbol_{\decoderparameter_1}\fun{\seq{\state}{T}, \seq{\reward}{T-1}, \seq{\labeling}{T} \mid \seq{\action}{T-1}} + \log \decodersymbol_{\decoderparameter_2}^{\policy}\fun{\seq{\action}{T - 1} \mid \seq{\state}{T - 1}} \\
     &- \dkl{\encodersymbol_{\encoderparameter_1}\fun{\sampledot \mid \trace}}{\decodersymbol_{\decoderparameter_1}\fun{\sampledot \mid \trace}} - \expectedsymbol{\seq{\latentstate}{T} \sim \encodersymbol_{\encoderparameter_1}\fun{\sampledot \mid \trace}} \dkl{\encodersymbol_{\encoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}{\decoder\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}
\end{align*}
which yields the first equality.
Then, by repeatedly applying Bayes' and chain rules, we have
\begin{align*}
    & \log \decoder\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \trace} \\
    = & \log \decodersymbol_{\decoderparameter_2}\fun{\seq{\latentstate}{T}, \trace \mid \seq{\latentaction}{T - 1}} + \log \decodersymbol_{\decoderparameter_2}\fun{\seq{\latentaction}{T - 1}} - \log \decodersymbol_{\decoderparameter}\fun{\seq{\latentstate}{T}, \trace}\\
    = & \log \decodersymbol_{\decoderparameter_2}\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} + \log \latentprobtransitions_{\decoderparameter_2}\fun{\seq{\latentstate}{T} \mid \seq{\latentaction}{T - 1}} + \log \decodersymbol_{\decoderparameter_2}\fun{\seq{\latentaction}{T - 1}} \\
    & - \log \decodersymbol_{\decoderparameter}\fun{\seq{\state}{T}, \seq{\reward}{T - 1}, \seq{\latentstate}{T}, \seq{\action}{T - 1}} \\
    = & \log \decodersymbol_{\decoderparameter_2}\fun{\seq{\state}{T}, \seq{\action}{T - 1}, \seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} + \log \latentprobtransitions_{\latentpolicy, \decoderparameter_2}\fun{\seq{\latentstate}{T}, \seq{\latentaction}{T - 1}}\\
    & - \log \big(\prod_{t = 0}^{T - 1} \decodersymbol^\policy_{\decoderparameter_2}\fun{\action_t \mid \state_t} \cdot \latentprobtransitions_{\decoderparameter_1}\fun{\latentstate_{t + 1} \mid \latentstate_{t}, \action_t} \cdot \decodersymbol_{\decoderparameter_1}^{\rewards}\fun{\reward_t \mid \latentstate_t, \action_t, \latentstate_{t + 1}} \cdot \decodersymbol_{\decoderparameter_1}^{\generative}\fun{\state_{t + 1} \mid \latentstate_{t+1}}\big)\\
    = & \log \decodersymbol_{\decoderparameter_1}^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}} +  \log \decodersymbol_{\decoderparameter_2}^{\generative}\fun{\seq{\action}{T - 1} \mid \seq{\latentstate}{T - 1}, \seq{\latentaction}{T - 1}} + \log  \decodersymbol_{\decoderparameter_2}^\rewards\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} \\
    & + \log \latentpolicy_{\decoderparameter_2}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T - 1}} + \log \latentprobtransitions_{\decoderparameter_2}\fun{\seq{\latentstate}{T} \mid \seq{\latentaction}{T - 1}} \\
    & - \log \decodersymbol_{\decoderparameter_2}^{\policy}\fun{\seq{\action}{T - 1} \mid \seq{\state}{T - 1}} - \log \latentprobtransitions_{\decoderparameter_1}\fun{\seq{\latentstate}{T} \mid \seq{\action}{T - 1}} - \log  \decodersymbol_{\decoderparameter_1}^\rewards\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} \\
    &  - \log \decodersymbol_{\decoderparameter_1}^{\generative}\fun{\seq{\state}{T} \mid \seq{\latentstate}{T}},
\end{align*}
meaning 
\begin{align*}
    & \expected{\trace \sim \mdp_{\policy}}{\log \decodersymbol^\policy_{\decoderparameter_2}\fun{\seq{\action}{T - 1} \mid \seq{\state}{T - 1}} - \expectedsymbol{\seq{\latentstate}{T} \sim \encodersymbol_{\encoderparameter_1}\fun{\sampledot \mid \trace}} \dkl{\encodersymbol_{\encoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}{\decodersymbol_{\decoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}} \\
    =& \expected{\trace \sim \mdp_{\policy}}{\log \decodersymbol^\policy_{\decoderparameter_2}\fun{\seq{\action}{T - 1} \mid \seq{\state}{T - 1}} - \expectedsymbol{}_{\substack{\seq{\latentstate}{T} \sim \encodersymbol_{\encoderparameter_1}\fun{\sampledot \mid \trace} \\ \seq{\latentaction}{T - 1} \sim \encodersymbol_{\encoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \trace}}}  \log \fun{\frac{\encodersymbol_{\encoderparameter_2}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \trace}}{\decodersymbol_{\decoderparameter_2}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \trace}}}} \\
    \begin{aligned}
    = \\ \, \\ \, \\ \, \\ \, \\ \,
    \end{aligned}& \; \begin{aligned}
        \expectedsymbol{}_{\substack{\trace \sim \mdp_{\policy} \\ \seq{\latentstate}{T} \sim \encodersymbol_{\encoderparameter_1}\fun{\sampledot \mid \trace} \\ \seq{\latentaction}{T - 1} \sim \encodersymbol_{\encoderparameter_2}\fun{\sampledot \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}}}} \Bigg[&  \log \decodersymbol_{\decoderparameter_2}^{\generative}\fun{\seq{\action}{T - 1} \mid \seq{\latentstate}{T - 1}, \seq{\latentaction}{T - 1}} \\
        &+ \log \latentprobtransitions_{\decoderparameter_2}\fun{\seq{\latentstate}{T} \mid \seq{\latentaction}{T - 1}} - \log \latentprobtransitions_{\decoderparameter_1}\fun{\seq{\latentstate}{T} \mid \seq{\action}{T - 1}} \\
        & + \log  \decodersymbol_{\decoderparameter_2}^\rewards\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\latentaction}{T - 1}} - \log  \decodersymbol_{\decoderparameter_1}^\rewards\fun{\seq{\reward}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} \\
        & - \log \encodersymbol_{\encoderparameter_2}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T}, \seq{\action}{T - 1}} + \log \latentpolicy_{\decoderparameter_2}\fun{\seq{\latentaction}{T - 1} \mid \seq{\latentstate}{T - 1}}\Bigg],
    \end{aligned}
\end{align*}
which yields the distortion and rate values when applying Lemma~\ref{lemma:trace-to-stationary}.
\end{proof}
%

\smallparagraph{Discrete latent distributions.} Similarly to the latent state space abstraction, we learn discrete latent distributions for $\embeda_{\encoderparameter}$ and $\latentpolicy_{\decoderparameter}$ by learning logits of a continuous relaxation of discrete distributions, through the \emph{Gumbel softmax trick} \citep{DBLP:conf/iclr/JangGP17,DBLP:conf/iclr/MaddisonMT17}.
Let $n = |\latentactions|$, and $\latentactions = \set{\latentaction_1, \dots, \latentaction_n}$.
Drawing $\latentaction_i \sim \categorical{\logits}$  from a discrete (categorical) distribution in $\distributions{\latentactions}$ with logits parameter $\logits \in \R^n$ is equivalent to applying an $\argmax$ operator to the sum of \emph{Gumble samples} and these logits, i.e., $i = \argmax_{k} \logits_k - \log\fun{- \log \vect{\epsilon}_k}$, where $\vect{\epsilon} \in \mathopen[0, 1\mathclose]^n$ is a uniform noise.
The sampling operator being fully reparameterizable here, $\argmax$ is however not derivable, preventing the operation to be optimized through gradient descent.
The proposed solution is to replace the $\argmax$ operator by a softmax function with temperature parameter $\temperature \in \mathopen]0, \left(n - 1\right)^{-1}\mathclose]$.

Concretely, $\vect{x} \in \mathopen[0, 1\mathclose]^n$ has a \emph{relaxed discrete distribution} $\vect{x} \sim \relaxedcategorical{\logits}{\temperature}$ with logits $\logits$, temperature parameter $\temperature$ iff
(a) let $\vect{\epsilon} \in [0, 1]^n$ be a uniform noise and $\vect{G}_k = {- \log \fun{- \log \vect{\epsilon}_k}}$, then $\vect{x}_k = {\frac{\exp{\fun{\fun{\logits_k + \vect{G}_k} \temperature^{-1}}}}{\sum_{i = 1}^{n} \exp{\fun{\fun{\logits_i + \vect{G}_i} \lambda^{-1}}}}}$ for each $k \in [n]$,
(b) $\lim_{\temperature \to 0} \relaxedcategorical{\logits}{\temperature} = \categorical{\logits}$, meaning $\Prob(\textstyle\lim_{\temperature \to 0} \vect{x}_k = 1) = \frac{\exp{\logits_k}}{\sum_{i = 1}^{n}\exp{\logits_i}}$,
and (c) let $p_{\logits, \temperature}$ be the density of $\relaxedcategorical{\logits}{\temperature}$, then $p_{\logits, \temperature}\fun{\vx}$ is log-convex in $\vx$.
In practice, we train $\embeda_{\encoderparameter}$ and $\latentpolicy_{\decoderparameter}$ to infer and generate logits parameter $\logits$, and we anneal $\temperature$ from $(n - 1)^{-1}$ to $0$ during training while using discrete distributions for evaluation.
Again, as prescribed in \cite{DBLP:conf/iclr/MaddisonMT17}, we use two different temperature parameters, one for $\embeda_{\encoderparameter}$ and another for $\latentpolicy_{\decoderparameter}$.

==> wae_objective_function_policy.tex <==
\section{Policy variant (no action encoder)}
We learn the latent space model $\tuple{\latentmdp_{\decoderparameter}, \embed_{\encoderparameter}, \embeda_{\encoderparameter, \decoderparameter}}$
%by adapting the \emph{Wasserstein autoencoder} (WAE) framework introduced by \cite{DBLP:conf/iclr/TolstikhinBGS18}.
by minimizing $\wassersteindist{\transitiondistance}{\stationary{\policy}}{\stationarydecoder}$ such that
% \begin{align*}
%     \stationarydecoder\fun{\sampledot, \sampledot, \reward, \state'} = \stationarydecoder\fun{\reward, \state'} =  \int_{\latentstates} \decoder\fun{\reward, \state' \mid \latentstate'} \latentstationaryprior\fun{\latentstate'} \, d\latentstate' %= \expectedsymbol{\state, \action \sim \stationary{\policy}} \expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \action}} \decoder\fun{\reward, \state' \mid \latentstate'}
% \end{align*}
% for some latent stationary distribution $\latentstationaryprior$.
% Notice that we are here again omitting the label terms since we assume a perfect reconstruction of labels by encoding them directly into the latent space.
% Moreover, we do not desire to learn an action embedding function since we assume the original and latent space models sharing the same action space, we thus make $\decoder$ and $\latentstationaryprior$ dependent on actions generated by $\stationary{\policy}$ as follows:
% \begin{align*}
%     \decoder\fun{\reward, \state' \mid \latentstate'} = \expectedsymbol{\state, \action \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}{\decoder\fun{\reward, \state' \mid \latentstate, \action, \latentstate'}} &&\text{ and }&&
%     \stationarydecoder\fun{\latentstate'} = \expectedsymbol{\state, \action \sim \stationary{\policy}} \expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}{\latentprobtransitions_{\decoderparameter}\fun{\latentstate' \mid \latentstate, \action}}.
% \end{align*}
\begin{align}
    \stationarydecoder\fun{\state, \action, \reward, \state'} =  \int_{\latentstates \times \latentstates} \decoder\fun{\state, \action, \reward, \state' \mid \latentstate, \latentstate'} \, d\latentstationaryprior\fun{\latentstate, \latentstate'} \label{eq:policy-stationary-decoder}
    %= \expectedsymbol{\state, \action \sim \stationary{\policy}} \expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \action}} \decoder\fun{\reward, \state' \mid \latentstate'}
\end{align}
where $\latentstationaryprior$ denotes the stationary distribution of the latent model $\latentmdp_{\decoderparameter}$ and $\latentstate, \latentstate'$ both follow this distribution with $\latentstationaryprior\fun{\latentstate, \latentstate'} = \latentstationaryprior\fun{\latentstate} \cdot \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}} \latentprobtransitions_{\decoderparameter}\fun{\latentstate' \mid \latentstate, \latentaction}$.

Given the definition of $\stationarydecoder$, it is sufficient to find an encoder $\embed$ whose marginal is given by $Q\fun{\latentstate, \latentstate'} = \expectedsymbol{\state, \state' \sim \stationary{\policy}} \embed\fun{\latentstate, \latentstate' \mid \state, \state'}$ % = \embed_{\encoderparameter}\stationary{\policy}$,
and identical to the prior distribution $\latentstationaryprior$ instead of finding the optimal coupling in the primal definition of \wassersteindist{\transitiondistance}{\stationary{\policy}}{\stationarydecoder} \citep{Bousquet2017FromOT,DBLP:conf/iclr/TolstikhinBGS18}.
\begin{theorem}
Let $\mdp$ be an MDP with state-action space $\states \times \actions$, $\latentmdp_{\decoderparameter}
$ be an ergodic latent MDP of $\mdp$ with state-action space $\latentstates \times \latentactions$ and reward function $\latentrewards_{\decoderparameter}$,
%= \tuple{\latentstates, \latentactions, \latentprobtransitions_{\decoderparameter}, \latentrewards_{\decoderparameter}, \latentlabels, \atomicprops, \zinit}$ be a latent MDP of $\mdp$,
$\latentpolicy_{\decoderparameter}$ be a policy for $\latentmdp_{\decoderparameter}$, $\stationarydecoder \in \distributions{\states \times \actions \times \R \times \states}$ and $\decoder \colon \latentstates^2 \to \distributions{\states \times \actions \times \R \times \states}$ be respectively a generator and a decoder as defined in Eq.~\ref{eq:policy-stationary-decoder}, $\generative_{\decoderparameter}\colon \latentstates \to \states$, $\embeda_{\decoderparameter} \colon \latentstates \times \latentactions \to \actions$, and
\begin{equation*}
    G_{\decoderparameter} \colon \latentstates^2 \to \states \times \actions \times \R \times \states, \; \tuple{\latentstate, \latentstate'} \mapsto \tuple{\generative_{\decoderparameter}\fun{\latentstate}, \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}\embeda_{\decoderparameter}\fun{\latentstate, \latentaction}, \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}{\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}}, \generative_{\decoderparameter}\fun{\latentstate'}}
\end{equation*}
\begin{enumerate}[(i)]
\iffalse
\item If $\latentpolicy_{\decoderparameter}$ is deterministic (write $\latentpolicy_{\decoderparameter}\colon \latentstates \to \latentactions$), then so is $\decoder$ when the distribution is characterized by $G_\decoderparameter$, and
%     \begin{align*}
%         \inf_{\coupling \in \couplings{\stationary{\policy}}{\stationarydecoder}} \, \expectedsymbol{\tau, \tau' \sim \coupling} \transitiondistance\fun{\tau, \tau'} = \inf_{Q: Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}} \transitiondistance\fun{\tuple{\state, \action, \reward, \state', \labels\fun{\state'}}, G_{\decoderparameter}\fun{\latentstate, \latentstate'}}
% \end{align*}
\begin{align*}
    \wassersteindist{\tracedistance}{\stationary{\policy}}{\stationarydecoder} = \inf_{\embed:\, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expected{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}{\distance_{\actions}\fun{\action, \embeda_{\decoderparameter}\fun{\latentstate, \latentpolicy_{\decoderparameter}\fun{\latentstate}}} + \left| r - \rewards_{\decoderparameter}\fun{\latentstate, \latentpolicy_{\decoderparameter}\fun{\latentstate}} \right| + \distance_{\states}\fun{\state', \generative_{\decoderparameter}\fun{\latentstate'}}}
\end{align*}
\item Otherwise, assume $\states = \R^{m}$, $\actions = \R^{n}$, and $\decoder\fun{\cdot \mid \latentstate, \latentstate'}$ have mean values $G_{\decoderparameter}\fun{\latentstate, \latentstate'} \in \R^{k}$ and marginal variances $\sigma_1^2, \dots, \sigma^2_{k} \geq 0$ for all $\latentstate, \latentstate' \in \latentstates$ with $k = 2 m + n + 1$. Take $\norm{.}^2_2$ as $\distance_{\states}$, $\distance_{\actions}$, and reward distance metric, then
\begin{align*}
    &\wassersteindist{\tracedistance}{\stationary{\policy}}{\stationarydecoder} \\
    \leq& \sum_{i=m+1}^{k} \sigma_i^2 + \inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expected{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}{\norm{\action - \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}\embeda_{\decoderparameter}\fun{\latentstate, \latentaction}} + \left| r - \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}{\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}} \right| + \norm{\state' - \generative_{\decoderparameter}\fun{\latentstate'}}}^2
\end{align*}
\fi
\item If $\latentpolicy_{\decoderparameter}$ is deterministic, then so is $\decoder$ when $G_\decoderparameter$ is its Dirac function, and
\begin{align*}
    &\wassersteindist{\tracedistance}{\stationary{\policy}}{\stationarydecoder} \\ =& \inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}\expected{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot\mid \latentstate}}{\distance_\states\fun{\state, \generative_{\decoderparameter}\fun{\latentstate}} + \distance_{\actions}\fun{\action, \embeda_{\decoderparameter}\fun{\latentstate, \latentaction}} + \left| r - \rewards_{\decoderparameter}\fun{\latentstate, \latentaction} \right| + \distance_{\states}\fun{\state', \generative_{\decoderparameter}\fun{\latentstate'}}}
\end{align*}
\item Otherwise, assume $\states = \R^{m}$, $\actions = \R^{n}$, and $\decoder\fun{\cdot \mid \latentstate, \latentstate'}$ have mean values $G_{\decoderparameter}\fun{\latentstate, \latentstate'} \in \R^{k}$ and marginal variances $\sigma_1^2, \dots, \sigma^2_{k} \geq 0$ for all $\latentstate, \latentstate' \in \latentstates$ with $k = 2 m + n + 1$.
%Take $\norm{.}^2_2$ as $\distance_{\states}$, $\distance_{\actions}$, and reward distance metric, then
Take the $\ell_2$-distance for $\distance_{\states}$, $\distance_{\actions}$,
%and let $c\fun{\vect{x}, \vect{y}} = \norm{\vect{x} - \vect{y}}^2$, 
then we bound the squared $2$-Wasserstein distance as:
\begin{align*}
    &\wassersteinsymbol{2}^2\fun{\stationary{\policy},{\stationarydecoder}} \\
    \leq& \sum_{i=1}^{k} \sigma_i^2 + \inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}\expected{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}{
    %    \norm{\state - \generative_{\decoderparameter}\fun{\latentstate}}^2 + \norm{\action - \embeda_{\decoderparameter}\fun{\latentstate, \latentaction}}^2 + \left| r - {\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}} \right|^2 + \norm{\state' - \generative_{\decoderparameter}\fun{\latentstate'}}^2
        \distance_{\states}^2\fun{\state, \generative_{\decoderparameter}\fun{\latentstate}} + \distance_{\actions}^2\fun{\action, \embeda_{\decoderparameter}\fun{\latentstate, \latentaction}} + \left| r - {\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}} \right|^2 + \distance_{\states}^2\fun{\state', \generative_{\decoderparameter}\fun{\latentstate'}}
    }
\end{align*}
\end{enumerate}
\end{theorem}
\begin{proof}
%The results follow directly from \citet[Theorem~1 and Corollary~1]{DBLP:conf/iclr/TolstikhinBGS18}.
First, assume $\latentpolicy_{\decoderparameter}$ is deterministic (write $\latentpolicy_{\decoderparameter}\colon \latentstates \to \latentactions$) and assume that $\decoder$ is deterministic with $G_{\decoderparameter}$ as its Dirac function.
In that case, we have
\begin{align*}
    \wassersteindist{\tracedistance}{\stationary{\policy}}{\stationarydecoder} &=
    \inf_{\coupling \in \couplings{\stationary{\policy}}{\stationarydecoder}} \, \expectedsymbol{\tau, \tau' \sim \coupling} \transitiondistance\fun{\tau, \tau'}\\
    &=\inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expected{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}{\distance_{\states}\fun{\state, \generative_{\decoderparameter}\fun{\latentstate}}+\distance_{\actions}\fun{\action, \embeda_{\decoderparameter}\fun{\latentstate, \latentpolicy_{\decoderparameter}\fun{\latentstate}}} + \left| r - \rewards_{\decoderparameter}\fun{\latentstate, \latentpolicy_{\decoderparameter}\fun{\latentstate}} \right| + \distance_{\states}\fun{\state', \generative_{\decoderparameter}\fun{\latentstate'}}} \tag{\citet[Theorem~1]{DBLP:conf/iclr/TolstikhinBGS18}}\\
    &= \inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}\expected{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot\mid \latentstate}}{\distance_{\states}\fun{\state, \generative_{\decoderparameter}\fun{\latentstate}} + \distance_{\actions}\fun{\action, \embeda_{\decoderparameter}\fun{\latentstate, \latentaction}} + \left| r - \rewards_{\decoderparameter}\fun{\latentstate, \latentaction} \right| + \distance_{\states}\fun{\state', \generative_{\decoderparameter}\fun{\latentstate'}}} \tag{since $\latentpolicy_{\decoderparameter}$ is deterministic}
\end{align*}

Second, assume $\states = \R^{m}$, $\actions = \R^{n}$, and $\decoder\fun{\cdot \mid \latentstate, \latentstate'}$ have mean values $G_{\decoderparameter}\fun{\latentstate, \latentstate'} \in \R^{k}$ and marginal variances $\sigma_1^2, \dots, \sigma^2_{k} \geq 0$ for all $\latentstate, \latentstate' \in \latentstates$ with $k = 2 m + n + 1$. Take $\norm{.}^2_2$ as $\distance_{\states}$, $\distance_{\actions}$, and reward distance metric, then %let $g_{\decoderparameter} \colon \latentstates^2 \to \states \times \actions \times \R \times \states , \; \tuple{\latentstate, \latentstate'} \mapsto \tuple{\generative_{\decoderparameter}\fun{\latentstate},  \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}\embeda_{\decoderparameter}\fun{\latentstate, \latentaction}, \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}{\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}}, \generative_{\decoderparameter}\fun{\latentstate'}} $, we have
we have
\begin{align*}
    &\wassersteindist{\tracedistance}{\stationary{\policy}}{\stationarydecoder} \\
    \leq& \sum_{i=m+1}^{k} \sigma_i^2 + \inf_{\coupling \in \couplings{\stationary{\policy}}{\latentstationaryprior}} \,
    \expected{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate', \latentstate'}\sim \coupling}{\norm{\tuple{\state, \action, \reward, \state'} - G_{\decoderparameter}\fun{\latentstate, \latentstate'}}^2} \tag{\citet[Corollary~1]{DBLP:conf/iclr/TolstikhinBGS18}}\\
    %\expected{\trace, \tuple{\latentstate', \latentstate'}\sim \coupling}{\norm{\trace - g_{\decoderparameter}\fun{\latentstate, \latentstate'}}^2} \tag{\citet[Corollary~1]{DBLP:conf/iclr/TolstikhinBGS18}}\\
    =& \sum_{i=m+1}^{k} \sigma_i^2 + \wassersteindist{c}{\stationary{\policy}}{\latentstationaryprior}
    %\leq& \sum_{i=m+1}^{k} \sigma_i^2 + \inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expected{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}{\norm{\action - \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}\embeda_{\decoderparameter}\fun{\latentstate, \latentaction}} + \left| r - \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}{\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}} \right| + \norm{\state' - \generative_{\decoderparameter}\fun{\latentstate'}}}^2
\end{align*}
for $c \colon \fun{\states \times \actions \times \R \times \states} \times \latentstates^2 \to \left[0, + \infty \right[, \; {\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentstate'}} \mapsto \norm{\tuple{\state, \action, \reward, \state'} - g_{\decoderparameter}\fun{\latentstate, \latentstate'}}^2$.
Observe that $\latentstationaryprior\fun{\latentstate, \latentstate'} = \int_{\latentvariables \times \latentvariables} \latentstationaryprior\fun{\latentstate, \latentstate' \mid \latentvariable, \latentvariable'} \,d\Xi\fun{\latentvariable, \latentvariable'}$ for any latent space $\latentvariables$ and latent prior distribution $\Xi \in \distributions{\latentvariables^2}$.
When $\latentvariables = \latentstates$, one can set $\Xi$ to $\latentstationaryprior$ to obtain
$\latentstationaryprior\fun{\latentstate_1, \latentstate_1'} = \int_{\latentstates \times \latentstates} \condition{=}\fun{\tuple{\latentstate_1, \latentstate_1'}, \tuple{\latentstate_2, \latentstate_2'}} \,d\latentstationaryprior\fun{\latentstate_2, \latentstate_2'}$.
Take $G' \colon \latentstates^2 \to \latentstates^2$ be the identity function, then we can apply again \citet[Theorem~1]{DBLP:conf/iclr/TolstikhinBGS18}, which gives us:
\begin{align*}
    &\wassersteindist{\tracedistance}{\stationary{\policy}}{\stationarydecoder}\\
    \leq& \sum_{i=m+1}^{k} \sigma_i^2 + \wassersteindist{c}{\stationary{\policy}}{\latentstationaryprior} \\
    =& \sum_{i=m+1}^{k} \sigma_i^2 + \inf_{\embed:\, Q=\Xi} \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \expectedsymbol{\latentvariable, \latentvariable' \sim \embed\fun{\sampledot \mid \state, \state'}} c\fun{\tuple{\state, \action, \reward, \state'}, G'\fun{\latentvariable, \latentvariable'}} \tag{\citet[Theorem~1]{DBLP:conf/iclr/TolstikhinBGS18}}\\
    =& \sum_{i=m+1}^{k} \sigma_i^2 + \inf_{\embed:\, Q=\latentstationaryprior} \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \expectedsymbol{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}} c\fun{\tuple{\state, \action, \reward, \state'}, \tuple{{\latentstate}, {\latentstate'}}}\\
    =& \sum_{i=m+1}^{k} \sigma_i^2 + \inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}\Big[\norm{\state - \generative_{\decoderparameter}\fun{\latentstate}}^2 + \norm{\action - \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}\embeda_{\decoderparameter}\fun{\latentstate, \latentaction}}^2 + \\
        &  \omit$\hfill \left| r - \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}{\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}} \right|^2 + \norm{\state' - \generative_{\decoderparameter}\fun{\latentstate'}}^2\Big]$\\
    \leq& \sum_{i=m+1}^{k} \sigma_i^2 + \inf_{\embed: \, Q = \latentstationaryprior} \, \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed\fun{\sampledot \mid \state, \state'}}\expected{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\cdot \mid \latentstate}}{\norm{\state - \generative_{\decoderparameter}\fun{\latentstate}}^2 + \norm{\action - \embeda_{\decoderparameter}\fun{\latentstate, \latentaction}}^2 + \left| r - {\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}} \right|^2 + \norm{\state' - \generative_{\decoderparameter}\fun{\latentstate'}}^2} \tag{Jensen's inequality}
\end{align*}
\end{proof}
%
From now on, fix $\embed_\encoderparameter$ as a parameterized state embedding function such that $\embed_\encoderparameter\fun{\latentstate, \latentstate' \mid \state, \state'} = \embed_{\encoderparameter}\fun{\latentstate \mid \state} \cdot \embed_{\encoderparameter}\fun{\latentstate' \mid \state'}$ for any $\state, \state' \in \states$, $\latentstate, \latentstate' \in \latentstates$, and $Q_\encoderparameter = \expectedsymbol{\state, \state' \sim \stationary{\policy}} \embed_{\encoderparameter}\fun{\cdot \mid \state, \state'}$.
Write $\Delta$ for set of deterministic distributions, then let
$\distance_{\states}$ and $\distance_\actions$ be the usual $\ell_2$ distance,
 $\Sigma_{\encoderparameter, \decoderparameter} = \sum_{i = m + 1}^{k} \sigma_i^2 \cdot \condition{\Delta}\fun{\latentpolicy_{\decoderparameter}}$, and
 %$c = \tracedistance^{\; 2 - \condition{\Delta}\fun{\latentpolicy_{\decoderparameter}}}$.
$c\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentaction, \latentstate'}} = \distance_{\states}^{\; 2 - \condition{\Delta}\fun{\latentpolicy_{\decoderparameter}}}\fun{\state, \generative_{\decoderparameter}\fun{\latentstate}} + \distance_{\actions}^{\; 2 - \condition{\Delta}\fun{\latentpolicy_{\decoderparameter}}}\fun{\action, \embeda_{\decoderparameter}\fun{\latentstate, \latentaction}} + \left| r - {\latentrewards_{\decoderparameter}\fun{\latentstate, \latentaction}} \right|^{\; 2 - \condition{\Delta}\fun{\latentpolicy_{\decoderparameter}}} + \distance_{\states}^{\; 2 - \condition{\Delta}\fun{\latentpolicy_{\decoderparameter}}}\fun{\state', \generative_{\decoderparameter}\fun{\latentstate'}}$.

We define the WAE-MDP objective as:
\begin{align*}
    \min_{\encoderparameter, \decoderparameter} \, \Sigma_{\encoderparameter, \decoderparameter} + \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}} \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} c\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentaction, \latentstate'}} + \beta \cdot \divergencesymbol\fun{\encoder, \latentstationaryprior},
\end{align*}
where $\divergencesymbol$ is an arbitrary discrepancy metric and $\beta > 0$ a hyperparameter.
% Take $G_{\decoderparameter}\fun{\latentstate, \action, \latentstate'} = \tuple{\generative_{\decoderparameter}\fun{\latentstate}, \action, \latentrewards_{\decoderparameter}\fun{\latentstate, \action}, \generative_{\decoderparameter}\fun{\latentstate'}, \latentlabels_{\decoderparameter}\fun{\latentstate'}}$ such that we assume a perfect reconstruction of labels through $\latentlabels$ and $\generative_{\decoderparameter} \colon \latentstates \to \states$ being a generative function mapping latent to grounded states.
% Notice that $G_{\decoderparameter}$ maps actions through the identity function since assuming the original and latent space models share the same action space is equivalent to having an action embedding function being the identity function.
% Consequently, the distance term $\transitiondistance\fun{\tuple{\state, \action, \reward, \state', \labels\fun{\state'}}, G_{\decoderparameter}\fun{\latentstate, \action, \latentstate'}}$ becomes simply $\left| \reward - \latentrewards_{\decoderparameter}\fun{\latentstate, \action} \right| + \distance_{\states}\fun{\state', \generative_{\decoderparameter}\fun{\latentstate'}}$.
%
In the same spirit than the work of \citet{DBLP:journals/corr/abs-1902-09323/zhang19}, one can set $\divergencesymbol$ to $\wassersteinsymbol{\distance_{\latentstates}}$, which yields the following Lemmae.
\begin{lemma}\label{lem:policy-regularizer-upper-bound}
Let $\originaltolatentstationary{} \in \distributions{\latentstates \times \latentstates}, \; \tuple{\latentstate, \latentstate'} \mapsto \expected{\state \sim \stationary{\policy}}{\embed_{\encoderparameter}\fun{\latentstate \mid \state} \cdot \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}}{ \latentprobtransitions_{\decoderparameter}\fun{\latentstate' \mid \latentstate, \latentaction}}}$, then
\begin{align*}
    \wassersteindist{\distance_{\latentstates}}{\encoder}{ \latentstationaryprior}
    \leq \wassersteindist{\distance_{\latentstates}}{\encoder}{\originaltolatentstationary{}} + \expectedsymbol{\state, \action \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \wassersteindist{\distance_{\latentstates}}{\embed_{\encoderparameter}\probtransitions\fun{\sampledot \mid \state, \action}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}}
\end{align*}
\end{lemma}
\begin{proof}
Wasserstein is compliant with the triangular inequality \cite{Villani2009}, which gives us:
\begin{align*}
    \wassersteindist{\distance_{\latentstates}}{\encoder}{ \latentstationaryprior}
    \leq \wassersteindist{\distance_{\latentstates}}{\encoder}{\originaltolatentstationary{}} + \wassersteindist{\distance_{\latentstates}}{\originaltolatentstationary{}}{ \latentstationaryprior},
\end{align*}
where
\begin{align}
    \wassersteindist{\distance_{\latentstates}}{\originaltolatentstationary{}}{ \latentstationaryprior} &= \sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy\fun{\sampledot \mid \latentstate}}\expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} f\fun{\latentstate, \latentstate'} - \expectedsymbol{\latentstate \sim \latentstationaryprior}\expectedsymbol{\latentaction \sim \latentpolicy\fun{\sampledot \mid \latentstate}}\expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} f\fun{\latentstate, \latentstate'}\text{, and} \notag\\
    \wassersteindist{\distance_{\latentstates}}{\encoder}{\originaltolatentstationary{}} &=
    \sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state, \action, \state' \sim \stationary{\policy}}\expectedsymbol{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}} f\fun{\latentstate, \latentstate'} - \expectedsymbol{\state \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy\fun{\sampledot \mid \latentstate}}\expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} f\fun{\latentstate, \latentstate'} \label{eq:proof-lemma-wdist-triangular-inequality-4} \\
    &\leq \expectedsymbol{\state, \action \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \; \sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \action}} \expectedsymbol{\latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state'}} f\fun{\latentstate, \latentstate'} - \expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} f\fun{\latentstate, \latentstate'} \label{eq:proof-lemma-wdist-triangular-inequality-5} \\
    &= \expectedsymbol{\state, \action \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \; \sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \action}} \expectedsymbol{\latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state'}} f\fun{\latentstate'} - \expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} f\fun{\latentstate'} \label{eq:proof-lemma-wdist-triangular-inequality-6} \\
    & = \expectedsymbol{\state, \action \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \wassersteindist{\distance_{\latentstates}}{\embed_{\encoderparameter}\probtransitions\fun{\sampledot \mid \state, \action}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}}. \notag
\end{align}
We pass from Eq.~\ref{eq:proof-lemma-wdist-triangular-inequality-4} to Eq.~\ref{eq:proof-lemma-wdist-triangular-inequality-5} by the Jensen's inequality.
To see how we pass from Eq.~\ref{eq:proof-lemma-wdist-triangular-inequality-5} to Eq.~\ref{eq:proof-lemma-wdist-triangular-inequality-6}, notice in the supremum over $\Lipschf{\distance_{\latentstates}}$ of Eq.~\ref{eq:proof-lemma-wdist-triangular-inequality-6} that
\begin{align*}
    \Lipschf{\distance_{\latentstates}} &= \set{f \colon f\fun{\latentstate_1, \latentstate_1'} - f\fun{\latentstate_2, \latentstate_2'} \leq \distance_{\latentstates}\fun{\latentstate_1, \latentstate_2} + \distance_{\latentstates}\fun{\latentstate_1', \latentstate_2'}} \\
    &= \set{f \colon f\fun{\latentstate, \latentstate_1'} - f\fun{\latentstate, \latentstate_2'} \leq \distance_{\latentstates}\fun{\latentstate, \latentstate} + \distance_{\latentstates}\fun{\latentstate_1', \latentstate_2'}} \tag{where $\latentstate$ is drawn from $\embed_{\encoderparameter}$} \\
    &= \set{f \colon f\fun{\latentstate_1'} - f\fun{\latentstate_2'} \leq \distance_{\latentstates}\fun{\latentstate_1', \latentstate_2'}}.
\end{align*}
\end{proof}
\begin{lemma}
% If $\embed_{\encoderparameter}$ is deterministic and traces are generated by running $\latentpolicy_{\decoderparameter}$ in the environment, then
Assume traces are generated by running $\latentpolicy_{\decoderparameter}$ in the environment, then
\begin{align*}
    %\wassersteindist{\distance_{\latentstates}}{\encoder}{ \latentstationaryprior}\leq
    \wassersteindist{\distance_{\latentstates}}{\encoder}{\originaltolatentstationary{}} + \wassersteindist{\distance_{\latentstates}}{\originaltolatentstationary{}}{ \latentstationaryprior} = \localtransitionloss{\stationary{\latentpolicy_{\decoderparameter}}}.
\end{align*}
\end{lemma}
\begin{proof}
Recall that we defined $\latentpolicy_{\decoderparameter}\fun{\sampledot \mid \state} = \expectedsymbol{\latentstate \sim \embed\fun{\sampledot \mid \state}}\latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentaction}$ for any $\state \in \states$.
Observe that $\wassersteindist{\distance_{\latentstates}}{\latentprobtransitions_{\latentpolicy_{\decoderparameter}}\stationary{\latentpolicy_{\decoderparameter}}}{ \latentstationaryprior} = 0$ (both distributions match).
%
Then, notice that 
\begin{align*}
&\wassersteindist{\distance_{\latentstates}}{\encoder}{\latentprobtransitions_{\latentpolicy_{\decoderparameter}}\stationary{\latentpolicy_{\decoderparameter}}} \\
=& \wassersteindist{\distance_{\latentstates}}{\encoder}{\latentstationaryprior}\\
=& \sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state, \state' \sim \stationary{\latentpolicy_{\decoderparameter}}}\expectedsymbol{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}} f\fun{\latentstate, \latentstate'} - \expectedsymbol{\state \sim \stationary{\latentpolicy_{\decoderparameter}}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}}\expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} f\fun{\latentstate, \latentstate'}\\
\leq& \expectedsymbol{\state \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}}\expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}} \; \sup_{f \in \Lipschf{\distance_{\latentstates}}} \expectedsymbol{\state' \sim \probtransitions\fun{\sampledot \mid \state, \latentaction}} \expectedsymbol{\latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state'}} f\fun{\latentstate'} - \expectedsymbol{\latentstate' \sim \latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}} f\fun{\latentstate'} \tag{by the Jensen's inequality and the development of $\Lipschf{\distance_{\latentstates}}$ in the proof of Lemma~\ref{lem:regularizer-upper-bound}.} \\
=& \expectedsymbol{\state, \latentaction \sim \stationary{\latentpolicy_{\decoderparameter}}} \wassersteindist{\distance_{\latentstates}}{\embed_{\encoderparameter}\probtransitions\fun{\sampledot \mid \state, \latentaction}}{\latentprobtransitions\fun{\sampledot \mid \embed_{\encoderparameter}\fun{\state}, \latentaction}} \\
=& \localtransitionloss{\stationary{\latentpolicy_{\decoderparameter}}}.
\end{align*}
\end{proof}

We choose to minimize the upper bound induced by Lemma~\ref{lem:regularizer-upper-bound} to recover the local transition loss when the latent policy matches the original one, which yields the following W$^2$AE-MDP (\emph{Wasserstein-Wasserstein auto-encoded MDP}) objective:
\begin{multline*}
    \min_{\encoderparameter, \decoderparameter} \, \Sigma_{\decoderparameter} + \expectedsymbol{\state, \action, \reward, \state' \sim \stationary{\policy}} \, \expectedsymbol{\latentstate, \latentstate' \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state, \state'}} \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}}{ c\fun{\tuple{\state, \action, \reward, \state'}, \tuple{\latentstate, \latentaction, \latentstate'}}} \\
    + \beta \cdot \fun{ \wassersteindist{\distance_{\latentstates}}{\originaltolatentstationary{}}{ \latentstationaryprior} + \expectedsymbol{\state, \action \sim \stationary{\policy}}\expectedsymbol{\latentstate \sim \embed_{\encoderparameter}\fun{\sampledot \mid \state}} \expectedsymbol{\latentaction \sim \latentpolicy_{\decoderparameter}\fun{\sampledot \mid \latentstate}}\wassersteindist{\distance_{\latentstates}}{\embed_{\encoderparameter}\probtransitions\fun{\sampledot \mid \state, \action}}{\latentprobtransitions_{\decoderparameter}\fun{\sampledot \mid \latentstate, \latentaction}}}
\end{multline*}

